Engineering Trustworthy AI: A Developer Guide for Empirical Risk Minimization

AI systems increasingly shape critical decisions across personal and societal domains. While empirical risk minimization (ERM) drives much of the AI success, it typically prioritizes accuracy over trustworthiness, often resulting in biases, opacity, and other adverse effects. This paper discusses how key requirements for trustworthy AI can be translated into design choices for the components of ERM. We hope to provide actionable guidance for building AI systems that meet emerging standards for trustworthiness of AI.

==> ADictML_Glossary.tex <==

\newglossaryentry{minimum}
{
	name=minimum,
	description={Given a set of real numbers, the minimum\index{minimum} is the smallest of those numbers.},
	first={minimum},text={minimum}
}


\newglossaryentry{maximum}
{name=maximum,
 description={Given a set of real numbers, the maximum\index{maximum} is the largest of those numbers.},
 first={maximum},text={maximum}
}

\newglossaryentry{discrepancy}
{name=discrepancy,
	description={
		Consider\index{discrepancy} a \gls{fl} application with \gls{netdata} represented by a \gls{empgraph}. 
		\gls{fl} methods use a discrepancy measure to compare \gls{hypothesis} maps from 
	local models at nodes $\nodeidx,\nodeidx'$ connected by an edge in the \gls{empgraph}.},
	first={discrepancy},text={discrepancy}
}



\newglossaryentry{hfl}
{name={horizontal \gls{fl}},description=
	{Horizontal \gls{fl}\index{horizontal FL} uses \gls{localdataset}s that are 
		constituted by different \gls{datapoint}s but using the same \gls{feature}s 
		to characterize them \cite{HFLChapter2020}. For example, weather 
		forecasting uses a network of spatially distributed weather (observation) 
		stations. Each weather station measures the same quantities such as daily 
		temperature, air pressure and precipitation. However, different weather 
		stations measure the characteristics or \gls{feature}s of different spatio-temporal regions 
		(each such region being a separate \gls{datapoint}).},
	first={horizontal \gls{fl}},text={horizontal \gls{fl}}
} 

\newglossaryentry{dimred}
{name={dimensionality reduction},
	description={Dimensionality reduction\index{dimensionality reduction} methods 
		map (typically many) raw \gls{feature}s to a (relatively small) set of new features. 
		These methods can be used to visualize \gls{datapoint}s by learning two \gls{feature}s 
		that can be used as the coordinates of a depiction in a \gls{scatterplot}.}, first={dimensionality reduction},text={dimensionality reduction}
} 

\newglossaryentry{featlearn}
{name={feature learning},
	description={Feature learning\index{feature learning} refers to the task of learning a map $\featuremapvec$ that 
		reads in raw \gls{feature}s of a \gls{datapoint} and delivers new \gls{feature}s. Different 
		\gls{feature} learning methods are obtained for different quantitative measures for the 
		usefulness of the new \gls{feature}s.},
	first={feature learning},text={feature learning}
} 

\newglossaryentry{autoencoder}
{name={autoencoder},
	description={An autoencoder\index{autoencoder} is a ML method that jointly learns an encoder map 
		$\hypothesis(\cdot) \in \hypospace$ and a decoder map $\hypothesis^{*}(\cdot) \in \hypospace^{*}$. 
		It is an instance of \gls{erm} using a \gls{loss} computed from the reconstruction error 
		$\featurevec - \hypothesis^{*}\big(  \hypothesis \big( \featurevec \big) \big)$.},
	first={autoencoder},text={autoencoder}
} 

\newglossaryentry{vfl}
{name={vertical \gls{fl}},description=
	{Vertical \gls{fl}\index{vertical FL} uses \gls{localdataset}s that are constituted 
	 by the same \gls{datapoint}s but characterizing them with different \gls{feature}s \cite{VFLChapter}. 
     For example, different healthcare providers might all contain information 
     about the same population of patients. However, different healthcare providers 
     collect different measurements (blood values, electrocardiography, lung X-ray) 
     for the same patients.},
	first={vertical \gls{fl}},text={vertical \gls{fl}}
} 

\newglossaryentry{interpretability}
{name={interpretability},description=
		{A ML method is interpretable\index{interpretability} for a specific user if 
			they can well anticipate the \gls{prediction}s delivered by the method. 
			The notion of interpretability can be made precise using quantitative 
			measures of the uncertainty about the \gls{prediction}s \cite{JunXML2020}.},
		first={interpretability},text={interpretability}
}

\newglossaryentry{multitask learning}
{name={multitask learning},description=
	{Multitask learning\index{multitask learning} aims at leveraging relations between 
	 different \gls{learningtask}s. Consider two \gls{learningtask}s obtained from the 
	 same \gls{dataset} of webcam snapshots. The first task is to predict the presence 
	 of a human, while the second is the predict the presence of a car. It might be useful 
	 to use the same \gls{deepnet} structure for both tasks and only allow the weights of 
	 the final output layer to be different.},
	first={multitask learning},text={multitask learning}
}

\newglossaryentry{learningtask}
{name={learning task},description=
	{Consider\index{learning task} a \gls{dataset} $\dataset$ constituted by several \gls{datapoint}s, each of them 
	 characterized by \gls{feature}s $\featurevec$. For example, the \gls{dataset} $\dataset$ 
	 might be constituted by the images of a particular database. Sometimes it might be useful 
	 to represent a \gls{dataset} $\dataset$, along with the choice of \gls{feature}s, by a \gls{probdist} $p(\featurevec)$. 
	 A learning task associated with $\dataset$ consists of a specific 
	 choice for the \gls{label} of a \gls{datapoint} and the corresponding \gls{labelspace}. 
	 Given a choice for the \gls{lossfunc} and \gls{model}, a learning task gives rise to an 
	 instance of \gls{erm}. Thus, we could define a learning task also via an instance of \gls{erm}, i.e., 
	 via an objective function.  Note that, for the same \gls{dataset}, we obtain different learning tasks by using 
	 different choices for the \gls{feature}s and \gls{label} of a \gls{datapoint}. These learning 
	 tasks are related, as they are based on the same \gls{dataset}, and solving them jointly 
	 (via multitask learning methods) is typically preferable over solving them separately \cite{Caruana:1997wk,JungGaphLassoSPL,CSGraphSelJournal}.},
	first={learning task},text={learning task}
}

\newglossaryentry{featuremtx}
{name={feature matrix},description=
	{Consider\index{feature matrix} a \gls{dataset} $\dataset$ of $\samplesize$ \gls{datapoint}s that are 
	characterized by feature vectors $\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)}$. It is 
	convenient to collect the individual \gls{feature} vectors into a \gls{feature} 
	matrix $\mX \defeq \big(\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)}\big)$. },
	first={feature matrix},text={feature matrix}
}



\newglossaryentry{explainability}
{name={explainability},description=
		{We\index{explainability} define the (subjective) explainability of a ML method 
			as the level of simulatability \cite{Colin:2022aa} of the \gls{prediction}s 
			delivered by a ML system to a human user. Quantitative measures for the 
			(subjective) explainability of a trained \gls{model} can be constructed by 
			comparing its \gls{prediction}s with the \gls{prediction}s provided by a user 
			on a test-set \cite{Zhang:2024aa,Colin:2022aa}. Alternatively, we can use 
			\gls{probmodel}s for \gls{data} and measure explainability of a trained ML model 
			via the conditional (differential) entropy of its \gls{prediction}s, given the user \gls{prediction}s \cite{JunXML2020,Chen2018}. 
		},
		first={explainability},text={explainability}
	}

\newglossaryentry{linmodel}{name={linear model},
	description={Consider\index{linear model}  \gls{datapoint}s, each characterized by a numeric \gls{feature} 
		vector $\featurevec \in \mathbb{R}^{\featuredim}$. A linear \gls{model} is 
		a \gls{hypospace} which consists of all linear maps, 
	\begin{equation} 
		\label{equ_def_lin_model_hypspace}
		\linmodel{\nrfeatures} \defeq \left\{ \hypothesis(\featurevec)= \weights^{T} \featurevec: \weights \in \mathbb{R}^{\nrfeatures} \right\}. 
	\end{equation} 
	Note that \eqref{equ_def_lin_model_hypspace} defines an entire family of \gls{hypospace}s, which is 
	parametrized by the number $\nrfeatures$ of \gls{feature}s that are linearly combined to form the 
	\gls{prediction} $\hypothesis(\featurevec)$. The design choice of $\nrfeatures$ is guided by \gls{compasp} 
	(smaller $\nrfeatures$ means less computation), \gls{statasp} (increasing $\nrfeatures$ might 
	reduce \gls{prediction} error) and \gls{interpretability}. A linear \gls{model} using few carefully chosen 
	\gls{feature}s tends to be considered more interpretable \cite{Ribeiro2016,rudin2019stop}.}, 
   first={linear model},text={linear model}}
	
	
\newglossaryentry{gradstep}{name={gradient step},description={Given a \gls{differentiable} 
		real-valued function $f(\weights)$ and a vector $\weights'$, the \gls{gradient} step\index{gradient step} 
		updates $\weights'$ by adding the scaled negative \gls{gradient} $\nabla f(\weights')$, $\weights' \mapsto \weights' - \lrate \nabla f(\weights')$.},first={gradient step},text={gradient step}}
	

\newglossaryentry{proxop}{name={proximal operator},description={Given\index{proximal operator} a \gls{convex} function 
		and a vector $\vx$, we define its proximal operator as \cite{ProximalMethods,Bauschke:2017} $$\proximityop{\locallossfunc{\nodeidx}{\cdot}}{\weights''}{2 \regparam}\defeq \argmin_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights) + (\rho/2) \normgeneric{\weights- \weights'}{2}^{2} \mbox{ with } \rho > 0. $$ 
		\Gls{convex} functions for which the proximal operator can be computed efficiently 
		are sometimes referred to as \emph{proximable} or \emph{simple} \cite{Condat2013}.},first={proximal operator},text={proximal operator}}

\newglossaryentry{proximable}{name={proximable},description={A\index{proximable} 
		\gls{convex} function for which the \gls{proxop} can be computed efficiently are 
		sometimes referred to as \emph{proximable} or \emph{simple} \cite{Condat2013}.},first={proximable},text={proximable}}


\newglossaryentry{connected}{name ={connected graph}, description={A\index{connected graph} 
		undirected graph $\graph=\pair{\nodes}{\edges}$ is connected\index{connected graph} if 
		it does not contain a (non-empty) subset $\nodes' \subset \nodes$ with no edges leaving 
		$\nodes'$.}, first={connected},text={connected}}

\newglossaryentry{mvndist}{name ={multivariate normal distribution}, description={The\index{multivariate normal distribution} 
		multivariate normal distribution $\mvnormal{\vm}{\mC}$ is an 
		important family of \gls{probdist}s for a continuous \gls{rv} $\featurevec \in \mathbb{R}^{\nrfeatures}$ \cite{BertsekasProb,GrayProbBook,Lapidoth09}. 
		This family is parametrized by the mean $\vm$ and \gls{covmtx} $\mC$ of $\featurevec$. 
		If the \gls{covmtx} is invertible, the \gls{probdist} of $\featurevec$ is 
		$$p(\featurevec) \propto \exp\bigg(-(1/2) \big( \featurevec - \vm \big)^{T} \mC^{-1} \big( \featurevec - \vm \big) \bigg).$$}, first={multivariate normal distribution},text={multivariate normal distribution}}

\newglossaryentry{statasp}{name ={statistical aspects}, description={By statistical aspects\index{statistical aspects} 
		of a ML method, we refer to (properties of) the \gls{probdist} of its output 
		under a \gls{probmodel} for the data fed into the method.},first={statistical aspects},text={statistical aspects}}

\newglossaryentry{compasp}{name ={computational aspects}, description={By computational 
		aspects\index{computational aspects} of a ML method, we mainly refer to the computational 
		resources required for its implementation. For example, if a ML method uses iterative 
		optimization techniques to solve \gls{erm}, then its computational aspects include (i) how 
		many arithmetic operations are needed to implement a single iteration (\gls{gradstep}) 
		and (ii) how many iterations are needed to obtain useful \gls{modelparams}. One important 
		example of an iterative optimization technique is \gls{gd}.}, first={computational aspects},text={computational aspects}}

\newglossaryentry{zerooneloss}{name={$0/1$ \gls{loss}},
	description={The $0/1$ \gls{loss}\index{$0/1$ loss} $\lossfunc{\pair{\featurevec}{\truelabel}}{\hypothesis}$ 
		measures the quality of a \gls{classifier} $\hypothesis(\featurevec)$ that delivers a \gls{prediction} $\predictedlabel$ (e.g., 
	via thresholding \eqref{equ_def_threshold_bin_classifier}) for the \gls{label} $\truelabel$ of a \gls{datapoint} with \gls{feature}s 
	$\featurevec$. 
	It is equal to $0$ if the \gls{prediction} is correct, i.e., 
	$\lossfunc{\pair{\featurevec}{\truelabel}}{\hypothesis}=0$ when $\predictedlabel=\truelabel$. It is 
	equal to $1$ if the \gls{prediction} is wrong, $\lossfunc{\pair{\featurevec}{\truelabel}}{\hypothesis}=1$ 
	when $\predictedlabel\neq\truelabel$.},
	sort=zerooneloss, 
    first={$0/1$ \gls{loss}},text={$0/1$ \gls{loss}}}

\newglossaryentry{probability}{name={probability},
	description={We\index{probability} assign a probability value, typically chosen in the 
		interval $[0,1]$, to each event that might occur in a random experiment \cite{KallenbergBook,BertsekasProb,BillingsleyProbMeasure,HalmosMeasure}.},first={probability},text={probability}}
	
\newglossaryentry{underfitting}{name={underfitting},description={Consider\index{underfitting} a ML method that uses 
		\gls{erm} to learn a \gls{hypothesis} with minimum \gls{emprisk} on a given \gls{trainset}. 
		Such a method is \emph{underfitting} the \gls{trainset} if it is not able to learn a \gls{hypothesis} 
		with sufficiently small \gls{emprisk} on the \gls{trainset}. If a method is underfitting it will typically 
	also not be able to learn a \gls{hypothesis} with a small \gls{risk}.},first={underfitting},text={underfitting}}

\newglossaryentry{overfitting}{name={overfitting},description={Consider\index{overfitting} a ML method that uses 
		\gls{erm} to learn a \gls{hypothesis} with minimum \gls{emprisk} on a given \gls{trainset}. 
		Such a method is \emph{overfitting} the \gls{trainset} if it learns \gls{hypothesis} with small 
		\gls{emprisk} on the \gls{trainset} but significantly larger \gls{loss} outside the \gls{trainset}.},first={overfitting},text={overfitting}}

\newglossaryentry{gdpr}{name={General Data Protection Regulation},description={The \emph{general data 
			protection regulation}\index{GDPR} (GDPR) is a law that has been passed by the European Union (EU) 
			and put into effect on May 25, 2018 \url{https://gdpr.eu/tag/gdpr/}. The GDPR imposes obligations 
			onto organizations anywhere, so long as they target, collect or in any other way process data 
			related to people (i.e., personal data) in the EU \cite{GDPR2016}.}, 
	first={general data protection regulation (GDPR) },text={GDPR}}
	
\newglossaryentry{gaussrv}{name={Gaussian random variable},description={A\index{Gaussian random variable} 
		Gaussian \gls{rv} $\vx \in \mathbb{R}^{\nrfeatures}$ with a \gls{mvndist}. The special case of $\nrfeatures=1$ 
		corresponds to a scalar Gaussian \gls{rv} \cite{papoulis,BertsekasProb,GrayProbBook}.},first={Gaussian RV},text={Gaussian RV}}

\newglossaryentry{trustworthiness}{name={trustworthiness},description=
	{Beside the \gls{compasp} and \gls{statasp}, a third main design aspect for ML methods 
		is their trustworthiness\index{trustworthy AI} \cite{pfau2024engineeringtrustworthyaideveloper}. 
		The European Union has put forward seven key requirements (KRs) for trustworthy 
		AI (that typically build on ML methods)
	\cite{ALTAIEU}: {\bf KR1 - Human Agency and Oversight}, {\bf KR2 - Technical Robustness and Safety}, 
	{\bf KR3 - Privacy and Data Governance}, {\bf KR4 - Transparency}, {\bf KR5 - Diversity Non-Discrimination and Fairness}, 
	{\bf KR6 Societal and Environmental Well-Being}, {\bf KR7 - Accountability}. 
	},first={trustworthiness},text={trustworthiness}}

\newglossaryentry{sqerrloss}{name={squared error loss},description={The squared 
		error\index{squared error loss} \gls{loss} measures the prediction error of a 
		\gls{hypothesis} $\hypothesis$ when predicting a numeric \gls{label} $\truelabel \in \mathbb{R}$ 
		from the \gls{feature}s $\featurevec$ of a \gls{datapoint}. It is 
	defined as 
\begin{equation} 
	\nonumber
%	\label{equ_squared_loss_gls}
	\lossfunc{(\featurevec,\truelabel)}{\hypothesis} \defeq \big(\truelabel - \underbrace{\hypothesis(\featurevec)}_{=\predictedlabel} \big)^{2}. 
\end{equation} 
},first={squared error loss},text={squared error loss}}


\newglossaryentry{projgd}{name={projected GD},description={Projected\index{projected gradient descent} \gls{gd} 
		extends basic \gls{gd} for unconstrained optimization to handle constraints on the 
		optimization variable (\gls{modelparams}). A single iteration of projected \gls{gd} consists 
		of first taking a \gls{gradstep} and then projecting the result back into a 
		constrain set.},first={projected \gls{gd}},text={projected \gls{gd}}}

\newglossaryentry{diffpriv}
{name=differential privacy,
  description={
  	Consider\index{differential privacy} some ML method $\algomap$ that reads in a $\dataset$ 
  	and delivers some output $\algomap(\dataset)$. The output could be the learnt \gls{modelparams} 
  	$\widehat{\weights}$ or the \gls{prediction} $\learnthypothesis(\featurevec)$ obtained for a specific \gls{datapoint} 
  	with \gls{feature}s $\featurevec$. Differential privacy is a precise measure of privacy leakage incurred 
  	by revealing the output $\algomap(\dataset)$. Roughly speaking, the algorithm is differentially 
  	private if the \gls{probdist} of $\algomap(\dataset)$ does not change too much if a \gls{sensattr} 
  	of one \gls{datapoint} in $\dataset$ is changed.}, 
	first = {differential privacy (DP)}, text={DP} 
}

\newglossaryentry{privprot}
{name=privacy protection,
     description={Consider\index{privacy protection} some ML method $\algomap$ that reads in a $\dataset$ 
     	and delivers some output $\algomap(\dataset)$. The output could be the learnt \gls{modelparams} 
     	$\widehat{\weights}$ or the \gls{prediction} $\learnthypothesis(\featurevec)$ obtained for a specific \gls{datapoint} 
		with \gls{feature}s $\featurevec$. Many important ML applications involve \gls{datapoint}s 
		representing humans. Each \gls{datapoint} is characterized by \gls{feature}s $\featurevec$, 
		potentially a \gls{label} $\truelabel$ and a \gls{sensattr} $\sensattr$ (e.g., a recent medical diagnosis). 
		Roughly speaking, \gls{privprot} means that it should be impossible to infer, from the output $\algomap(\dataset)$, 
		any of the \gls{sensattr}s of \gls{datapoint}s in $\dataset$. Mathematically, \gls{privprot} requires non-invertibility 
		of the map $\algomap(\dataset)$. In general, just making $\algomap(\dataset)$ non-invertible 
		is typically insufficient for \gls{privprot}. We need to make $\algomap(\dataset)$ sufficiently non-invertible. 
	}, 
	first = {privacy protection}, text={privacy protection} 
}

\newglossaryentry{privleakage}
{
	name=privacy leakage,
	description={Consider\index{privacy leakage} a (ML or \gls{fl}) system that processes a \gls{localdataset} $\localdataset{\nodeidx}$ 
		and shares data, such as the predictions obtained for new \gls{datapoint}s, with 
		other parties. Privacy leakage arises if the shared data carries information about a 
		private (sensitive) \gls{feature} of a \gls{datapoint} (which might be a human) of $\localdataset{\nodeidx}$.  
		The amount of privacy leakage can be measured via \gls{mutualinformation} using a 
		\gls{probmodel} for the local \gls{dataset}. Another quantitative measure for privacy 
		leakage is \gls{diffpriv}. 
	}, 
	first = {privacy leakage}, text={privacy leakage} 
}



\newglossaryentry{probmodel}
{
	name=probabilistic model,
	description={A probabilistic model\index{probabilistic model} interprets \gls{datapoint}s 
		as \gls{realization}s of \gls{rv}s with a joint \gls{probdist}. This joint \gls{probdist} typically 
		involves parameters which have to be manually chosen or learnt via statistical inference 
		methods such as \gls{ml} \cite{LC}. }, 
	first = {probabilistic model}, text={probabilistic model} 
}



\newglossaryentry{mean}
{
	name=mean,
	description={The\index{mean} expectation $\expect \{ \featurevec \}$ of a numeric \gls{rv} $\featurevec$.}, 
		first = {mean}, text={mean} 
}

\newglossaryentry{variance}
{
	name={variance},
	description={The\index{variance} variance of a real-valued \gls{rv} $\feature$ is defined as the expectation 
		$\expect\big\{ \big( x - \expect\{x \} \big)^{2} \big\}$ of the squared difference $\feature$ 
		and its expectation $\expect\{x \}$. We extend this definition to vector-valued \gls{rv}s $\featurevec$ 
		as $\expect\big\{ \big\| \featurevec - \expect\{\featurevec \} \big\|_{2}^{2} \big\}$.} ,first={variance},text={variance} 
}

\newglossaryentry{nn}
{
	name={nearest neighbour},
	description={Nearest neighbour\index{nearest neighbour} methods learn a \gls{hypothesis} 
		$\hypothesis: \featurespace \rightarrow \labelspace$ whose function value $\hypothesis(\featurevec)$ 
		is solely determined by the nearest neighbours within a given \gls{dataset}. Different 
		methods use different metrics for determining the nearest neighbours. If \gls{datapoint}s 
		are characterized by numeric \gls{feature} vectors, we can use their Euclidean distances as 
		the metric.},
	first={nearest neighbour (NN)},text={NN} 
}

\newglossaryentry{neighbourhood}
{
	name={neighbourhood},
	description={The\index{neighbourhood} neighbourhood of a node $\nodeidx \in \nodes$ is the subset of nodes 
	constituted by the \gls{neighbours} of $\nodeidx$.},
	first={neighbourhood},text={neighbourhood} 
}


\newglossaryentry{neighbours}
{
	name={neighbours},
	description={The\index{neighbours} neighbours of a node $\nodeidx \in \nodes$ within a \gls{empgraph} are 
	those nodes $\nodeidx' \in \nodes \setminus \{ \nodeidx\}$ that are connected (via an edge) to node $\nodeidx$.},
	first={neighbours},text={neighbours} 
}

\newglossaryentry{bias}
{
	name={bias},
	description={Consider\index{bias} a ML method using a parametrized \gls{hypospace} $\hypospace$. 
		It learns the \gls{modelparams} $\weights \in \mathbb{R}^{\dimlocalmodel}$ using the \gls{dataset} $\dataset=\big\{ \pair{\featurevec^{(\sampleidx)}}{\truelabel^{(\sampleidx)}} \big\}_{\sampleidx=1}^{\samplesize}$. 
		To analyze the properties of the ML method, we typically interpret the \gls{datapoint}s as \gls{realization}s 
		of \gls{iid} \gls{rv}s, $$ \truelabel^{(\sampleidx)} = \hypothesis^{(\overline{\weights})}\big( \featurevec^{(\sampleidx)} \big) + \bm{\varepsilon}^{(\sampleidx)}, \sampleidx=1,\ldots,\samplesize.$$ 
		We can then interpret the ML method as an estimator $\widehat{\weights}$, 
		computed from $\dataset$ (e.g., by solving \gls{erm}). The (squared) bias incurred by the estimate $\widehat{\weights}$ 
		is then defined as $\biasterm^{2} \defeq \big\| \expect \{ \widehat{\weights}  \}- \overline{\weights}\big\|_{2}^{2}$. },
first={bias},text={bias} 
}

\newglossaryentry{classification}
{
	name={classification},
	description={Classification\index{classification} is the task of determining a 
		discrete-valued label $\truelabel$ of a \gls{datapoint} based solely on its 
		features $\featurevec$. The label $\truelabel$ belongs to a finite set, such 
		as $\truelabel \in \{ -1,1\}$, or $\truelabel \in \{1,\ldots,19\}$ and represents a 
		category to which the corresponding \gls{datapoint} belongs to. Some classification 
		problems involve a countably infinite \gls{labelspace}.},first={classification},text={classification} 
}


\newglossaryentry{privfunnel}
{
	name={privacy funnel},
	description={The privacy funnel is a method for learning privacy-friendly features of \gls{datapoint}s \cite{MakhdoumiFunnel2014}. },
	first={privacy funnel},text={privacy funnel} 
}




\newglossaryentry{condnr}
{
	name={condition number},
	description={The condition number\index{condition number} $\kappa(\mathbf{Q}) \geq 1$ of a \gls{psd} 
		matrix $\mathbf{Q}$ is the ratio $\eigvalgen_{\rm max} /\eigvalgen_{\rm min}  $ between the 
		largest $\eigvalgen_{\rm max}$ and the smallest $\eigvalgen_{\rm min}$ \gls{eigenvalue} of 
		$\mathbf{Q}$. The condition number is useful for the analysis of ML methods. 
		The computational complexity of \gls{gdmethods} for \gls{linreg} crucially depends on the 
		condition number of the matrix $\mQ = \mX \mX^{T}$, with the \gls{featuremtx} $\mX$ 
		of the \gls{trainset}. Thus, from a computational perspective, we prefer \gls{feature}s of 
		\gls{datapoint}s such that $\mQ$ has a condition number close to $1$.},first={condition number},text={condition number} 
}

\newglossaryentry{classifier}
{
	name={classifier},
	description={A classifier\index{classifier} is a \gls{hypothesis} (map) $\hypothesis(\featurevec)$ 
		used to predict a \gls{label} taking values from a finite \gls{labelspace}. We might use the 
		function value $\hypothesis(\featurevec)$ itself as a \gls{prediction} $\predictedlabel$ for 
		the \gls{label}. However, it is customary to use a map $\hypothesis(\cdot)$ that delivers 
		a numeric quantity. The \gls{prediction} is then obtained by a simple thresholding step. 
		For example, in a binary classification problem with \label{labelspace} $\labelspace \in  \{ -1,1\}$, 
		we might use real-valued \gls{hypothesis} map $\hypothesis(\featurevec) \in \mathbb{R}$ 
		as classifier. A \gls{prediction} $\predictedlabel$ can then be obtained via thresholding,  
		 \begin{equation} 
		 	\label{equ_def_threshold_bin_classifier}
		 	\predictedlabel =1   \mbox{ for } \hypothesis(\featurevec) \geq 0, \mbox{ and } 	\predictedlabel =-1  \mbox{ otherwise.}
	 		\end{equation}
 		We can characterize a classifier by its \gls{decisionregion}s $\decreg{a}$, for 
 		every possible \gls{label} value $a \in \labelspace$. },first={classifier},text={classifier} 
}

\newglossaryentry{emprisk}
{name={empirical risk},
  description={The empirical risk\index{empirical risk} $\emprisk{\hypothesis}{\dataset}$ 
  	of a \gls{hypothesis} on a \gls{dataset} $\dataset$ is the average \gls{loss} incurred 
  	by $\hypothesis$ when applied to the \gls{datapoint}s in $\dataset$.},
  first={empirical risk},text={empirical risk} 
}

\newglossaryentry{nodedegree}
{name={node degree},
	description={The degree\index{node degree} $\nodedegree{\nodeidx}$ of a node $\nodeidx \in \nodes$ 
		in an undirected \gls{graph} is the number of its \gls{neighbours}, $\nodedegree{\nodeidx} \defeq \big|\neighbourhood{\nodeidx}\big|$.},first={node degree},text={node degree} 
}

\newglossaryentry{graph}
{name={graph},
	description={A graph\index{graph} $\graph = \pair{\nodes}{\edges}$ is a pair that consists of 
		a node set $\nodes$ and an edge set $\edges$. In its most general form, a graph is 
		specified by a map that assigns to each edge $\edgeidx \in \edges$ a pair of nodes \cite{RockNetworks}. 
		One important family of graphs are simple undirected graphs. A simple undirected graph 
		is obtained by identifying each edge $\edgeidx \in \edges$ with two different nodes $\{\nodeidx,\nodeidx'\}$. 
		Weighted graphs also specify numeric weights $\edgeweight_{\edgeidx}$ for each 
		edge $\edgeidx \in \edges$.},first={graph},text={graph} 
}

\newglossaryentry{empgraph}
{name={federated network},
	description={A federated network\index{federated network} is an undirected weighted \gls{graph} whose 
		nodes represent data generators that aim to train a local (or personalized) \gls{model}. 
		Each node in a federated network represents some device, capable to collect a \gls{localdataset} 
		and, in turn, train a local \gls{model}. 
	    \Gls{fl} methods learn a local \gls{hypothesis} $\localhypothesis{\nodeidx}$, for 
	    each node $\nodeidx \in \nodes$, such that it incurs small \gls{loss} on the \gls{localdataset}s.},first={federated network},text={federated network} 
}

\newglossaryentry{norm}
{name={norm},
	description={A norm\index{norm} is a function that maps each element (vector) 
		of a linear vector space to a non-negative real number. This function must be 
		homogeneous, definite and satisfy the triangle inequality \cite{HornMatAnalysis}. },
	first={norm},text={norm} 
}

\newglossaryentry{explanation}
{name={explanation},
	description={One approach to make ML methods transparent, is to provide an 
		explanation\index{explanation} along with the \gls{prediction} delivered by an 
		ML method. Explanations can take on many different forms. An explanation 
		could be some natural text or some quantitative measure for the importance 
		of individual \gls{feature}s of a \gls{datapoint} \cite{Molnar2019}. We can also 
		use visual forms of explanations such as intensity plots for image classification \cite{GradCamPaper}.},
	first={explanation},text={explanation} 
}

\newglossaryentry{risk}
{name={risk},
	description={Consider\index{risk} a \gls{hypothesis} $\hypothesis$ used to predict the \gls{label} 
		$\truelabel$ of a \gls{datapoint} based on its \gls{feature}s $\featurevec$. We measure 
		the quality of a particular \gls{prediction} using a \gls{lossfunc} $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$. 
		If we interpret \gls{datapoint}s as the \gls{realization}s of \gls{iid} \gls{rv}s, 
		also the $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$ becomes the \gls{realization} 
		of a \gls{rv}. The \gls{iidasspt} allows to define the risk of a \gls{hypothesis} 
		as the expected \gls{loss} $\expect \big\{\lossfunc{(\featurevec,\truelabel)}{\hypothesis} \big\}$. 
		Note that the risk of $\hypothesis$ depends on both, the specific choice for the \gls{lossfunc} and the 
		\gls{probdist} of the \gls{datapoint}s.},
	first={risk},text={risk} 
}

\newglossaryentry{actfun}
{name={activation function},
	description={Each\index{activation function} artificial neuron within an \gls{ann} is 
		assigned an activation function $g(\cdot)$ that maps a weighted combination of 
		the neuron inputs $\feature_{1},\ldots,\feature_{\nrfeatures}$ to a single output 
		value $a = g\big(\weight_{1} \feature_{1}+\ldots+\weight_{\nrfeatures} \feature_{\nrfeatures} \big)$. 
		Note that each neuron is parametrized by the weights $\weight_{1},\ldots,\weight_{\nrfeatures}$.},
first={activation function},text={activation function} 
}




\newglossaryentry{transparency}
{name={transparency},
	description={Transparency\index{transparency} is a key requirement for 
		trustworthy AI \cite{HLEGTrustworhtyAI}. In the context of ML methods, 
		such as \gls{erm}-based methods, transparency is mainly used synonymously for \gls{explainability} \cite{gallese2023ai,JunXML2020}. 
		However, in the wide context of AI systems, transparency also includes providing information 
		about limitations and reliability of the AI system. As a point in case, \gls{logreg} provides a 
		quantitative measure for the reliability of a \gls{classification} in the form of the value $|\hypothesis(\featurevec)|$. 
		Transparency also includes the user interface, by requiring to clearly indicate when a user is 
		interaction with an AI system. Another component of transparency is the documentation 
		of the system’s purpose, design choices and intended use cases \cite{Shahriari2017,DatasheetData2021,10.1145/3287560.3287596}. },
	first={transparency},text={transparency} 
}


\newglossaryentry{sensattr}
{name={sensitive attribute},
	description={ML\index{sensitive attribute} revolves around learning a \gls{hypothesis} map that allows 
		to predict the \gls{label} of a \gls{datapoint} from its \gls{feature}s. In some 
		applications we must ensure that the output delivered by an ML system does 
		not allow to infer sensitive attributes of a \gls{datapoint}. Which parts of a \gls{datapoint} 
		is considered as a sensitive attribute is a design choice that varies across 
		different application domains.},
	first={sensitive attribute},text={sensitive attribute} 
}


\newglossaryentry{sbm}
{name={stochastic block model},
	description={The\index{stochastic block model} stochastic block model (SBM) is a 
		probabilistic generative model for an undirected graph $\graph = \big( \nodes, \edges \big)$ 
		with a given set of nodes $\nodes$ \cite{AbbeSBM2018}. In its most basic variant, 
		the SBM generates a graph by first randomly assigning each node $i \in \nodes$ to 
		a cluster index $c_{i} \in \{1,\ldots,\nrcluster\}$. A pair of different nodes in the 
		graph is connected by an edge with probability $p_{i,j}$ that depends solely on the labels $c_{i}, c_{j}$. 
		The presence of edges between different pairs of nodes is statistically independent. },
	first={stochastic block model (SBM)},text={SBM} 
}

\newglossaryentry{deepnet}
{name={deep net},
	description={We\index{deep net} refer to an \gls{ann} with a (relatively) large number of hidden layers as a 
		deep \gls{ann} or \emph{deep net}. Deep nets are used to represent the \gls{hypospace}s 
		of deep learning methods \cite{Goodfellow-et-al-2016}.},
	first={deep \gls{ann} (deep net)},text={deep net} 
}

\newglossaryentry{baseline}
{name={baseline},
	description={A\index{baseline} reference value or benchmark for the average \gls{loss} 
		incurred by a \gls{hypothesis} when applied to the \gls{datapoint}s generated in a 
		specific ML application. Such a reference value might be obtained from 
		human performance (e.g., the error rate of dermatologists diagnosing cancer 
		from visual inspection of skin areas) or other ML methods \cite[Ch. 6]{MLBasics}.}, 
	first={baseline},text={baseline} 
}


\newglossaryentry{spectrogram}
{name={spectrogram},
	description={The spectrogram\index{spectrogram} of a time signal, e.g., an audio recording, 
		characterizes the time-frequency distribution of the signal. Loosely speaking, the spectrogram 
		quantifies the signal energy within a specific period and frequency interval.}, 
	first={spectrogram},text={spectrogram} 
}

\newglossaryentry{specclustering}
{name={spectral clustering},
	description={Spectral clustering\index{spectral clustering} groups the nodes of an 
		undirected graph by applying \gls{kmeans} clustering to node-wise feature vectors. 
		These feature vectors are built from the \gls{eigenvector}s of the graph \gls{LapMat} \cite{Luxburg2007,FlowSpecClustering2021}. }, 
	first={spectral clustering},text={spectral clustering} 
}

\newglossaryentry{flowbasedclustering}
{name={flow-based clustering},
	description={Flow-basted clustering\index{flow-based clustering} groups the nodes 
		of an undirected graph by applying \gls{kmeans} clustering to node-wise feature 
		vectors. These feature vectors are built from flows between carefully selected 
		source and destination nodes \cite{FlowSpecClustering2021}. }, 
	first={flow-based clustering},text={flow-based clustering} 
}



\newglossaryentry{esterr}
{name={estimation error},
	description={Consider\index{estimation error} \gls{datapoint}s with feature vectors $\featurevec$ and \gls{label} 
		$\truelabel$. In some applications we can model the relation between the \gls{feature}s and the \gls{label}
		of a \gls{datapoint} as $\truelabel = \bar{\hypothesis}(\featurevec) + \varepsilon$. Here we 
		used some true \gls{hypothesis} $\bar{\hypothesis}$ and a noise term $\varepsilon$ which might represent 
		modelling or labelling errors. The estimation error incurred by a ML method that learns a 
		\gls{hypothesis} $\widehat{\hypothesis}$, e.g., using \gls{erm}, is defined as 
		$\widehat{\hypothesis}(\featurevec) - \bar{\hypothesis}(\featurevec)$, for some \gls{feature} vector. 
		For a parametrized \gls{hypospace}, consisting of \gls{hypothesis} maps that are determined by 
		a \gls{modelparams} $\weights$, we can define the estimation error in terms of parameter vectors 
		as $\Delta \weights = \widehat{\weights} - \overline{\weights}$ \cite{kay,hastie01statisticallearning}.}
	first={estimation error},text={estimation error} 
}


\newglossaryentry{dob}
{name={degree of belonging},
	description={A\index{degree of belonging} number that indicates the extent by which a \gls{datapoint} 
		belongs to a \gls{cluster} \cite[Ch. 8]{MLBasics}. The degree of belonging can be 
		interpreted as a soft \gls{cluster} assignment. Soft clustering methods typically represent 
		the degree of belonging by a real number in the interval $[0,1]$. The extreme case 
		when the degree of belonging only takes on values $0$ or $1$ correspond to 
		hard clustering.}, first={degree of belonging},text={degree of belonging} 
}

\newglossaryentry{msee}
{name={mean squared estimation error},
	description={Consider\index{mean squared estimation error} a ML method that 
		learns \gls{modelparams} $\widehat{\weights}$ based on some \gls{dataset} $\dataset$. 
		If we interpret the \gls{datapoint}s in $\dataset$ as \gls{iid} \gls{realization}s of a \gls{rv} $\datapoint$, 
		we define the \gls{esterr} $\Delta \weights \defeq \widehat{\weight} - \overline{\weights}$. 
		Here, $\overline{\weights}$ denotes the true \gls{modelparams} of the \gls{probdist} 
		of $\datapoint$.The mean squared estimation error is 
		defined as the \gls{expectation} $\expect \big\{ \big\| \Delta \weights \big\|^{2} \big\}$ of the 
		squared Euclidean norm of the \gls{esterr} \cite{LC,kay}.},
	first={mean squared estimation error (MSEE)},text={MSEE} 
}

\newglossaryentry{gtvmin}
{name={GTV minimization},
	description={GTV minimization\index{total variation minimization} is an instance of \gls{rerm} 
		using the \gls{gtv} of local \gls{modelparams} as a \gls{regularizer} \cite{ClusteredFLTVMinTSP}.},
	first={GTV minimization (GTVMin)},text={GTVMin} 
}

\newglossaryentry{regression}
{name={regression},
	description={Regression\index{regression} problems revolve around the problem of 
		predicting a numeric \gls{label} solely from the \gls{feature}s of a \gls{datapoint} \cite[Ch. 2]{MLBasics}.},
	first={regression},text={regression} 
}

\newglossaryentry{acc}
{name={accuracy},
	description={Consider\index{accuracy} \gls{datapoint}s characterized by \gls{feature}s $\featurevec \in \featurespace$ and 
		a categorical label $\truelabel$ which takes on values from a finite \gls{labelspace} $\labelspace$. The 
		accuracy of a \gls{hypothesis} $\hypothesis: \featurespace \rightarrow \labelspace$, when applied 
		to the \gls{datapoint}s in a \gls{dataset} $\dataset = \big\{ \big(\featurevec^{(1)}, \truelabel^{(1)} \big), \ldots, \big(\featurevec^{(\samplesize)},\truelabel^{(\samplesize)}\big) \big\}$ 
		is then defined as $1 - (1/\samplesize)\sum_{\sampleidx=1}^{\samplesize} \lossfunc{\big(\featurevec^{(\sampleidx)},\truelabel^{(\sampleidx)}\big)}{\hypothesis}$ using the \gls{zerooneloss}.},
	first={accuracy},text={accuracy} 
}



\newglossaryentry{expert}
{name={expert},
	description={ML\index{expert} aims at learning a \gls{hypothesis} $\hypothesis$ that accurately predicts the label 
		of a \gls{datapoint} based on its features. We measure the prediction error using 
		some \gls{lossfunc}. Ideally we want to find a \gls{hypothesis} that incurs minimum \gls{loss}. 
		One approach to make this goal precise is to use the \gls{iidasspt} and use the resulting 
		\gls{bayesrisk} as the benchmark level for the (average) \gls{loss} of a \gls{hypothesis}. 
		Alternatively, we might know a reference or benchmark \gls{hypothesis} $\hypothesis'$ 
		which might be obtained by some existing ML method. We can then compare the \gls{loss} 
		incurred by $\hypothesis$ against the \gls{loss} incurred by $\hypothesis'$. Such a reference 
		or baseline hypothesis $\hypothesis'$ is referred to as an \gls{expert} \cite{PredictionLearningGames}. 
		Note that an expert might deliver very poor predictions. We typically compare against many 
	   different experts and aim at incurring not much more \gls{loss} than the best among those experts (this is 
	   known as regret minimization) \cite{PredictionLearningGames,HazanOCO}.}
	first={expert},text={expert} 
}

\newglossaryentry{nfl}
{name={networked federated learning},
	description={Networked\index{networked federated learning} federated learning refers 
		to methods that learn personalized models in a distributed fashion from \gls{localdataset}s 
		that are related by an intrinsic network structure.},
 first={networked federated learning (NFL)},text={NFL} 
}




\newglossaryentry{regret}
{name={regret},
	description={The regret\index{regret} of a \gls{hypothesis} $\hypothesis$ relative to 
		another \gls{hypothesis} $\hypothesis'$, which serves as a reference (or baseline), 
		is the difference between the \gls{loss} incurred by $\hypothesis$ and the \gls{loss} 
		incurred by $\hypothesis'$ \cite{PredictionLearningGames}. 
		      The baseline \gls{hypothesis} $\hypothesis'$ is also referred to as an \gls{expert}.},
	first={regret},text={regret} 
}

\newglossaryentry{strcvx}
{name={strongly convex},
	description={A\index{strongly convex} continuously \gls{differentiable} real-valued 
		function $f(\featurevec)$ is strongly convex with coefficient $\sigma$ if $f(\vy) \geq f(\vx) + \nabla f(\vx)^{T} (\vy - \vx) + (\sigma/2) \normgeneric{\vy - \vx}{2}^{2}$ \cite{nesterov04},\cite[Sec. B.1.1.]{CvxAlgBertsekas}.},
	first={strongly convex},text={strongly convex} 
}

\newglossaryentry{differentiable}
{name={differentiable},
	description={A\index{differentiable} function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}$  is differentiable if it 
		has a \gls{gradient} $\nabla f ( \mathbf{x})$ everywhere (for every $\mathbf{x} \in \mathbb{R}^{\featuredim}$) \cite{RudinBookPrinciplesMatheAnalysis}.},
	first={differentiable},text={differentiable} 
}

\newglossaryentry{gradient}
{name={gradient},
	description={For\index{gradient} a real-valued function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}: \weights \mapsto f(\weights)$, 
	a vector $\vg$ such that $\lim_{\weights \rightarrow \weights'} \frac{f(\weights) - \big(f(\weights')+ \vg^{T} (\weights- \weights') \big) }{\| \weights-\weights'\|}=0$ 
	is referred to as the gradient of $f$ at $\weights'$. If such a vector exists it is 
	denoted $\nabla f(\weights')$ or $\nabla f(\weights)\big|_{\weights'}$ \cite{RudinBookPrinciplesMatheAnalysis}.},
	first={gradient},text={gradient} 
}

\newglossaryentry{subgradient}
{name={subgradient},
description={For\index{subgradient} a real-valued function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}: \weights \mapsto f(\weights)$, 
		a vector $\va$ such that $f(\weights) \geq  f(\weights') +\big(\weights-\weights' \big)^{T} \va$ is 
		referred to as a subgradient of $f$ at $\weights'$ \cite{BertCvxAnalOpt,BertsekasNonLinProgr}.},
	first={subgradient},text={subgradient} 
}

\newglossaryentry{fedavg}
{name={federated averaging (FedAvg)},
	description={Federated\index{federated averaging (FedAvg)} averaging is an iterative \gls{fl} algorithm that alternates between local model trainings and 
	averaging the resulting local model parameters. Different variants of this algorithm are obtained 
	by different techniques for the model training. The authors of \cite{pmlr-v54-mcmahan17a} consider 
	federated averaging methods where the local model training is implemented by running several \gls{gd} steps }, first = {federated averaging (FedAvg)}, text={FedAvg} 
}

\newglossaryentry{relu}
{name={rectified linear unit (ReLU)},
	description={The\index{rectified linear unit (ReLU)} rectified linear unit (ReLU) is 
		a popular choice for the \gls{actfun} of a neuron within an \gls{ann}. It is defined 
		as $g(z) = \max\{0,z\}$ with $z$ being the weighted input of the artificial neuron.}, first = {rectified linear unit (ReLU)}, text={ReLU} 
}

\newglossaryentry{hypothesis}
{name={hypothesis},
	description={A\index{hypothesis} map (or function) $\hypothesis: \featurespace \rightarrow \labelspace$ from the 
		\gls{featurespace} $\featurespace$ to the \gls{labelspace} $\labelspace$. 
		Given a \gls{datapoint} with \gls{feature}s $\featurevec$ we use a hypothesis map $\hypothesis$
		to estimate (or approximate) the \gls{label} $\truelabel$ using the \gls{prediction}  
		$\hat{\truelabel} = \hypothesis(\featurevec)$. ML is all about learning (or finding) a 
		hypothesis map $\hypothesis$ such that $\truelabel \approx \hypothesis(\featurevec)$ 
		for any \gls{datapoint} (having \gls{feature}s $\featurevec$ and \gls{label} $\truelabel$).},
	first={hypothesis},text={hypothesis}  
}



\newglossaryentry{vcdim}
{name={Vapnik–Chervonenkis (VC) dimension},
	description={The\index{VC dimension} VC dimension of an infinite \gls{hypospace} is a widely-used measure 
		for its size. We refer to \cite{ShalevMLBook} for a precise definition of VC dimension 
		as well as a discussion of its basic properties and use in ML.},
	first={Vapnik–Chervonenkis (VC) dimension},text={VC dimension}  
}

\newglossaryentry{effdim}
{name={effective dimension},
	description={The\index{effective dimension} effective dimension $\effdim{\hypospace}$ of 
		an infinite \gls{hypospace} $\hypospace$ is a measure of its size. Loosely speaking, the 
		effective dimension is equal to the effective number of independent tunable parameters 
		of the model. These parameters might be the coefficients used in a linear map or the 
		weights and bias terms of an \gls{ann}.},
	first={effective dimension},text={effective dimension}  
}

\newglossaryentry{labelspace}
{name={label space},
	description={Consider\index{label space} a ML application that involves \gls{datapoint}s characterized by features 
		and labels. The \gls{label} space is constituted by all potential values that the \gls{label} 
		of a \gls{datapoint} can take on. Regression methods, aiming at predicting numeric \gls{label}s, often
 use the \gls{label} space $\labelspace = \mathbb{R}$. Binary classification methods use a label space 
		 that consists of two different elements, e.g., $\labelspace =\{-1,1\}$, $\labelspace=\{0,1\}$ 
		or $\labelspace = \{ \mbox{``cat image''}, \mbox{``no cat image''} \}$  }, first={label space},text={label space}  
}

\newglossaryentry{prediction}
{name={prediction},
	description={A\index{prediction} prediction is an estimate or approximation for some 
		quantity of interest. ML revolves around learning or finding a \gls{hypothesis} map $\hypothesis$ 
		that reads in the \gls{feature}s $\featurevec$ of a \gls{datapoint} and delivers a \gls{prediction} 
		$\widehat{\truelabel} \defeq \hypothesis(\featurevec)$ for its \gls{label} $\truelabel$. },
	first={prediction},text={prediction}  
}


\newglossaryentry{histogram}
{name={histogram},
	description={Consider\index{histogram} a \gls{dataset} $\dataset$ that consists of $\samplesize$ \gls{datapoint}s 
		$\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}$, each of them belonging to some 
		cell $[-U,U] \times \ldots \times [-U,U] \subseteq \mathbb{R}^{\featuredim}$ with side 
		length $U$. We partition this cell evenly into smaller elementary cells with side 
		length $\Delta$. The histogram of $\dataset$ assigns each elementary cell to 
		the corresponding fraction of \gls{datapoint}s in $\dataset$ that fall into this 
		elementary cell. 
	},
	first={histogram},text={histogram}  
}

\newglossaryentry{bootstrap}
{name={bootstrap},
	description={For\index{bootstrap}  the analysis of ML methods it is often useful to interpret 
		a given set of \gls{datapoint}s $\dataset = \big\{ \datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}\big\}$ 
		as realizations of \gls{iid} \gls{rv}s with a common \gls{probdist} $p(\datapoint)$. In general, we 
		do not know $p(\datapoint)$ exactly, but we need to estimate it. The bootstrap uses the 
		histogram of $\dataset$ as an estimator for the underlying \gls{probdist} $p(\datapoint)$. 
	},
	first={bootstrap},text={bootstrap}  
}

\newglossaryentry{featurespace}
{name={feature space},
	description={
		The\index{feature space} \gls{feature} space of a given ML application or method is 
		constituted by all potential values that the \gls{feature} vector of a \gls{datapoint} can 
		take on. A widely used choice for the feature space is the \gls{euclidspace} $\mathbb{R}^{\featuredim}$ 
		with dimension $\featurelen$ being the number of individual \gls{feature}s of a \gls{datapoint}.},
	first={feature space},text={feature space}  
}


\newglossaryentry{missingdata}
{name={missing data},
	description={Consider\index{missing data} a \gls{dataset} constituted by \gls{datapoint}s collected via 
		some physical device. Due to imperfections and failures, some of the \gls{feature} 
		or \gls{label} values of \gls{datapoint}s might be corrupted or simply \emph{missing}. 
		Data imputation aims at estimating these missing values \cite{Abayomi2008DiagnosticsFM}. 
		We can interpret data imputation as a ML problem where the \gls{label} of a \gls{datapoint} is 
		the value of the corrupted \gls{feature}. },
	first={missing data},text={missing data}  
}


\newglossaryentry{psd}
{name={positive semi-definite},
	description={A\index{positive semi-definite} symmetric real-valued 
		matrix $\mQ = \mQ^{T} \in \mathbb{R}^{\featuredim \times \featuredim}$ is referred to as 
		positive semi-definite if $\featurevec^{T} \mQ \featurevec \geq 0$ for every 
		vector $\featurevec \in \mathbb{R}^{\featuredim}$.},
	first={positive semi-definite (psd)},text={psd}  
}

\newglossaryentry{feature}
{name={feature},
	description={A\index{feature} feature of a \gls{datapoint} is one of its properties that can be 
		measured or computed easily without the need for human supervision. For example, if a \gls{datapoint} 
		is a bitmap image, then we could use the red-green-blue intensities of its pixels as features. 
		Some widely used synonyms for the term feature are \emph{covariate}, \emph{explanatory variable}, \emph{independent variable}, 
		\emph{input (variable)}, \emph{predictor (variable)} or \emph{regressor} \cite{Gujarati2021,Dodge2003,Everitt2022}. 
		}, first={feature},text={feature}  
}

\newglossaryentry{label}
{name={label},
	description={A\index{label} higher-level fact or quantity of interest associated with a \gls{datapoint}. 
		For example, if the \gls{datapoint} is an image, the label could indicate whether the 
		image contains a cat or not. Synonyms for label, commonly used in specific domains, 
		include \emph{response variable}, \emph{output variable}, and \emph{target} \cite{Gujarati2021,Dodge2003,Everitt2022}.
 },
	first={label},text={label}  
}


\newglossaryentry{data}
{name={data},
	 description={See\index{data} \gls{dataset}.},
	text={data}
}

\newglossaryentry{dataset}
{name={dataset},
	description={With\index{dataset} a slight abuse of notation we use the term \emph{dataset} or \emph{set of \gls{datapoint}s} 
		to refer to an indexed list of \gls{datapoint}s $\datapoint^{(1)},\datapoint^{(2)},\ldots$. Thus, there 
		is a first \gls{datapoint} $\datapoint^{(1)}$, a second \gls{datapoint} $\datapoint^{(2)}$ and so on. 
		Strictly speaking, a dataset is a list and not a set \cite{HalmosSet}. The implementation of ML 
		methods requires a more detailed specification of a dataset, e.g., in the form of a relational database 
		schema \cite{silberschatz2019database}.},first={dataset},text={dataset}  
}

\newglossaryentry{predictor}
{name={predictor},
	description={A\index{predictor} predictor is a real-valued \gls{hypothesis} map. 
		Given a \gls{datapoint} with \gls{feature}s $\featurevec$, the value 
		$\hypothesis(\featurevec) \in \mathbb{R}$ is used as a \gls{prediction} for the true 
		numeric label $\truelabel \in \mathbb{R}$ of the \gls{datapoint}. },first={predictor},text={predictor}  
}

\newglossaryentry{labeled datapoint}
{name={labeled datapoint},
 description={A\index{labeled data} \gls{datapoint} whose label is known or has been determined 
 	by some means which might involve human experts.},
 first={labeled datapoint},text={labeled datapoint}  
}

\newglossaryentry{rv}
{name={random variable (RV)},
 description={A\index{random variable (RV)} random\index{probability space} 
 		variable is a mapping from a probability space $\mathcal{P}$ to a value space \cite{BillingsleyProbMeasure}. 
 	The probability space, whose elements are elementary events, is equipped with a probability 
 	 measure that assigns a probability to subsets of $\mathcal{P}$. A binary random variable maps elementary events 
 	to a set containing two different values, e.g., $\{-1,1\}$ or $\{ \mbox{cat}, \mbox{no cat} \}$. 
 	A real-valued random variable maps elementary events to real numbers $\mathbb{R}$. 
 	A vector-valued random variable maps elementary events to the \gls{euclidspace} $\mathbb{R}^{\featuredim}$. 
 	Probability theory uses the concept of measurable spaces to rigorously define and study the properties of (large) 
 	collections of random variables \cite{GrayProbBook,BillingsleyProbMeasure}.}, first={RV},text={RV}  }
 
	
\newglossaryentry{realization}
{name={realization},
	description={Consider\index{realization} a \gls{rv} $x$ which maps each element (outcome, or elementary event) $\omega \in \mathcal{P}$ of a 
		probability space $\mathcal{P}$ to an element $a$ of a measurable space $\mathcal{N}$ \cite{BillingsleyProbMeasure,RudinBookPrinciplesMatheAnalysis,HalmosMeasure}. 
		A realization of $x$ is any element $a' \in \mathcal{N}$ such that there is 
		an element $\omega' \in \mathcal{P}$ with $x(\omega') = a'$.  }, first={realization},text={realization}  }

\newglossaryentry{trainset}
{name={training set},
description={A\index{training set} \gls{dataset} $\dataset$, constituted by some \gls{datapoint}s used in \gls{erm} 
	to learn a \gls{hypothesis} $\learnthypothesis$. The average \gls{loss} of $\learnthypothesis$ on the 
	training set is referred to as the \gls{trainerr}. The comparison between \gls{trainerr} and \gls{valerr} 
	of $\learnthypothesis$ allows to diagnose ML methods and informs how to improve them (e.g., using a different \gls{hypospace} 
	or collecting more \gls{datapoint}s) \cite[Sec. 6.6.]{MLBasics}.},first={training set},text={training set}  
}

\newglossaryentry{netmodel}
{name={networked model},
  description={A\index{networked model} networked model over a \gls{empgraph} $\graph = \pair{\nodes}{\edges}$ assigns 
   a \gls{localmodel} (\gls{hypospace}) to each node $\nodeidx \in \nodes$ of the \gls{empgraph} $\graph$.}, 
   first={networked model},text={networked model}  
}

\newglossaryentry{batch}
{
	name={batch},
	description={A\index{batch} set of \gls{datapoint}s randomly selected from 
		(typically very large) \gls{dataset}.}, 
	first={batch},text={batch}  
}

\newglossaryentry{netdata}
{
	name={networked data},
	description={Networked\index{networked data} data consists of \gls{localdataset}s that are 
		related by some notion of pair-wise similarity. We can represent networked data using a \gls{empgraph} whose nodes carry \gls{localdataset}s and an edge indicates a similarity between the connected nodes.}, 
	first={networked data},text={networked data}  
}

\newglossaryentry{trainerr}
{
	name={training error},
	description={The\index{training error} average \gls{loss} of a \gls{hypothesis} when 
		predicting the \gls{label}s of \gls{datapoint}s in a \gls{trainset}. We sometimes refer 
		by training error also the minimum average \gls{loss} incurred on the \gls{trainset} 
		by the optimal \gls{hypothesis} from a \gls{hypospace}.},first={training error},text={training error}  
}

\newglossaryentry{datapoint}
{name={data point},
description={A\index{data point} \gls{datapoint} is any object that conveys information \cite{coverthomas}. Data points might be 
		students, radio signals, trees, forests, images, \gls{rv}s, real numbers or proteins. We characterize data points 
		using two types of properties. One type of property is referred to as a \gls{feature}. \Gls{feature}s are properties of a 
		\gls{datapoint} that can be measured or computed in an automated fashion. 
		A different kind of property is referred to as \gls{label}s. The \gls{label} of 
		a \gls{datapoint} represents some higher-level fact (or quantity of interest). In 
		contrast to \gls{feature}s, determining the \gls{label} of a \gls{datapoint} typically 
		requires human experts (domain experts). Roughly speaking, ML aims to predict 
		the \gls{label} of a \gls{datapoint} based solely on its \gls{feature}s. 
		}, first={data point},text={data point}  
}


\newglossaryentry{valerr}
{name={validation error},
 description={Consider\index{validation error} a \gls{hypothesis} $\learnthypothesis$ which is 
 	obtained by some ML method, e.g., using \gls{erm} on a \gls{trainset}. The average \gls{loss} 
 	of $\learnthypothesis$ on a \gls{valset}, which is different from the \gls{trainset}, is referred 
 	to as the validation error.},first={validation error},text={validation error}  
}

\newglossaryentry{validation} 
{name={validation},
	description={Consider\index{validation} a \gls{hypothesis} $\learnthypothesis$ that has been 
		learnt via some ML method, e.g., by solving \gls{erm} on a \gls{trainset} $\dataset$. 
		Validation refers to the practice of evaluating the \gls{loss} incurred by 
		\gls{hypothesis} $\learnthypothesis$ on a \gls{valset} that consists of 
		\gls{datapoint}s that are not contained in the \gls{trainset} $\dataset$. },first={validation},text={validation}  
}

\newglossaryentry{quadfunc}
{name={quadratic function},
	description={A\index{quadratic function} quadratic function $f(\weights)$, reading in a 
		vector $\weights \in \mathbb{R}^{\nrfeatures}$ as its argument, is such that $$f(\weights) =  \weights^{T} \mathbf{Q} \mathbf{w} + \mathbf{q}^{T} \weights+a,$$ with some matrix $\mQ \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$, 
		vector $\vq \in \mathbb{R}^{\nrfeatures}$ and scalar $a \in \mathbb{R}$.  },first={quadratic function},text={quadratic function}  
}

\newglossaryentry{valset}
{name={validation set},
  description={A\index{validation set} set of \gls{datapoint}s used to estimate 
  	the \gls{risk} of a \gls{hypothesis} $\learnthypothesis$ that has been learnt by some 
  	ML method (e.g., solving \gls{erm}). The average \gls{loss} of $\learnthypothesis$ 
  	on the validation set is referred to as the validation error and can be used to diagnose a 
  	ML method (see \cite[Sec. 6.6.]{MLBasics}). The comparison between \gls{trainerr} 
  	and \gls{valerr} can inform directions for improvements of the ML method (such as 
  	using a different \gls{hypospace}).},first={validation set},text={validation set}  
}

\newglossaryentry{testset}
{name={test set},
	description={A\index{test set} set of \gls{datapoint}s that have neither 
		been used to train a \gls{model}, e.g., via \gls{erm}, nor in a \gls{valset} 
		to choose between different \gls{model}s.},first={test set},text={test set}  
}


\newglossaryentry{modelsel}
{name={model selection},
	description={In\index{model selection} ML, model selection refers to the 
		process of choosing between different candidate \gls{model}s. In its most 
		basic form, \gls{model} selection amounts to (i) training each candidate \gls{model}, 
		(ii) computing the \gls{valerr} for each trained \gls{model}, (iii) choosing the \gls{model} 
		with smallest \gls{valerr} \cite[Ch. 6]{MLBasics}. },first={model selection},text={model selection}  
}





\newglossaryentry{linclass}{name={linear classifier}, description={
	    Consider\index{linear classifier} \gls{datapoint}s characterized by numeric \gls{feature}s $\featurevec \in \mathbb{R}^{\nrfeatures}$ 
	    and a \gls{label} $\truelabel \in \labelspace$ from some finite \gls{labelspace} $\labelspace$. 
		A linear \gls{classifier} characterized by having \gls{decisionregion}s separated 
		by hyperplanes in the \gls{euclidspace} $\mathbb{R}^{\featuredim}$ \cite[Ch. 2]{MLBasics}.},first={linear classifier},text={linear classifier} }

\newglossaryentry{erm}{name={empirical risk minimization}, description={Empirical risk 
		minimization\index{empirical risk minimization} is the optimization problem of finding 
		a \gls{hypothesis} (out of a \gls{model}) with minimum average \gls{loss} (or \gls{emprisk}) on a given \gls{dataset} 
		$\dataset$ (the \gls{trainset}). Many ML methods are obtained from 
		\gls{emprisk} via specific design choices for the \gls{dataset}, \gls{model} and \gls{loss} \cite[Ch. 3]{MLBasics}.},
	first={empirical risk minimization (ERM)},text={ERM} }

\newglossaryentry{multilabelclass}{name={multi-label classification}, description={Multi-label 
		classification\index{multi-label classification} problems and methods use \gls{datapoint}s 
		that are characterized by several \gls{label}s. As an example, consider a \gls{datapoint} 
		representing a picture with one binary \gls{label} indicating the presence of a human 
		in this picture and another \gls{label} indicating the presence of a car.},
	    first={multi-label classification},text={multi-label classification} }


\newglossaryentry{ssl}{name={semi-supervised learning}, description={Semi-supervised\index{semi-supervised learning} 
		learning methods use unlabeled \gls{datapoint}s to support the learning of a \gls{hypothesis} 
		from labeled \gls{datapoint}s \cite{SemiSupervisedBook}. This approach is particularly useful 
		for ML applications that offer a large amount of unlabeled \gls{datapoint}s, but only a limited 
		number of  labeled \gls{datapoint}s.}, 
		first={semi-supervised learning (SSL)},text={SSL} }
	
	
\newglossaryentry{objfunc}{name={objective function}, description={An\index{objective function} 
		objective function is a map that assigns each value of an optimization variable, such 
		as the \gls{modelparams} $\weights$ of a \gls{hypothesis} $\hypothesis^{(\weights)}$, to 
		an objective value $f(\weights)$. The objective value $f(\weights)$ could be the 
		\gls{risk} or the \gls{emprisk} of a \gls{hypothesis} $\hypothesis^{(\weights)}$.},first={objective function},text={objective function} }
	
\newglossaryentry{regularizer}{name={regularizer}, description={A regularizer\index{regularizer} 
		assigns each \gls{hypothesis} $\hypothesis$ from a \gls{hypospace} $\hypospace$ a quantitative 
		measure $\regularizer{\hypothesis}$ for how much its prediction error on a \gls{trainset} might 
		differ from its prediction errors on \gls{datapoint}s outside the \gls{trainset}. \Gls{ridgeregression} 
		uses the regularizer $\regularizer{\hypothesis} \defeq \normgeneric{\weights}{2}^{2}$ for linear \gls{hypothesis} maps $\hypothesis^{(\weights)}(\featurevec) \defeq \weights^{T} \featurevec$ \cite[Ch. 3]{MLBasics}. 
		The \gls{lasso} uses the regularizer $\regularizer{\hypothesis} \defeq \normgeneric{\weights}{1}$ 
		for linear \gls{hypothesis} maps $\hypothesis^{(\weights)}(\featurevec) \defeq \weights^{T} \featurevec$ \cite[Ch. 3]{MLBasics}. },first={regularizer},text={regularizer} }


\newglossaryentry{regularization}{name={regularization}, description={Regularization\index{regularization} 
		techniques modify \gls{erm} such that the learnt \gls{hypothesis} performs well (generalizes) 
		also outside the \gls{trainset}. One specific implementation of \gls{regularization} is to add a penalty 
		or regularization term to the objective function of \gls{erm} (which is the average \gls{loss} on the \gls{trainset}). This regularization 
		term can be interpreted as an estimate for the increase in the expected \gls{loss} (\gls{risk}) compared to the 
		average \gls{loss} on the \gls{trainset}. },first={regularization},text={regularization} }

\newglossaryentry{rerm}{name={regularized empirical risk minimization}, 
	description={Synonym\index{regularized empirical risk minimization} for \gls{srm}.},
	first={regularized empirical risk minimization (RERM)},text={RERM} }
	
\newglossaryentry{gtv}{name={generalized total variation}, description={Generalized\index{generalized total variation} 
		total variation measures the changes of vector-valued node attributes over a 
		weighted undirected \gls{graph}.},first={generalized total variation (GTV)},text={GTV} }
	
\newglossaryentry{srm}{name={structural risk minimization}, description={Structural\index{structural risk minimization} 
		risk minimization is the problem of finding the \gls{hypothesis} that optimally 
		balances the average \gls{loss} (or \gls{emprisk}) on a \gls{trainset} with a 
		\gls{regularization} term. The \gls{regularization} term penalizes a \gls{hypothesis}
		that is not robust against (small) perturbations of the \gls{datapoint}s in the \gls{trainset}.},first={structural risk minimization (SRM)},text={SRM} }

\newglossaryentry{datapoisoning}{name={data poisoning}, description={Data\index{data poisoning} 
		poisoning refers to the intentional manipulation (or fabrication) of \gls{datapoint}s to 
		steer the training of a ML model \cite{Liu2021,PoisonGAN}. The protection against 
		data poisoning is particularly important in distributed ML applications where \gls{dataset}s are de-centralized.},first={data poisoning},text={data poisoning} }
	
	
\newglossaryentry{backdoor}{name={backdoor}, description={A\index{backdoor} backdoor attack refers 
		to the intentional manipulation of the training process underlying a ML method. This manipulation 
		can be implemented by perturbing the \gls{trainset} (data poisoning) or the 
		optimization algorithm used by an \gls{erm}-based method. The goal of a 
		backdoor attack is to nudge the learnt \gls{hypothesis} $\learnthypothesis$ 
		towards specific \gls{prediction}s for a certain range of \gls{feature} values. This range of \gls{feature} 
		values serves as a key (or trigger) to unlock a \emph{backdoor} in the sense of 
		delivering anomalous \gls{prediction}s. The key $\featurevec$ and the corresponding 
		anomolous \gls{prediction} $\learnthypothesis(\featurevec)$ are only known to the attacker.},
	first={backdoor},text={backdoor} }


\newglossaryentry{clustasspt}{name={clustering assumption}, description={The\index{clustering assumption} 
		clustering assumption postulates that \gls{datapoint}s in a \gls{dataset} form a (small) number of 
		groups or clusters. \Gls{datapoint}s in the same \gls{cluster} are more similar with each 
		other than with those outside the cluster \cite{SemiSupervisedBook}. We obtain different 
		clustering methods by using different notions of similarity between \gls{datapoint}s.},first={clustering assumption},text={clustering assumption} }
	
\newglossaryentry{dosattack}{name={denial-of-service attack}, description={A\index{denial-of-service attack} 
		denial-of-service attack aims (e.g., via \gls{datapoisoning}) to steer the training of a \gls{model} 
		such that it performs poorly for typical \gls{datapoint}s},
	first={denial-of-service attack},text={denial-of-service attack} }

\newglossaryentry{netexpfam}{name={networked exponential families}, 
	description={A\index{networked exponential families} collection of exponential 
		families, each of them assigned to a node of a \gls{empgraph}. The \gls{modelparams} are coupled 
	   via the network structure by requiring them to have a small \gls{gtv} \cite{JungNetExp2020}. },first={networked exponential family (nExpFam)},text={nExpFam} }
	 


\newglossaryentry{scatterplot}{name={scatterplot}, description={A\index{scatterplot} 
		visualization technique that depicts data points by markers in a two-dimensional plane. 
		\begin{figure}[htbp]
			\begin{center}
				\begin{tikzpicture}[scale=0.9]
					\tikzset{x=1cm,y=1cm,every path/.style={>=latex},node style/.style={circle,draw}}
					\begin{axis}[axis x line=none,
						axis y line=none,
						ylabel near ticks,
						xlabel near ticks,
						enlarge y limits=true,
						xmin=-5, xmax=30,
						ymin=-5, ymax=30,
						width=5cm, height=5cm ]
						\addplot[only marks] table [x=mintmp, y=maxtmp, col sep = semicolon] {FMIData1.csv};
						\node at (axis cs:26,2) [anchor=west] {$\feature$};
						\node at (axis cs:0,30) [anchor=west] {$\truelabel$};
						\draw[->] (axis cs:-5,0) -- (axis cs:30,0);
						\draw[->] (axis cs:0,-5) -- (axis cs:0,30);
					\end{axis}
				\end{tikzpicture}
				\vspace*{-14mm}
			\end{center}
			\caption{A scatterplot of \gls{datapoint}s that represent daily weather conditions in Finland. 
				Each \gls{datapoint} is characterized by its minimum daytime temperature $\feature$ 
				as \gls{feature} and its maximum daytime temperature $\truelabel$ as the \gls{label}. 
				The temperatures have been measured at the \gls{fmi} weather station \emph{Helsinki Kaisaniemi} 
				during 1.9.2024 - 28.10.2024.}
			\label{fig_scatterplot_temp_FMI}
			\vspace*{-3mm}
			\end{figure}
		},first={scatterplot},text={scatterplot} }


\newglossaryentry{stepsize}{name={step size}, description={
		See\index{step size} \gls{learnrate}. 
%		Many ML methods use iterative optimization methods (such as \gls{gdmethods}) 
%		to construct a sequence of increasingly accurate hypothesis 
%		maps $h^{(1)},h^{(2)},\ldots$. The $\itercntr$th iteration of such an algorithm starts from the current 
%		hypothesis $h^{(\itercntr)}$ and tries to modify it to obtain an improved hypothesis $h^{(\itercntr+1)}$. 
%		Iterative algorithms often use a step size (hyper-) parameter. The step size controls the amount by 
%		which a single iteration can change or modify the current hypothesis. Since the overall goal of such 
%		iteration ML methods is to learn a (approximately) optimal hypothesis we refer to a step size parameter 
%		also as a \gls{learnrate}.
}, 
	first={step size},text={step size} }

\newglossaryentry{learnrate}{name={learning rate}, description={Consider\index{learning rate} 
		an iterative method for finding or learning a useful \gls{hypothesis} $\hypothesis \in \hypospace$. 
		Such an iterative method repeats similar computational (update) steps that adjust or 
		modify the current \gls{hypothesis} to obtain an improved \gls{hypothesis}. A prime example of 
		such an iterative learning method is \gls{gd} and its variants such as \gls{stochGD} or \gls{projgd}. 
		We refer by learning rate to a parameter of an iterative learning 
		method that controls the extent by which the current \gls{hypothesis} 
		can be modified during a single iteration. A prime example of such a parameter is the 
				step size used in \gls{gd} \cite[Ch. 5]{MLBasics}.},
	first={learning rate},text={learning rate} }

\newglossaryentry{featuremap}{name={feature map}, description={A\index{feature map} map that transforms the original  
		 \gls{feature}s of a \gls{datapoint} into new \gls{feature}s. The so-obtained new \gls{feature}s might 
		 be preferable over the original features for several reasons. For example, the shape of datasets might 
		 become simpler in the new feature space, allowing to use linear models in the new \gls{feature}s. 
		 Another reason could be that the number of new \gls{feature}s is much smaller which is preferable 
		 in terms of avoiding \gls{overfitting}. The special case of a \gls{feature} map delivering 
		 two numeric \gls{feature}s is particularly useful for data visualization. Indeed, we can depict 
		 \gls{datapoint}s in a \gls{scatterplot} by using two \gls{feature}s as the coordinates of a \gls{datapoint}.},
	first={feature map},text={feature map} }
 
  \newglossaryentry{lasso}{name={least absolute shrinkage and selection operator (Lasso)}, 
	description={The\index{Lasso} least absolute shrinkage and selection operator (Lasso) is an 
		instance of \gls{srm} to learn the weights $\weights$ of a linear map 
		$\hypothesis(\featurevec) = \weights^{T} \featurevec$ based on a \gls{trainset}. 
		The Lasso is obtained from \gls{linreg} by adding the scaled $\ell_{1}$-norm 
		$\regparam \normgeneric{\weights}{1}$ to the average \gls{sqerrloss} incurred on the \gls{trainset}. 
	},
	first={ least absolute shrinkage and selection operator (Lasso)},text={Lasso} }
 
 \newglossaryentry{simgraph}{name={similarity graph}, 
 	description={Some\index{similarity graph} ML applications generate \gls{datapoint}s that 
 		are related by a domain-specific notion of similarity. These similarities can be 
 		represented conveniently using a similarity \gls{graph} $\graph = \big(\nodes \defeq \{1,\ldots,\samplesize\},\edges\big)$. 
 		The node $\sampleidx \in \nodes$ represents the $\sampleidx$-th \gls{datapoint}. Two 
 		nodes are connected by an undirected edge if the corresponding \gls{datapoint}s are similar. 
 	},
 	first={similarity graph},text={similarity graph} }
 
 
 \newglossaryentry{kld}{name={Kullback-Leibler divergence}, 
 	description={
 		 The\index{KL divergence} Kullback–Leibler divergence is a quantitative 
 		 measure for how much one \gls{probdist} is different from another \gls{probdist} \cite{coverthomas}.  
 	},
 	first={Kullback-Leibler divergence},text={KL divergence} }

\newglossaryentry{LapMat}{name={Laplacian matrix}, 
	description={
		The\index{Laplacian matrix} geometry or structure of a graph $\graph$ can be 
		analyzed using the properties of special matrices that are associated with $\graph$. 
		One such matrix is the graph Laplacian matrix $\mL$ which is defined for an 
		undirected and weighted \gls{graph} \cite{Luxburg2007,Ng2001}. One important 
		example of such a \gls{graph} is the \gls{empgraph} in a \gls{fl} application. 
	},
	first={Laplacian matrix},text={Laplacian matrix} }


\newglossaryentry{kernel}{name={kernel}, 
	description={Consider\index{kernel} \gls{datapoint}s characterized by a \gls{feature} vector $\featurevec \in \featurespace$ 
	with a generic \gls{featurespace} $\featurespace$. A kernel is a map that assigns each pair of \gls{feature} vectors  
	$\featurevec, \featurevec' \in \featurespace$ a real number. This number measures the similarity between 
	$\featurevec$ and $\featurevec'$. For more details about kernels and the resulting kernel methods, 
	we refer to the literature \cite{LampertNowKernel,LearningKernelsBook}.},
	first={kernel},text={kernel} }

\newglossaryentry{cm}{name={confusion matrix}, 
	description={Consider\index{confusion matrix} \gls{datapoint}s characterized by \gls{feature}s $\featurevec$ 
		and \gls{label} $\truelabel$ having values from the finite \gls{labelspace} $\labelspace = \{1,\ldots,\nrcluster\}$. 
		The confusion matrix is $\nrcluster \times \nrcluster$ matrix with rows representing different values $\clusteridx$ 
		of the true label of a \gls{datapoint}. The columns of a confusion matrix correspond to different values 
		$\clusteridx'$ delivered by a hypothesis $\hypothesis(\featurevec)$. The $(\clusteridx,\clusteridx')$-th entry of 
		the confusion matrix is the fraction of \gls{datapoint}s with \gls{label} $\truelabel\!=\! \clusteridx$ and the 
		\gls{prediction} $\hat{\truelabel}\!=\!\clusteridx'$ assigned by the \gls{hypothesis} $\hypothesis$.},
	first={confusion matrix},text={confusion matrix} }


\newglossaryentry{featurematrix}{name={feature matrix}, 
	description={Consider\index{feature matrix} a \gls{dataset} $\dataset$ with $\samplesize$ \gls{datapoint}s, each of them 
		characterized by the \gls{feature}s $\featurevec^{(\sampleidx)}$, $\sampleidx=1,\ldots,\samplesize$. 
		The feature matrix $\featuremtx$ of $\dataset$ is constructed by stacking, column-wise, 
	the \gls{feature}s of the \gls{datapoint}s into a matrix $\featuremtx = \big( \featurevec^{(1)},\ldots, \featurevec^{(\samplesize)} \big)$ 
	of size $\samplesize \times \nrfeatures$.} 
	first={feature matrix},text={feature matrix} }


\newglossaryentry{dbscan}{name={density-based spatial clustering of applications with noise}, 
	description={A\index{DBSCAN} clustering algorithm for \gls{datapoint}s that are characterized by numeric feature vectors. 
		Like \gls{kmeans} and \gls{softclustering} via \gls{gmm}, also DBSCAN uses the Euclidean 
		distances between \gls{feature} vectors to determine the \gls{cluster}s. However, in contrast to \gls{kmeans} 
		and \gls{gmm}, DBSCAN uses a different notion of similarity between \gls{datapoint}s. 
		DBSCAN considers two \gls{datapoint}s as similar if they are \emph{connected} 
		via a sequence (path) of close-by intermediate \gls{datapoint}s. Thus, DBSCAN might consider 
		two \gls{datapoint}s as similar (and therefore belonging to the same cluster) even if 
		their \gls{feature} vectors have a large Euclidean distance.},
	first={density-based spatial clustering of applications with noise (DBSCAN)},text={DBSCAN} }

\newglossaryentry{fl}{name={federated learning (FL)}, description={Federated\index{federated learning} 
		learning is an umbrella term for ML methods that train models in a collaborative 
		fashion using decentralized data and computation.},first={federated learning (FL)},text={FL} }
	
\newglossaryentry{cfl}{name={clustered federated learning (CFL)}, description={
		Clustered\index{clustered federated learning} \gls{fl} (CFL) assumes that \gls{localdataset}s form clusters. 
		The \gls{localdataset}s belonging to the same cluster have similar statistical properties. 
		CFL pools \gls{localdataset}s in the same cluster to obtain a \gls{trainset} 
		for training a cluster-specific \gls{model}. \Gls{gtvmin} implements this pooling implicitly 
		by forcing the local \gls{modelparams} to be approximately identical over well-connected 
		subsets of the \gls{empgraph}.},
	first={clustered \gls{fl}},text={CFL} }

\newglossaryentry{iid}{name={i.i.d.}, description={It\index{i.i.d.} can be useful to 
		interpret \gls{datapoint}s $\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}$ 
		as \gls{realization}s of independent and identically distributed \gls{rv}s with 
		a common \gls{probdist}. If these \gls{rv}s are continuous-valued, their joint \gls{pdf} is $p\big(\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)} \big) = \prod_{\sampleidx=1}^{\samplesize} p \big(\datapoint^{(\sampleidx)}\big)$ with $p(\datapoint)$ being the common 
		marginal \gls{pdf} of the underlying \gls{rv}s.},
	first={independent and identically distributed (i.i.d.)},text={{i.i.d.}} }


\newglossaryentry{outlier}{name={outlier}, description={Many\index{outlier} ML methods 
		are motivated by the \gls{iidasspt} which interprets \gls{datapoint}s as realizations of 
		\gls{iid} \gls{rv}s with a common \gls{probdist}. The \gls{iidasspt} is useful for applications  
		where the statistical properties of the data generation process are stationary (or time-invariant) \cite{Brockwell91}. 
		However, in some applications the data consists of a majority of \emph{regular} \gls{datapoint}s 
		that conform with an \gls{iidasspt} and a small number of data points that have fundamentally different 
        statistical properties compared to the regular \gls{datapoint}s. We refer to a \gls{datapoint} that 
        substantially deviates from the statistical properties of most \gls{datapoint}s as an 
        outlier. Different methods for outlier detection use different measures for this deviation. 
        Stastistical learning theory studies fundamental limits on the ability to mitigate outliers reliably \cite{doi:10.1137/0222052,10.1214/20-AOS1961}.},
	          first={outlier},text={outlier} }

\newglossaryentry{decisionregion}{name={decision region}, description={Consider\index{decision region} 
		a \gls{hypothesis} map $\hypothesis$ that delivers values from a finite set $\labelspace$. 
		We refer to the set of \gls{feature}s $\featurevec \in \featurespace$ that result 
		in the same output $\hypothesis(\featurevec)=a$ as a decision region of 
		the \gls{hypothesis} $\hypothesis$. },first={decision region},text={decision region} }

\newglossaryentry{decisionboundary}{name={decision region}, description={Consider\index{decision boundary} a 
		\gls{hypothesis} map $\hypothesis$ that reads in a \gls{feature} vector 
		$\featurevec \in \mathbb{R}^{\featuredim}$ and delivers a value from a finite set $\labelspace$. 
		The decision boundary of $\hypothesis$ is the set of vectors $\featurevec \in \mathbb{R}^{\featuredim}$ 
		that lie between different \gls{decisionregion}s. More precisely, a 
		vector $\featurevec$ belongs to the decision boundary if and only 
		if each neighbourhood $\{ \featurevec': \| \featurevec - \featurevec' \| \leq \varepsilon \}$, 
		for any $\varepsilon >0$, contains at least two vectors with different function values.},first={decision boundary},text={decision boundary} }


\newglossaryentry{euclidspace}{name={Euclidean space}, description={The\index{Euclidean space} 
		Euclidean space $\mathbb{R}^{\featuredim}$ of dimension $\featuredim \in \mathbb{N}$ consists 
		of vectors $\featurevec= \big(\feature_{1},\ldots,\feature_{\featurelen}\big)$, with $\featuredim$ 
		real-valued entries $\feature_{1},\ldots,\feature_{\featuredim} \in \mathbb{R}$. Such an Euclidean 
		space is equipped with a geometric structure defined by the inner product 
		$\featurevec^{T} \featurevec' = \sum_{\featureidx=1}^{\featuredim} \feature_{\featureidx} \feature'_{\featureidx}$ 
		between any two vectors $\featurevec,\featurevec' \in \mathbb{R}^{\featuredim}$ \cite{RudinBookPrinciplesMatheAnalysis}.},first={Euclidean space},text={Euclidean space} }

\newglossaryentry{eerm}{name={explainable empirical risk minimization}, description={An\index{explainable empirical risk minimization} 
		instance of structural risk minimization that adds a \gls{regularization} term to the 
		average \gls{loss} in the objective function of \gls{erm}. 
		The \gls{regularization} term is chosen to favour \gls{hypothesis} maps that are intrinsically 
		explainable for a specific user. This user is characterized by their \gls{prediction}s provided 
		for the \gls{datapoint}s in a \gls{trainset} \cite{Zhang:2024aa}.},first={explainable empirical risk minimization (EERM)},text={EERM} }
	
	
\newglossaryentry{kmeans}{name={$k$-means}, description={The\index{$k$-means} $k$-means algorithm 
		is a hard \gls{clustering} method which assigns each \gls{datapoint} of a \gls{dataset} 
		to precisely one of $k$ different \gls{cluster}s. The method alternates between updating 
		the \gls{cluster} assignments (to the cluster with nearest cluster mean) and, given the updated \gls{cluster} assignments, 
		re-calculating the cluster means \cite[Ch. 8]{MLBasics}.},first={$k$-means},text={$k$-means} }


\newglossaryentry{xml}{name={explainable ML}, description={Explainable\index{explainable AI} 
		ML methods aim at complementing each \gls{prediction} with an \gls{explanation} for how the \gls{prediction} 
		has been obtained. The construction of an explicit \gls{explanation} might not be necessary 
		if the ML method uses a sufficiently simple (or interpretable) \gls{model} \cite{rudin2019stop}.},first={explainable ML},text={explainable ML} }

\newglossaryentry{fmi}{name={Finnish Meteorological Institute}, description={The\index{Finnish Meteorological Institute}
		Finnish Meteorological Institute is a government agency responsible for gathering 
		and reporting weather data in Finland.},first={Finnish Meteorological Institute (FMI)},text={FMI} }
	
\newglossaryentry{samplemean}{name={sample mean}, description={The\index{sample mean} sample mean 
			$\vm \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$ for a given set of \gls{feature} 
			vectors $\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)} \in \mathbb{R}^{\nrfeatures}$ 
			is defined as 
			$$\vm = (1/\samplesize) \sum_{\sampleidx=1}^{\samplesize} \featurevec^{(\sampleidx)}.$$ 
		},
		first={sample mean},text={sample mean} }
	
\newglossaryentry{samplecovmtx}{name={sample covariance matrix}, description={The\index{sample covariance matrix} 
		sample covariance matrix $\widehat{\bf \Sigma} \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$ 
		for a given set of \gls{feature} vectors $\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)} \in \mathbb{R}^{\nrfeatures}$ is defined as 
		$$\widehat{\bf \Sigma} = (1/\samplesize) \sum_{\sampleidx=1}^{\samplesize} (\featurevec^{(\sampleidx)}\!-\!\widehat{\vm}) (\featurevec^{(\sampleidx)}\!-\!\widehat{\vm})^{T}.$$ 
		Here, we used the \gls{samplemean} $\widehat{\vm}$. 
	},
	first={sample covariance matrix},text={sample covariance matrix} }

\newglossaryentry{covmtx}{name={covariance matrix}, description={The\index{covariance matrix} covariance matrix of 
		a \gls{rv} $\vx \in \mathbb{R}^{\featuredim}$ is defined as $\expect \bigg \{ \big( \vx - \expect \big\{ \vx \big\} \big)  \big(\vx - \expect \big\{ \vx \big\} \big)^{T} \bigg\}$.},
	first={covariance matrix},text={covariance matrix} }
	
\newglossaryentry{highdimregime}{name={high-dimensional regime}, description={The\index{high-dimensional regime} 
		high-dimensional regime of \gls{erm} is characterized by the \gls{effdim} of the \gls{model} 
		being larger than the \gls{samplesize}, i.e., the number of (labeled) \gls{datapoint}s in the \gls{trainset}. 
		For example, \gls{linreg} methods operate in the high-dimensional regime whenever the number $\featuredim$ of \gls{feature}s 
		used to characterize \gls{datapoint}s exceeds the number of \gls{datapoint}s in the \gls{trainset}. 
		Another example of ML methods that operate in the high-dimensional regime are large \gls{ann}s, having 
		far more tunable weights (and bias terms) than the number of \gls{datapoint}s in the \gls{trainset}. 
		High-dimensional statistics is a recent main thread of probability theory that studies the 
		behavior of ML methods in the high-dimensional regime \cite{Wain2019,BuhlGeerBook}.},
   first={high-dimensional regime},text={high-dimensional regime} }

\newglossaryentry{gmm}{name={Gaussian mixture model}, description={Gaussian\index{Gaussian mixture model} mixture models (GMM) are a family of 
		\gls{probmodel}s for \gls{datapoint}s characterized by a numeric \gls{feature} vector $\featurevec$. A GMM interprets 
	     $\featurevec$ as being drawn from one of $\nrcluster$ different \gls{mvndist}s $p^{(\clusteridx)} = \mvnormal{\meanvec{\clusteridx}}{\covmtx{\clusteridx}}$, indexed by $\clusteridx=1,\ldots,\nrcluster$. 
	     The probability that $\featurevec$ is drawn from the $\clusteridx$-th \gls{mvndist} is 
	     denoted $p_{\clusteridx}$. Thus, a GMM is parametrized by the probability $p_{\clusteridx}$, the 
		mean vector $\clustermean^{(\clusteridx)}$ and \gls{covmtx} $\clustercov^{(\clusteridx)}$ for each $\clusteridx=1,\ldots,\nrcluster$. 
	 },first={Gaussian mixture model (GMM)},text={GMM} }
 
\newglossaryentry{ml}{name={maximum likelihood}, description={
		Consider\index{maximum likelihood} \gls{datapoint}s $\dataset=\big\{ \datapoint^{(1)}, \ldots, \datapoint^{(\samplesize)} \}$ that are interpreted 
		as realizations of \gls{iid} \gls{rv}s with a common \gls{probdist} $\prob{\datapoint; \weights}$ which 
		depends on a parameter vector $\weights \in \mathcal{W} \subseteq \mathbb{R}^{n}$. Maximum likelihood methods aim at finding a parameter vector $\weights$ 
		such that the probability (density) $\prob{\dataset; \weights} = \prod_{\sampleidx=1}^{\samplesize} \prob{\datapoint^{(\sampleidx)}; \weights}$ 
		of observing the data is maximized. Thus, the maximum 
		likelihood estimator is obtained as a solution to the optimization 
		problem $\max_{\weights \in \mathcal{W}} \prob{\dataset; \weights}$.
	},first={maximum likelihood},text={maximum likelihood}}



\newglossaryentry{em}{name={expectation maximization}, description={Expectation\index{expectation maximization} 
		maximization is a generic technique for estimating the \gls{modelparams} of a \gls{probmodel} $\prob{\datapoint; \weights}$ 
		from data \cite{BishopBook,hastie01statisticallearning,GraphModExpFamVarInfWainJor}. Expectation maximization 
		delivers an approximation to the \gls{ml} estimate for the model parameters $\weights$. 
  },first={expectation maximization (EM)},text={EM}}

\newglossaryentry{ppca}{name={probabilistic PCA}, description={Probabilistic\index{probabilistic PCA} \gls{pca} (PPCA) 
		extends basic \gls{pca} by using a \gls{probmodel} for \gls{datapoint}s. The \gls{probmodel} of PPCA 
		reduces the task of dimensionality reduction to an estimation problem that can be solved using \gls{em} 
		methods.},first={probabilistic PCA (PPCA)},text={PPCA}}
	
\newglossaryentry{polyreg}{name={polynomial regression}, description={Polynomial\index{polynomial regression} 
		regression aims at learning a polynomial \gls{hypothesis} map to predict a numeric \gls{label} based
		 on numeric \gls{feature}s of a \gls{datapoint}. For \gls{datapoint}s characterized by a single 
		 numeric \gls{feature}, polynomial regression uses the \gls{hypospace} 
			$\hypospace^{(\rm poly)}_{\nrfeatures} \defeq \{ \hypothesis(x) = \sum_{\featureidx=0}^{\nrfeatures-1} x^{\featureidx} \weight_{\featureidx} \}.$
			The quality of a polynomial \gls{hypothesis} map is measured using the average \gls{sqerrloss} 
			incurred on a set of labeled \gls{datapoint}s (which we refer to as \gls{trainset}).},first={polynomial regression},text={polynomial regression}}

\newglossaryentry{linreg}{name={linear regression}, description={Linear\index{linear regression} 
		regression aims to learn a linear \gls{hypothesis} map to predict a numeric \gls{label} based 
		on numeric \gls{feature}s of a \gls{datapoint}. The quality of a linear \gls{hypothesis} map is 
		measured using the average \gls{sqerrloss} incurred on a set of labeled \gls{datapoint}s, 
		which we refer to as the \gls{trainset}.},first={linear regression},text={linear regression}}
        
\newglossaryentry{ridgeregression}{name={ridge regression}, description={Ridge\index{ridge regression} 
		regression learns the \gls{weights} $\weights$ of a linear \gls{hypothesis} map $\hypothesis^{(\weights)}(\featurevec)= \weights^{T} \featurevec$. 
		The quality of a particular choice for the parameter vector $\weights$ is measured by the sum 
		of two components. The first component is the average \gls{sqerrloss} incurred by $\hypothesis^{(\weights)}$ on a set of 
		labeled \gls{datapoint}s (the \gls{trainset}). The second component is the scaled squared 
		Euclidean norm $\regparam \| \weights \|^{2}_{2}$ with a \gls{regularization} parameter 
		$\regparam > 0$. It can be shown that the effect of adding to $\regparam \| \weights \|^{2}_{2}$ to 
	the average \gls{sqerrloss} is equivalent to replacing the original \gls{datapoint}s by an ensemble of 
realizations of a \gls{rv} centered around these \gls{datapoint}s.},first={ridge regression},text={ridge regression}}


\newglossaryentry{expectation}{name={expectation}, description={
		Consider\index{expectation} a numeric \gls{feature} vector $\featurevec \in \mathbb{R}^{\featuredim}$ 
		which we interpret as the \gls{realization} of a \gls{rv} with \gls{probdist} $p(\featurevec)$. 
		The expectation of $\featurevec$ is defined as the integral $\expect \{ \featurevec \} \defeq \int \featurevec p(\featurevec)$ \cite{HalmosMeasure,BillingsleyProbMeasure,RudinBookPrinciplesMatheAnalysis}. Note that 
		the expectation is only defined if this integral exists, i.e., if the \gls{rv} is integrable.},first={expectation},text={expectation}}

\newglossaryentry{logreg}{name={logistic regression}, description={Logistic\index{logistic regression} regression learns a 
		linear \gls{hypothesis} map (\gls{classifier}) $\hypothesis(\featurevec) = \weights^{T} \featurevec$ 
		to predict a binary \gls{label} $\truelabel$ based on numeric \gls{feature} vector 
		$\featurevec$ of a \gls{datapoint}. The quality of a linear \gls{hypothesis} map is 
		measured by the average \gls{logloss} on some labeled \gls{datapoint}s (the \gls{trainset}).},
		first={logistic regression},text={logistic regression}}
	
\newglossaryentry{logloss}{name={logistic loss}, description={Consider\index{logistic loss} 
		a \gls{datapoint}, characterized by the \gls{feature}s $\featurevec$ and a binary \gls{label} $\truelabel \in \{-1,1\}$. 
		We use a real-valued \gls{hypothesis} $\hypothesis$ to predict the label $\truelabel$ 
		from the features $\featurevec$. The logistic loss incurred by this \gls{prediction} is 
		defined as 
	\begin{equation} 
		\label{equ_log_loss_gls}
		\lossfunc{(\featurevec,\truelabel)}{\hypothesis} \defeq  \log ( 1 + \exp(- \truelabel \hypothesis(\featurevec))).
\end{equation}
Carefully note that the expression \eqref{equ_log_loss_gls} 
for the logistic loss applies only if for the \gls{labelspace} $\labelspace = \{ -1,1\}$ and using 
the thresholding rule \eqref{equ_def_threshold_bin_classifier}. },first={logistic loss},text={logistic loss}}
	
\newglossaryentry{hingeloss}{name={hinge loss}, description={Consider\index{hinge loss} a \gls{datapoint}, 
		characterized by a \gls{feature} vector $\featurevec \in \mathbb{R}^{\featuredim}$ and a 
		binary \gls{label} $\truelabel \in \{-1,1\}$. The hinge loss incurred by a real-valued 
		\gls{hypothesis} map $\hypothesis(\featurevec)$ is defined as 
		\begin{equation} 
			\label{equ_hinge_loss_gls}
				\lossfunc{(\featurevec,\truelabel)}{\hypothesis} \defeq \max \{ 0 , 1 - \truelabel \hypothesis(\featurevec) \}. 
			\end{equation}
	    A regularized variant of the hinge loss is used by the \gls{svm} \cite{LampertNowKernel} to learn 
	    a \gls{linclass} with maximum margin between the two classes (see Figure \ref{fig_svm_gls}). 
		\begin{figure}[htbp]
			\begin{center}
				\begin{tikzpicture}[auto,scale=0.8]
					%\draw [thick] (0,-3) rectangle (4,4) node [anchor=east,above] {$\featurespace$} ;
					\draw [thick] (1,2) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(5)}$};
					\draw [thick] (0,1.6) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(4)}$};
					\draw [thick] (0,3) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(3)}$};
					\draw [thick] (2,1) circle (0.1cm)node[anchor=east,above] {\hspace*{0mm}$\featurevec^{(6)}$};
					\node[] (B) at (-2,0) {\emph{support vector}};
					\draw[->,dashed] (B) to (1.9,1) ; 
					\draw [|<->|,thick] (2.05,0.95)  -- (2.75,0.25)node[pos=0.5] {$\xi$} ; 
					\draw [thick] (1,-1.5) -- (4,1.5) node [right] {$\hypothesis^{(\weights)}$} ; 
					\draw [thick] (3,-1.9) rectangle ++(0.1cm,0.1cm) node[anchor=west,above]  {\hspace*{0mm}$\featurevec^{(2)}$};
					\draw [thick] (4,.-1) rectangle ++(0.1cm,0.1cm) node[anchor=west,above] {\hspace*{0mm}$\featurevec^{(1)}$};
				\end{tikzpicture}
				\caption{The \gls{svm} learns a hypothesis (or classifier) $\hypothesis^{(\weights)}$ with 
					minimum average soft-margin \gls{hingeloss}. Minimizing this \gls{loss} is equivalent 
					to maximizing the margin $\xi$ between the \gls{decisionboundary} of $\hypothesis^{(\weights)}$ 
					and each class of the \gls{trainset}.}
				\label{fig_svm_gls}
			\end{center}
		\end{figure}
	},first={hinge loss},text={hinge loss}}

\newglossaryentry{iidasspt}{name={i.i.d.\ assumption}, description={The i.i.d.\ assumption\index{i.i.d.} interprets \gls{datapoint}s of a \gls{dataset} 
		as the realizations of \gls{iid} \gls{rv}s.},first={i.i.d.\ assumption},text={i.i.d.\ assumption} }

\newglossaryentry{hypospace}{name={hypothesis space}, description={Every\index{hypothesis space} 
		practical ML method uses a hypothesis space (or \gls{model}) $\hypospace$. The hypothesis space of a ML 
		method is a subset of all possible maps from the \gls{featurespace} to \gls{labelspace}. The design 
		choice of the hypothesis space should take into account available computational resources and 
		statistical aspects. If the computational infrastructure allows for efficient matrix operations, and there 
		is a (approximately) linear relation between \gls{feature}s and \gls{label}, a useful choice for the 
		hypothesis space might be the \gls{linmodel}.},first={hypothesis space},text={hypothesis space} }
	
\newglossaryentry{model}{name={model}, description={In the context of ML methods, 
		the term \emph{model} typically refers to the \gls{hypospace} used by a ML method \cite{ShalevMLBook,MLBasics}.},first={model},text={model} }

\newglossaryentry{modelparams}{name={model parameters}, 
	description={Model parameters are numbers that select a \gls{hypothesis} map from a \gls{hypospace}.},
	first={model parameters},text={model parameters} }

\newglossaryentry{ai}{name={artificial intelligence}, description={Artificial intelligence\index{artificial intelligence} 
		aims to develop systems that behave rational in the sense of maximizing a long-term reward. 
		In MLterms, these systems train a \gls{model} to predict optimal actions in order to 
		minimize a \gls{loss} computed from reward signals.},first={artificial intelligence (AI)},text={AI} }
	
\newglossaryentry{hardclustering}{name={hard clustering}, description={Hard clustering\index{hard clustering} 
		refers to the task of partitioning a given set of \gls{datapoint}s into (few) non-overlapping \gls{cluster}s. 
		Each \gls{datapoint} is assigned to one \gls{cluster}.},first={hard clustering},text={hard clustering} }
	
\newglossaryentry{softclustering}{name={soft clustering}, description={Soft clustering\index{soft clustering} 
		refers to the task of partitioning a given set of \gls{datapoint}s into (few) overlapping clusters. 
		Each \gls{datapoint} is assigned to several different clusters with varying \gls{dob}. Soft clustering 
		methods determine the \gls{dob} (or soft cluster assignment) for each \gls{datapoint} and each \gls{cluster}.
		A principled approach to soft clustering is by interpreting \gls{datapoint}s as \gls{iid} realizations of a 
		\gls{gmm}. We then obtain a natural choice for the \gls{dob} as the conditional probability of a \gls{datapoint} 
		belonging to a specific mixture component.},first={soft clustering},text={soft clustering} }
	
\newglossaryentry{clustering}{name={clustering}, description={Clustering\index{clustering} methods decompose a given 
		set of \gls{datapoint}s into few subsets, which are referred to as \gls{cluster}s. 
		Each \gls{cluster} consists of \gls{datapoint}s that are more similar to each 
		other than to \gls{datapoint}s outside the \gls{cluster}. Different clustering methods 
		use different measures for the similarity between \gls{datapoint}s and different 
		forms of \gls{cluster} representations. The clustering method \gls{kmeans} uses the 
		average \gls{feature} vector (\emph{cluster mean}) of a \gls{cluster} as its representative. 
		A popular \gls{softclustering} method based on \gls{gmm} represents 
		a \gls{cluster} by a \gls{mvndist}.},first={clustering},text={clustering} }
	
\newglossaryentry{cluster}{name={cluster}, description={A\index{cluster} \gls{cluster} is a subset of 
		\gls{datapoint}s that are more similar to each other than to the \gls{datapoint}s outside the \gls{cluster}. 
		The quantitative measure of similarity between \gls{datapoint}s is a design choice. If \gls{datapoint}s 
		are characterized by Euclidean \gls{feature} vectors $\featurevec \in \mathbb{R}^{\nrfeatures}$, 
		we can define the similarity between two \gls{datapoint}s via the Euclidean distance between 
		their \gls{feature} vectors.},first={cluster},text={cluster} }

%\newglossaryentry{softclustering}{name={soft clustering}, description={Soft clustering methods determine, for each \gls{datapoint} within a dataset, 
%		a soft cluster assignment or the degree of belonging to a particular cluster.},first={soft clustering},text={soft clustering} }


\newglossaryentry{huberloss}{name={Huber loss}, description={The\index{Huber loss} 
		Huber \gls{loss} is a generalization and combination of the \gls{sqerrloss} and 
		the absolute error \gls{loss}.},first={Huber loss},text={Huber loss} }

\newglossaryentry{svm}{name={support vector machine}, description={The\index{support vector machine} 
		support vector machine is a binary classification method that learns a linear \gls{hypothesis} map. 
		It aims at maximally separating \gls{datapoint}s from the two different classes in the \gls{feature} 
		space (\emph{maximum margin principle}). Maximizing this separation is equivalent to minimizing a regularized variant of 
		the \gls{hingeloss} \eqref{equ_hinge_loss_gls}.},first={support vector machine (SVM)},text={SVM} }

\newglossaryentry{eigenvalue}{name={eigenvalue}, description={We refer to a number $\lambda \in \mathbb{R}$ 
		as eigenvalue of a square matrix $\mathbf{A} \in \mathbb{R}^{\featuredim \times \featuredim}$ if there is a 
		non-zero vector $\vx \in \mathbb{R}^{\featuredim} \setminus \{ \mathbf{0} \}$ such that $\mathbf{A} \vx = \lambda \vx$. },first={eigenvalue},text={eigenvalue} }
	
\newglossaryentry{eigenvector}{name={eigenvector}, description={An\index{eigenvector} 
		eigenvector of a matrix $\mathbf{A} \in \mathbb{R}^{\featuredim \times \featuredim}$ 
		is a non-zero vector $\vx \in \mathbb{R}^{\featuredim} \setminus \{ \mathbf{0} \}$ 
		such that $\mathbf{A} \vx = \lambda \vx$ with some \gls{eigenvalue} $\lambda$.},first={eigenvector},text={eigenvector} }

\newglossaryentry{evd}{name={eigenvalue decomposition}, 
	description={The\index{eigenvalue decomposition} \gls{eigenvalue} 
		decomposition for a square matrix $\mA \in \mathbb{R}^{\dimlocalmodel \times \dimlocalmodel}$ 
		is a factorization of the form 
		$$\mA = \mathbf{V} {\bm \Lambda} \mathbf{V}^{-1}.$$ 
		The columns of the matrix $\mV = \big( \vv^{(1)},\ldots,\vv^{(\dimlocalmodel)} \big)$ are the 
		\gls{eigenvector}s of the matrix $\mV$. The diagonal matrix 
		${\bm \Lambda} = {\rm diag} \big\{ \eigval{1},\ldots,\eigval{\dimlocalmodel} \big\}$ 
		contains the \gls{eigenvalue}s $\eigval{\featureidx}$ corresponding to the \gls{eigenvector}s $\vv^{(\featureidx)}$. 
		Note that the above decomposition exists only if the matrix $\mA$ is diagonalizable.},first={eigenvalue decomposition (EVD)},text={EVD} }

\newglossaryentry{svd}{name={singular value decomposition}, 
  	description={The\index{singular value decomposition} singular value 
  		decomposition for a matrix 
		$\mA \in \mathbb{R}^{\samplesize \times \dimlocalmodel}$ 
		is a factorization of the form 
		$$\mA = \mathbf{V} {\bm \Lambda} \mathbf{U}^{T},$$ 
		with orthonormal matrices $\mV \in \mathbb{R}^{\samplesize \times \samplesize}$ 
		and $\mU \in \mathbb{R}^{\dimlocalmodel \times \dimlocalmodel}$ \cite{GolubVanLoanBook}. 
		The matrix ${\bm \Lambda} \in \mathbb{R}^{\samplesize \times \dimlocalmodel}$ is 
		only non-zero along the main diagonal, whose entries $\Lambda_{\featureidx,\featureidx}$ 
		are non-negative and referred to as singular values.
	},first={singular value decomposition (SVD)},text={SVD} }


\newglossaryentry{tv}{name={total variation}, description={See \gls{gtv}.},
	first={total variation},text={total variation} }


\newglossaryentry{gdmethods}{name={gradient-based method}, description={Gradient-based\index{gradient-based methods} 
		methods are iterative techniques for finding the minimum (or maximum) 
		of a \gls{differentiable} objective function of the \gls{modelparams}. These 
		methods construct a sequence of approximations to an optimal choice for 
		\gls{modelparams} that results in a minimum objective function value. 
		As their name indicates, gradient-based methods use the \gls{gradient}s of the objective function 
		evaluated during previous iterations to construct new (hopefully) improved \gls{modelparams}.},
		first={gradient-based methods},text={gradient-based methods} }

\newglossaryentry{sgd}{name={subgradient descent}, description={Subgradient\index{subgradient descent} 
		descent is a generalization of \gls{gd} that does not require differentiability of the 
		function to be minimized. This generalization is obtained by replacing the concept 
		of a \gls{gradient} with that of a sub-gradient. Similar to \gls{gradient}s, also sub-gradients 
		allow to construct local approximations of an objective function. The objective function 
		might be the \gls{emprisk} $\emperror\big( \hypothesis^{(\weights)} \big| \dataset \big)$ viewed 
		as a function of the \gls{modelparams} $\weights$ that select a \gls{hypothesis} $\hypothesis^{(\weights)} \in \hypospace$.},first={subgradient descent},text={subgradient descent} }
	
\newglossaryentry{stochGD}{name={stochastic gradient descent}, description={Stochastic\index{stochastic gradient descent} \gls{gd} is 
		obtained from \gls{gd} by replacing the \gls{gradient} of the objective function with some e
		stimate (or approximation). A main application of stochastic gradient descent is to solve \gls{erm} 
		where the objective function and its gradient consists of a sum over the \gls{datapoint}s in a \gls{dataset} $\dataset$. 
		Here, the gradient estimate can be obtained by replacing the sum over the entire \gls{dataset} with 
		a sum over a randomly selected subset of $\dataset$. },first={stochastic gradient descent (SGD)},text={SGD} }

\newglossaryentry{pca}{name={principal component analysis (PCA)}, description={Principal\index{principal component analysis} 
		component analysis determines a linear \gls{featuremap} such that the new \gls{feature}s allow to reconstruct 
		the original \gls{feature}s with minimum reconstruction error \cite{MLBasics}.},first={principal component analysis (PCA)},text={PCA} }
	
\newglossaryentry{loss}{name={loss}, description={ML\index{loss} methods use a 
		\gls{lossfunc} $\lossfunc{\datapoint}{\hypothesis}$ to measure the error incurred 
		by applying a specific \gls{hypothesis} to a specific \gls{datapoint}. With 
		slight abuse of notation, we use the term \emph{loss} for both, the \gls{lossfunc} $\loss$ 
		itself and for its value $\lossfunc{\datapoint}{\hypothesis}$ for a specific \gls{datapoint} $\datapoint$ 
		and \gls{hypothesis} $\hypothesis$.},first={loss},text={loss} }

\newglossaryentry{lossfunc}{name={loss function}, description={A\index{loss function} loss function is a map 
		$$\lossfun: \featurespace \times \labelspace \times \hypospace \rightarrow \mathbb{R}_{+}: \big( \big(\featurevec,\truelabel\big), \hypothesis\big) \mapsto  \lossfunc{(\featurevec,\truelabel)}{\hypothesis}$$ which assigns a pair 
		of a \gls{datapoint}, with features $\featurevec$ 
		and label $\truelabel$, and a \gls{hypothesis} $\hypothesis \in \hypospace$ the 
		non-negative real number $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$. The 
		loss value $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$ quantifies the discrepancy 
		between the true \gls{label} $\truelabel$ and the \gls{prediction} $\hypothesis(\featurevec)$. 
		Lower (closer to zero) values $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$ indicate a smaller 
		discrepancy between \gls{prediction} $\hypothesis(\featurevec)$ and label $\truelabel$. 
		Figure \ref{fig_loss_function_gls} depicts a \gls{lossfunc} for a given \gls{datapoint}, 
		with \gls{feature}s $\featurevec$ and label $\truelabel$, as a function of the \gls{hypothesis} $\hypothesis \in \hypospace$. 
		\begin{figure}[htbp]
			\begin{center}
				\begin{tikzpicture}[scale = 0.7]
					\begin{axis}
						[%grid, 
						axis x line=center,
						axis y line=center,
						%	xtick={-2,-1,...,2},
						%	ytick={0,1,...,2},
						xlabel={},
						%	ylabel={\hspace*{3mm} loss $\lossfun$},
						xlabel style={below right},
						ylabel style={above right},
						xtick=\empty,
						ytick=\empty,
						xmin=-4,
						xscale = 1.4, 
						xmax=4,
						ymin=-0.5,
						ymax=2.5
						]
						\addplot [smooth, ultra thick] table [x=a, y=b, col sep=comma] {logloss.csv};    
					\end{axis}
					\node [above] at (1,5) {$\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$};
					\node [above] at (10,1) {\gls{hypothesis} $\hypothesis$};
						\node [right] at (4,6) {\gls{loss}};
				\end{tikzpicture}
			\end{center}
			\vspace*{-7mm}
			\caption{Some \gls{lossfunc} $\lossfunc{(\featurevec,\truelabel)}{\hypothesis}$ for a fixed \gls{datapoint}, with 
				\gls{feature} vector $\featurevec$ and \gls{label} $\truelabel$, and varying \gls{hypothesis} $\hypothesis$. 
				ML methods try to find (learn) a \gls{hypothesis} that incurs minimum \gls{loss}.}
			\label{fig_loss_function_gls}
	\end{figure}
 },first={loss function},text={loss function} }

\newglossaryentry{decisiontree}{name={decision tree}, description={A\index{decision tree} 
		decision tree is a flow-chart-like representation of a \gls{hypothesis} map $\hypothesis$. 
		More formally, a decision tree is a directed graph which reads in the feature vector $\featurevec$ 
		of a \gls{datapoint} at its root node. The root node then forwards the \gls{datapoint} to one 
		of its children nodes based on some elementary test on the \gls{feature}s $\featurevec$. 
		If the receiving children node is not a leaf node, i.e., it has itself children nodes, 
	  it represents another test. Based on the test result, the \gls{datapoint} is further 
	  pushed to one of its descendants. This testing and forwarding of the \gls{datapoint} is continued 
	  until the \gls{datapoint} ends up in a leaf node (having no children nodes). 
	  Each leaf node corresponds to a \gls{decisionregion}, a subset of the \gls{featurespace} 
	  mapped to the same output $\hypothesis(\featurevec)$.},first={decision tree},text={decision tree} }

%\newglossaryentry{noniid}{name={non-i.i.d.\}, description={We\index{non-i.i.d.} refer to a 
%			\gls{dataset} as non-i.i.d.\ if its \gls{datapoint}s cannot be well modelled as \gls{realization}s 
%			of \gls{iid} \gls{rv}s.},first={non-i.i.d.\ data},text={non-i.i.d.\ data} }
%\newglossaryentry{linclass}
%{
%	name=linear classifier,
%	description={A linear classifier $h(\vx)$ divides the feature space $\mathbb{R}^{\featurelen}$ into two half-spaces 
%		such that data points in the same half-space result in the same predicted label.}
%}

\newglossaryentry{API} 
{
	name={Application Programming Interface (API)},
	description={An\index{application programming interface} application programming 
		interface (API) is a precise specification of the services and resources 
		offered by software or hardware implementing that API.},
	first={application programming interface (API)},
	text={API}
}

\newglossaryentry{hilbertspace}{name={Hilbert space},description={A\index{Hilber space} 
		Hilbert space is a linear vector space equipped with an inner product between 
		pairs of vectors. One important example of a Hilbert space is the Euclidean space 
		$\mathbb{R}^{\featuredim}$, for some dimension $\featuredim$, which consists of 
		Euclidean vectors $\vu = \big(u_{1},\ldots,u_{\featurelen}\big)^{T}$ along with the inner 
		product $\vu^{T} \vv$.},first={Hilbert space},text={Hilbert space}}



\newglossaryentry{sample}{name={sample},description={A\index{sample} 
		finite sequence (list) of \gls{datapoint}s $\datapoint^{(1)},\ldots,\datapoint^{(\sampleidx)}$ that 
		is obtained or interpreted as the realizations of $\samplesize$ \gls{iid} \gls{rv}s 
		with the common \gls{probdist} $p(\datapoint)$. The length $\samplesize$ of 
		the sequence is referred to as the \gls{samplesize}.},first={sample},text={sample}}
	
\newglossaryentry{samplesize}
{name=sample size,
	description={The\index{sample size} number of individual \gls{datapoint}s 
		contained in a \gls{dataset} obtained as the \gls{realization}s of \gls{iid} \gls{rv}s with 
		common \gls{probdist}.},first={sample size},text={sample size}
}

\newglossaryentry{ann}
{name=artificial neural network,
	description={An\index{artificial neural network} artificial neural network is a 
		graphical (signal-flow) representation of a map from \gls{feature}s of 
		a \gls{datapoint} at its input to a \gls{prediction} for the \gls{label} 
		as its output.},first={artificial neural network (ANN)},text={ANN}
}

\newglossaryentry{randomforest}
{name=random forest,
	description={A\index{random forest} random forest is a set (ensemble) of different \gls{decisiontree}s. 
		Each of these \gls{decisiontree}s is obtained by fitting a perturbed copy of 
		the original \gls{dataset}.},first = {random forest}, text={random forest}
}

\newglossaryentry{bagging}{name={bagging},description={Bagging\index{bagging} (or \emph{bootstrap aggregation}) is a generic 
		technique to improve (the robustness of) a given ML method. The idea is to use the \gls{bootstrap} 
		to generate perturbed copies of a given \gls{dataset} and then to learn a separate \gls{hypothesis} for 
		each copy. The resulting set of hypotheses is then used to predict the \gls{label} of a \gls{datapoint} 
		by combining or aggregating the individual predictions of each \gls{hypothesis}. 
		For \gls{hypothesis} maps delivering numeric label values, this aggregation 
		could be implemented by computing the average of individual \gls{prediction}s.},first={bootstrap aggregation (bagging)},text={bagging}}

\newglossaryentry{gd}{name={gradient descent (GD)},description={Gradient\index{gradient descent} 
		descent is an iterative method for finding the minimum of a \gls{differentiable} 
		function $f(\weights)$. },first={gradient descent (GD)},text={GD}}


\newglossaryentry{ladregression}{name={least absolute deviation regression},description={
		%Consider a \gls{dataset} constituted by \gls{datapoint}s, each characterized by \gls{feature}s 
		%$\featurevec$ and a numeric \gls{label} $\label \in \mathbb{R}$. 
		Least\index{least absolute deviation regression} absolute deviation regression is an instance of \gls{erm} 
		using the absolute error loss.
		},
		first={least absolute deviation regression},text={least absolute deviation regression}}

%\newglossaryentry{metric}{name={metric},description={We\index{metric} sometimes use \emph{metric} to refer to 
%		a \gls{lthat is used solely 
%	    for the final performance evaluation of a learnt hypothesis. The metric is typically a \gls{lossfunc} that 
%	    has a ``natural'' interpretation (such as the \gls{zerooneloss}) but is not a good choice to guide 
%	    the learning process, e.g., via \gls{erm}. For \gls{erm}, we typically prefer \gls{lossfunc}s that depend smoothly 
%	    on the (parameters of the) hypothesis. Examples for such smooth \gls{lossfunc}s include the \gls{sqerrloss} 
%	    and the \gls{logloss} \eqref{equ_log_loss_gls}.},first={metric},text={metric}}

\newglossaryentry{bayesrisk}{name={Bayes risk},description={Consider \gls{datapoint}s being \gls{realization}s of 
		\gls{iid} \gls{rv}s with a common \gls{probdist}. The\index{Bayes risk} 
		Bayes risk is the minimum possible \gls{risk} that can be achieved by 
		any \gls{hypothesis} $\hypothesis$ out of a model $\hypospace$. 
		Any \gls{hypothesis} map achieving the minimum \gls{risk} is referred 
		to as a \gls{bayesestimator} \cite{LC}.},first={Bayes risk},text={Bayes risk}}
	
\newglossaryentry{bayesestimator}{name={Bayes estimator},description={A\index{Bayes estimator} 
		\gls{hypothesis} $\hypothesis$ whose \gls{bayesrisk} coincides with the \gls{bayesrisk} \cite{LC}.},
		first={Bayes estimator},text={Bayes estimator}}


\newglossaryentry{weights}{name={weights},
	description={Consider\index{weights} a parametrized \gls{hypospace} $\hypospace$. 
		We\index{weights} use the term weights for numeric \gls{modelparams} that are 
		used to scale \gls{feature}s or their transformations in order to compute $\hypothesis^{(\weights)} \in \hypospace$. A \gls{linmodel} uses weights $\weights=\big(\weight_{1},\ldots,\weight_{\nrfeatures}\big)^{T}$ to compute 
		the linear combination $\hypothesis^{(\weights)}(\featurevec)= \weights^{T} \featurevec$. 
		Weights are also used in \gls{ann}s to form linear combinations of \gls{feature}s or the 
		outputs of neurons in hidden layers.},first={weights},text={weights}}
	
\newglossaryentry{probdist}{name={probability distribution},
	description={To\index{probability distribution} analyze ML methods it can be useful 
		to interpret \gls{datapoint}s as \gls{iid} \gls{realization}s of a \gls{rv}. The typical 
		properties of such \gls{datapoint}s are then governed by the probability distribution 
		of this \gls{rv}. The probability distribution of a binary \gls{rv} $\truelabel \in \{0,1\}$ 
		is fully specified by the probabilities $\prob{\truelabel = 0}$ and 
		$\prob{\truelabel=1} \big(\!=\!1\!-\!\prob{\truelabel=0} \big)$. The probability 
		distribution of a real-valued \gls{rv} $\feature \in \mathbb{R}$ might be specified 
		by a probability density function $p(\feature)$ such that $\prob{ \feature \in [a,b] } \approx  p(a) |b-a|$. 
	    In the most general case, a probability distribution is defined by a probability measure \cite{GrayProbBook,BillingsleyProbMeasure}.},first={probability distribution},text={probability distribution}}
    
    
\newglossaryentry{pdf}{name={probability density function (pdf)},
	description={The\index{probability density function} probability density function (pdf) $p(\feature)$ 
		of a real-valued \gls{rv} $\feature \in \mathbb{R}$ is a particular representation of its \gls{probdist}. 
		If the pdf exists, it can be used to compute the probability that $\feature$ takes on a value 
		from a (measurable) set $\mathcal{B} \subseteq \mathbb{R}$ via $\prob{\feature \in \mathcal{B}} = \int_{\mathcal{B}} p(\feature') d \feature'$ \cite[Ch. 3]{BertsekasProb}. The pdf of a vector-valued \gls{rv} $\featurevec \in \mathbb{R}^{\featuredim}$ (if it exists) 
        allows to compute the probability that $\featurevec$ falls into a (measurable) region $\mathcal{R}$ via 
        $\prob{\featurevec \in \mathcal{R}} = \int_{\mathcal{R}} p(\featurevec') d \feature_{1}' \ldots d \feature_{\featuredim}' $ \cite[Ch. 3]{BertsekasProb}.},
first={probability density function (pdf)},text={pdf}}


\newglossaryentry{parameters}{name={parameters},
	description={The\index{parameters} parameters of a ML \gls{model} are tunable 
		(learnable or adjustable) quantities that allow to choose between different \gls{hypothesis} maps. 
		For example, the linear model $\hypospace \defeq \{\hypothesis^{(\weights)}: \hypothesis^{(\weights)}(\feature)= \weight_{1} \feature + \weight_{2}\}$ 
		consists of all \gls{hypothesis} maps $\hypothesis^{(\weights)}(\feature)= \weight_{1} \feature + \weight_{2}$ 
		with a particular choice for the parameters $\weights = \big(\weight_{1},\weight_{2}\big)^{T} \in \mathbb{R}^{2}$. 
		Another example of parameters is the weights assigned to the connections 
		between neurons of an \gls{ann}.},first={parameters},text={parameters}}

\newglossaryentry{lln}{name={law of large numbers},
	description={The\index{law of large numbers} law of large numbers refers to the 
		convergence of the average of an increasing (large) number of \gls{iid} \gls{rv}s 
		to the \gls{mean} of their common \gls{probdist}. Different instances of the 
		law of large numbers are obtained using different notions of convergence \cite{papoulis}.},first={law of large numbers},text={law of large numbers}}
    
\newglossaryentry{stopcrit}{name={stopping criterion},
	description={Many\index{stopping criterion} ML methods use iterative algorithms that construct a 
		sequence of model parameters (such as the weights of a linear map or 
		the weights of an \gls{ann}) that (hopefully) converge to an optimal choice 
		for the model parameters. In practice, given finite computational 
		resources, we need to stop iterating after a finite number of times. 
		A stopping criterion is any well-defined condition required for stopping 
		iterating.},first={stopping criterion},text={stopping criterion}}

\newglossaryentry{kCV}{name={$k$-fold cross-validation ($\nrfolds$-fold CV)},
	description={$k$-fold cross-validation\index{k-fold cross-validation} is a 
		method for learning and validating a \gls{hypothesis} using a given \gls{dataset}. 
		This method divides the \gls{dataset} evenly into $k$ subsets or \emph{folds} 
		and then executes $k$ repetitions of \gls{model} training (e.g., via \gls{erm}) and \gls{validation}. 
		Each repetition uses a different fold as the \gls{valset} and the remaining $k-1$ folds 
		as a \gls{trainset}. The final output is the average of the \gls{valerr}s obtained 
		from the $k$ repetitions.},first={$k$-fold cross-validation ($k$-fold CV)},text={$k$-fold CV}}
	
\newglossaryentry{renyidiv}{name={R\'enyi divergence}, 
	description={The R\'enyi divergence\index{R\'enyi divergence} measures the (dis-)similarity 
		between two \gls{probdist}s \cite{RenyiInfo95}.}, 
	first = {R\'enyi divergence}, text = {R\'enyi divergence}} 

\newglossaryentry{nonsmooth}{name={non-smooth},
	description={We\index{non-smooth} refer to a function as non-smooth if it is not 
		\gls{smooth} \cite{nesterov04}.},first={non-smooth},text={non-smooth}}

\newglossaryentry{convex}{name={convex},
	description={A\index{convex} subset $\mathcal{C} \subseteq \mathbb{R}^{\featuredim}$ of the 
		\gls{euclidspace} $\mathbb{R}^{\featuredim}$ is referred to as 
		convex if it contains the line segment between any two points 
		of that set. We define a function as convex if its epigraph is a 
		convex set \cite{BoydConvexBook}.},first={convex},text={convex}}


\newglossaryentry{smooth}{name={smooth},
	description={We\index{smooth} refer to a real-valued function as smooth if it is \gls{differentiable} 
		and its \gls{gradient} is continuous \cite{nesterov04,CvxBubeck2015}. A 
		differentiable function $f(\weights)$ is referred to as $\beta$-smooth if the \gls{gradient} 
		$\nabla f(\weights)$ is Lipschitz continuous with Lipschitz constant $\beta$, i.e., 
		$$\| \nabla f(\weights) - \nabla f(\weights') \| \leq \beta \| \weights - \weights' \|.$$ },first={smooth},text={smooth}}

\newglossaryentry{dataug}{name={data augmentation},
	description={Data augmentation\index{data augmentation} methods add synthetic \gls{datapoint}s 
		to an existing set of \gls{datapoint}s. These synthetic \gls{datapoint}s might be obtained by 
		perturbations (adding noise) or transformations (rotations of images) of the original \gls{datapoint}s. 
		These perturbations and transformations are such that the resulting synthetic \gls{datapoint}s should 
		still have the same \gls{label}. As a case in point, a rotated cat image is still a cat image even if 
		their \gls{feature} vectors (obtained by stacking pixel color intensities) are very different.},first={data augmentation},text={data augmentation}}
	
	
\newglossaryentry{localdataset}{name={local dataset},description={The\index{local dataset} concept of a local dataset is 
		in-between the concept of a \gls{datapoint} and a \gls{dataset}. A local dataset consists of several 
		individual \gls{datapoint}s which are characterized by \gls{feature}s and \gls{label}s. In contrast to a 
		single \gls{dataset} used in basic ML methods, a local dataset is also related to other local datasets via different notions 
		of similarities. These similarities might arise from \gls{probmodel}s or communication infrastructure and 
		are encoded in the edges of a \gls{empgraph}.},first={local dataset},text={local dataset}}
	
\newglossaryentry{localmodel}{name={local model},description={Consider\index{local model} a collections 
		of \gls{localdataset}s that are assigned to the nodes of a \gls{empgraph}. A local model $\localmodel{\nodeidx}$ 
		is a \gls{hypospace} assigned to a node $\nodeidx \in \nodes$. Different nodes might be assigned 
		different \gls{hypospace}s, i.e., in general $\localmodel{\nodeidx} \neq \localmodel{\nodeidx'}$ for different 
		nodes $\nodeidx, \nodeidx' \in \nodes$.  },first={local model},text={local model}}
	
\newglossaryentry{mutualinformation}
{name={mutual information},
 description={The\index{mutual information} mutual information $\mutualinformation{\featurevec}{\truelabel}$ 
 	between two \gls{rv}s $\featurevec$, $\truelabel$ defined on the same probability 
 	space is given by \cite{coverthomas} $$\mutualinformation{\featurevec}{\truelabel} \defeq \expect \left\{ \log \frac{p (\featurevec,\truelabel)}{p(\featurevec)p(\truelabel)} \right\}.$$ It is a measure for how well we can estimate $\truelabel$ based 
	solely from $\featurevec$. A large value of $\mutualinformation{\featurevec}{\truelabel}$ indicates that 
	$\truelabel$ can be well predicted solely from $\featurevec$. This \gls{prediction} could be obtained by a 
		\gls{hypothesis} learnt by a \gls{erm}-based ML method. 
	 }, first = {mutual information (MI)}, text={MI} 
}

\newglossaryentry{zerogradientcondition}{name={zero-gradient condition},
	description={Consider\index{zero-gradient condition} the unconstrained 
		optimization problem $\min_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights)$  with 
			a \gls{smooth} and \gls{convex} \gls{objfunc} $f(\weights)$. A necessary and 
			sufficient condition for a vector $\widehat{\weights} \in \mathbb{R}^{\dimlocalmodel}$ 
			to solve this problem is that the \gls{gradient} $\nabla f \big( \widehat{\weights} \big)$ is the zero-vector, 
			$$ \nabla f \big( \widehat{\weights} \big) = \mathbf{0} \Leftrightarrow  f \big( \widehat{\weights} \big) = \min_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights) .$$ }, 
			first={zero-gradient condition},text={zero-gradient condition}}


\newglossaryentry{edgeweight}{name={edge weight},
	description={Each\index{edge weight} edge $\edge{\nodeidx}{\nodeidx'}$ of a \gls{empgraph} is 
		assigned a non-negative \gls{edgeweight}  $\edgeweight_{\nodeidx,\nodeidx'}\geq0$. 
		A zero \gls{edgeweight} $\edgeweight_{\nodeidx,\nodeidx'}=0$ indicates the absence 
		of an edge between nodes $\nodeidx, \nodeidx' \in \nodes$.}, 
	first={edge weight},text={edge weight}}


\newglossaryentry{dataminprinc}{name={data minimization principle},
	description={European\index{data minimization principle} data protection regulation 
		includes a data minimization principle. This principle requires a data controller to 
		limit the collection of personal information to what is directly relevant and necessary 
		to accomplish a specified purpose. The data should be retained only for as long as 
		necessary to fulfill that purpose \cite[Article 5(1)(c)]{GDPR2016} \cite{EURegulation2018}.}, 
	first={data minimization principle},text={data minimization principle}}




==> trusterm_glossary.tex <==

\newglossaryentry{minimum}
{
	name=minimum,
	description={Given a set of real numbers, the minimum is the smallest of those numbers.},
	first={minimum},text={minimum}
}


\newglossaryentry{maximum}
{name=maximum,
 description={Given a set of real numbers, the maximum is the largest of those numbers.},
 first={maximum},text={maximum}
}

\newglossaryentry{discrepancy}
{name=discrepancy,
	description={
		Consider a \gls{fl} application with networked data represented by an \gls{empgraph}. 
		\gls{fl} methods use a discrepancy measure to compare \gls{hypothesis} maps from 
	local models at nodes $\nodeidx,\nodeidx'$ connected by an edge in the \gls{empgraph}.},
	first={discrepancy},text={discrepancy}
}



\newglossaryentry{hfl}
{name={horizontal \gls{fl}},description=
	{Horizontal \gls{fl} refers to applications with \gls{localdataset}s that are constituted by different 
		\gls{datapoint}s but using the same \gls{feature}s to characterize them \cite{HFLChapter2020}. 
		One example for horizontal \gls{fl} is numerical weather prediction using a network of 
		weather (observation) stations. Each weather station measures the same quantities 
		such as daily temperature, air pressure and precipitation. However, different weather 
		stations measure the characteristics or \gls{feature}s of different spatio-temporal regions 
		(each such region being a separate \gls{datapoint}).},
	first={horizonal \gls{fl}},text={horizontal \gls{fl}}
} 

\newglossaryentry{dimred}
{name={dimensionality reduction},
	description={Dimensionality reduction methods map (typically many) raw 
		features to a (relatively small) set of new features. These methods can 
		be used to visualize \gls{datapoint}s by learning two \gls{feature}s 
		that can be used as the coordinates of a depication in a \gls{scatterplot}.}, first={dimensionality reduction},text={dimensionality reduction}
} 

\newglossaryentry{featlearn}
{name={feature learning},
	description={Feature learning refers to the task of learning a map $\featuremapvec$ that 
		reads in raw \gls{feature}s of a \gls{datapoint} and delivers new \gls{feature}s. Different 
		\gls{feature} learning methods are obtained for different quantitative measures for the 
		usefulness of the new \gls{feature}s.},
	first={feature learning},text={feature learning}
} 

\newglossaryentry{autoencoder}
{name={autoencoder},
	description={An autoencoder is a ML method that jointly learns an encoder map 
		$\hypothesis(\cdot) \in \hypospace$ and a decoder map $\hypothesis^{*}(\cdot) \in \hypospace^{*}$. 
		It is an instance of \gls{erm} using a \gls{loss} computed from the reconstruction error 
		$\featurevec - \hypothesis^{*}\big(  \hypothesis \big( \featurevec \big) \big)$.},
	first={autoencoder},text={autoencoder}
} 

\newglossaryentry{vfl}
{name={vertical \gls{fl}},description=
	{Vertical \gls{fl} refers to applications with \gls{localdataset}s that are constituted 
	 by the same \gls{datapoint}s but characterizing them with different \gls{feature}s \cite{VFLChapter}. 
     For example, different healthcare providers might all contain information about the same population 
     of patients. However, different healthcare providers collect different measurements (blood 
      values, electrocardiography, lung x-ray) for the same patients.},
	first={vertical \gls{fl}},text={vertical \gls{fl}}
} 

\newglossaryentry{interpretability}
{name={interpretability},description=
		{A ML method is interpretable for a specific user if she can well anticiapte the predictions 
			delivered by the method. The notion of interpretability can be made precise using quantitative 
			measures of the uncertainty about the predictions \cite{JunXML2020}.},
		first={interpretability},text={interpretability}
}

\newglossaryentry{learningtask}
{name={learning task},description=
	{A learning tasks consists of a specific choice for a collection of \gls{datapoint}s (e.g., all images 
		stored in a particular database), their \gls{feature}s and \gls{label}s.},
	first={learning task},text={learning task}
}

\newglossaryentry{featuremtx}
{name={feature matrix},description=
	{Consider a \gls{dataset} $\dataset$ of $\samplesize$ \gls{datapoint}s that are 
		characterized by feature vectors $\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)}$. It is 
	convenient to collect these feature vectors into a feature matrix $\mX \defeq \big(\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)}\big)$. },
	first={feature matrix},text={feature matrix}
}



\newglossaryentry{explainability}
{name={explainability},description=
		{We define the (subjective) explainability of a ML method as the level of 
		 simulatability \cite{Colin:2022aa} of the \gls{prediction}s delivered to a 
		 specific human user. Quantitative measures for the (subjective) explainability of 
		a trained model can be constructed by comparing its predictions with the corresponding 
		guesses provided by a user on a test-set \cite{Zhang:2024aa}. Alternatively, 
		we can use \gls{probmodel}s for \gls{data} and measure explainability of a trained ML model 
		via the (differential) conditional entropy of its \gls{prediction}s \cite{JunXML2020,Chen2018}. 
		},
		first={explainability},text={explainability}
	}

\newglossaryentry{linmodel}{name={linear model},
	description={We use the term linear model in a very specific sense. 
		In particular, a linear model is a \gls{hypospace} which consists of all linear maps, 
	\begin{equation} 
		\label{equ_def_lin_model_hypspace}
		\linmodel{\nrfeatures} \defeq \left\{ \hypothesis(\featurevec)= \weights^{T} \featurevec: \weights \in \mathbb{R}^{\nrfeatures} \right\}. 
	\end{equation} 
	Note that \eqref{equ_def_lin_model_hypspace} defines an entire family of \gls{hypospace}s, which is 
	parametrized by the number $\nrfeatures$ of \gls{feature}s that are linearly combined to form the 
	\gls{prediction} $\hypothesis(\featurevec)$. The design choice of $\nrfeatures$ is guided by \gls{compasp} 
	(smaller $\nrfeatures$ means less computation), \gls{statasp} (increasing $\nrfeatures$ might reduce \gls{prediction} 
	error) and \gls{interpretability} (a linear model using few carefully chosen \gls{feature}s might be considered interpretable).}, 
   first={linear model},text={linear model}}
	
	
\newglossaryentry{gradstep}{name={gradient step},description={Given a \gls{differentiable} real-valued 
		function $f(\weights)$ and a vector $\weights'$, the \gls{gradient} step updates $\weights'$ by adding 
		the scaled negative \gls{gradient} $\nabla f(\weights')$, $\weights' \mapsto \weights' - \lrate \nabla f(\weights')$.},first={gradient step},text={gradient step}}
	

\newglossaryentry{proxop}{name={proximal operator},description={Given a \gls{convex} function 
		and a vector $\vx$, we define its proximity operator as $$\proximityop{\locallossfunc{\nodeidx}{\cdot}}{\weights''}{2 \regparam}\defeq \argmin_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights) + (\rho/2) \normgeneric{\weights- \weights'}{2}^{2} \mbox{ with } \rho > 0. $$ 
		\Gls{convex} functions for which the proximity operator can be computed efficiently are sometimes referred 
		to as ``proximable'' or ``simple'' \cite{Condat2013}.},first={proximity operator},text={proximity operator}}

\newglossaryentry{proximable}{name={proximable},description={A \Gls{convex} function for which the \gls{proxop} 
		can be computed efficiently are sometimes referred to as ``proximable'' or ``simple'' \cite{Condat2013}.},first={proximable},text={proximable}}


\newglossaryentry{connected}{name ={connected graph}, description={An undirected graph $\graph=\pair{\nodes}{\edges}$ 
		is connected if we cannot find a (non-empty) subset $\nodes' \subset \nodes$ with no edges leaving 
		$\nodes'$.}, first={connected},text={connected}}

\newglossaryentry{mvndist}{name ={multivariate normal distribution}, description={The multivariate normal 
		distribution $\mvnormal{\vm}{\mC}$ is an important family of\gls{probdist}s for a continuous 
		\gls{rv} $\featurevec \in \mathbb{R}^{\nrfeatures}$ \cite{BertsekasProb,GrayProbBook,Lapidoth09}. 
		This family is paramtrized by the mean $\vm$ and \gls{covmtx} $\mC$ of $\featurevec$. If the \gls{covmtx} 
		is invertible, the \gls{probdist} of $\featurevec$ is 
		$$p(\featurevec) \propto \exp\bigg(-(1/2) \big( \featurevec - \vm \big)^{T} \mC^{-1} \big( \featurevec - \vm \big) \bigg).$$}, first={multivariate normal distribution},text={multivariate normal distribution}}

\newglossaryentry{statasp}{name ={statistical aspects}, description={By statistical aspects 
		of a ML method, we refer to (properties of) the \gls{probdist} of its ouput given a \gls{probmodel} 
		for the data fed into the method.},first={statistical aspects},text={statistical aspects}}

\newglossaryentry{compasp}{name ={computational aspects}, description={By computational 
		aspects of a ML method, we mainly refer to the computational resources required for its 
		implementation. For example, if a ML method uses iterative optimization techniques to 
		solve \gls{erm}, then its computational aspects include (i) how many arithmetic operations are 
		needed to implement a single iteration (\gls{gradstep}) and (ii) how many iterations are needed 
		to obtain useful \gls{modelparams}. One important example for an iterative optimization 
		technique is \gls{gd}.}, first={computational aspects},text={computational aspects}}

\newglossaryentry{zerooneloss}{name={$0/1$ \gls{loss}},
	description={The $0/1$ loss $\loss{\pair{\featurevec}{\truelabel}}{\hypothesis}$ measures the quality of a 
	\gls{classifier} $\hypothesis(\featurevec)$ that delivers a \gls{prediction} $\predictedlabel$ (e.g., 
	via thresholding \eqref{equ_def_threshold_bin_classifier}) for a \gls{label} $\truelabel$ of a \gls{datapoint}. 
	It is equal to $0$ if the \gls{prediction} is correct, i.e., 
	$\loss{\pair{\featurevec}{\truelabel}}{\hypothesis}=0$ when $\predictedlabel=\truelabel$. It is 
	equal to $1$ if the \gls{prediction} is wrong, $\loss{\pair{\featurevec}{\truelabel}}{\hypothesis}=1$ 
	when $\predictedlabel\neq\truelabel$.},
    first={$0/1$ \gls{loss}},text={$0/1$ \gls{loss}}}

\newglossaryentry{probability}{name={probability},
	description={We assign a probability value, typically chosen in the interval $[0,1]$, to each event that might 
		occur in a random experiment \cite{KallenbergBook,BertsekasProb,BillingsleyProbMeasure,HalmosMeasure}.},first={probability},text={probability}}
	
\newglossaryentry{underfitting}{name={underfitting},description={Consider a ML method that uses 
		\gls{erm} to learn a \gls{hypothesis} with minimum \gls{emprisk} on a given \gls{trainset}. 
		Such a method is ``underfitting'' the \gls{trainset} if it is not able to learn a \gls{hypothesis} 
		with sufficiently small \gls{emprisk} on the \gls{trainset}. If a method is underfitting it will typically 
	also not be able to learn a \gls{hypothesis} with a small \gls{risk}.},first={underfitting},text={underfitting}}

\newglossaryentry{overfitting}{name={overfitting},description={Consider a ML method that uses 
		\gls{erm} to learn a \gls{hypothesis} with minimum \gls{emprisk} on a given \gls{trainset}. 
		Such a method is ``overfitting'' the \gls{trainset} if it learns \gls{hypothesis} with small 
		\gls{emprisk} on the \gls{trainset} but unacceptably large \gls{loss} outside the \gls{trainset}.},first={overfitting},text={overfitting}}

\newglossaryentry{gdpr}{name={General Data Protection Regulation},description={The General Data Protection Regulation (GDPR) 
		is a law that has been passed by the European Union (EU) and put into effect on May 25, 2018 \url{https://gdpr.eu/tag/gdpr/}. 
		The GDPR imposes obligations onto organizations anywhere, so long as they target, collect 
		or in any other way process data related to people (i.e., personal data) in the EU.}, 
	first={general data protection regulation (GDPR) },text={GDPR}}
	
\newglossaryentry{gaussrv}{name={Gaussian random variable},description={A Gaussian \gls{rv} $\vx \in \mathbb{R}^{\nrfeatures}$ 
	with a \gls{mvndist}. The special case of $\nrfeatures$ corresponds to a scalar 
	Gaussian \gls{rv} \cite{papoulis,BertsekasProb,GrayProbBook}.},first={Gaussian RV},text={Gaussian RV}}

\newglossaryentry{trustworthiness}{name={trustworthiness},description=
	{Beside the \gls{compasp} and \gls{statasp}, a third main design aspect for 
		ML methods is their trustworthiness. The European Union has put forward seven 
		key requirements for trustworthy AI systems (that typically build on ML methods)
	\cite{ALTAIEU}: {\bf human agency and oversight}, {\bf technical robustness and safety}, 
	{\bf privacy and data governance}, {\bf transparency}, {\bf diversity non-discrimination and fairness}, 
	{\bf societal and environmental well-being}, {\bf accountability}. 
	},first={trustworthiness},text={trustworthiness}}

\newglossaryentry{sqerrloss}{name={squared error loss},description={The squared 
		error \gls{loss} measures the prediction error of a \gls{hypothesis} $\hypothesis$ 
		when predicting a numeric \gls{label} $\truelabel \in \mathbb{R}$ 
		from the \gls{feature}s $\featurevec$ of a \gls{datapoint}. It is 
	defined as 
\begin{equation} 
	\label{equ_squared_loss_gls}
	\loss{(\featurevec,\truelabel)}{\hypothesis} \defeq \big(\truelabel - \underbrace{\hypothesis(\featurevec)}_{=\predictedlabel} \big)^{2}. 
\end{equation} 
},first={squared error loss},text={squared error loss}}


\newglossaryentry{projgd}{name={projected GD},description={Projected \gls{gd} 
		extends basic \gls{gd} for unconstrained optimization to handle constraints on the 
		optimization variable (\gls{modelparams}). A single iteration of projected \gls{gd} consists 
		of first taking a \gls{gradstep} and then projecting the result back into a 
		constrain set.},first={projected \gls{gd}},text={projected \gls{gd}}}

\newglossaryentry{diffpriv}
{
	name=differential privacy,
	description={Consider an algorithm used to compute some output based on a dataset. 
		Differential privacy is a precise measure of this algorithm's privacy leakage. 
		Roughly speaking, the algorithm is differentially private if the \gls{probdist} of 
		its output does not allow it to infer if the dataset contains a specific \gls{datapoint}.}, 
	 first = {differential privacy (DP)}, text={DP} 
}




\newglossaryentry{privprot}
{
	name=privacy protection,
	description={Privacy protection aims at avoiding (or minimizing) the \gls{privleakage} occuring 
		within data processing systems (such as ML or \gls{fl} methods).}, 
	first = {privacy protection}, text={privacy protection} 
}

\newglossaryentry{privleakage}
{
	name=privacy leakage,
	description={Consider a (ML or \gls{fl}) system that processes a \gls{localdataset} $\localdataset{\nodeidx}$ 
		and shares data, such as the predictions obtained for new \gls{datapoint}s, with 
		other parties. Privacy leakage arises if the shared data carries information about a 
		private (sensitive) \gls{feature} of a \gls{datapoint} (which might be a human) of $\localdataset{\nodeidx}$.  
		The amount of privacy leakage can be measured via \gls{mutualinformation} using a 
		\gls{probmodel} for the local \gls{dataset}. 
	}, 
	first = {privacy leakage}, text={privacy leakage} 
}



\newglossaryentry{probmodel}
{
	name=probabilistic model,
	description={A probabilistic model interprets \gls{datapoint}s as \gls{realization}s of \gls{rv}s with a  
	joint \gls{probdist}.This joint \gls{probdist} typically involves parameters which have to be manually 
   chosen (=design choice) or learnt via statistical inference methods \cite{LC}. }, 
	first = {probabilistic model}, text={probabilistic model} 
}



\newglossaryentry{mean}
{
	name=mean,
	description={The expectation $\expect \{ \featurevec \}$ of a numeric \gls{rv} $\featurevec$.}, 
		first = {mean}, text={mean} 
}

\newglossaryentry{variance}
{
	name={variance},
	description={The variance of a real-valued \gls{rv} $\feature$ is defined as the expectation 
		$\expect\big\{ \big( x - \expect\{x \} \big)^{2} \big\}$ of the squared difference $\feature$ 
		and its expectation $\expect\{x \}$. We extend this definition to vector-valued \gls{rv}s $\featurevec$ 
		as $\expect\big\{ \big\| \featurevec - \expect\{\featurevec \} \big\|_{2}^{2} \big\}$.} ,first={variance},text={variance} 
}

\newglossaryentry{nn}
{
	name={nearest neighbour},
	description={Nearest neighbour methods learn a hypothesis $\hypothesis: \featurespace \rightarrow \labelspace$ whose 
		function value $\hypothesis(\featurevec)$ is solely determined by the nearest neighbours in the 
		feature space $\featurespace$ },
	first={nearest neighbour (NN)},text={NN} 
}

\newglossaryentry{neighbourhood}
{
	name={neighbourhood},
	description={The neighbourhood of a node $\nodeidx \in \nodes$ within an \gls{empgraph} are 
		those nodes $\nodeidx' \in \nodes \setminus \{ \nodeidx\}$ that are connected to $\nodeidx$ 
		by an edge with $\nodeidx$.},
	first={neighbourhood},text={neighbourhood} 
}


\newglossaryentry{neighbours}
{
	name={neighbours},
	description={The neighbours of a node $\nodeidx \in \nodes$ within an \gls{empgraph} are 
	those nodes $\nodeidx' \in \nodes$ that are connected by an edge with $\nodeidx$.},
	first={neighbours},text={neighbours} 
}

\newglossaryentry{bias}
{
	name={bias},
	description={Consider some unknown quantity $\bar{\weight}$, e.g., the true weight in a \gls{linmodel} $\truelabel = \bar{\weight} \feature + e$ 
		relating feature and label of a \gls{datapoint}. We might use an ML method (e.g., based on \gls{erm}) to 
		compute an estimate $\hat{\weight}$ for the $\bar{\weight}$ based on a set of \gls{datapoint}s that are 
		realizations of \gls{rv}s. The (squared) bias incurred by the estimate $\hat{\weight}$ is typically defined as 
		$\biasterm^{2} \defeq \big( \expect \{ \hat{\weight}  \}- \bar{\weight}\big)^{2}$. We extend this definition to 
		vector-valued quantities using the squared Euclidean norm $\biasterm^{2} \defeq \big\| \expect \{ \widehat{\weights}  \}- \overline{\weights}\big\|_{2}^{2}$.},
first={bias},text={bias} 
}

\newglossaryentry{classification}
{
	name={classification},
	description={Classification is the task of determining a discrete-valued label $\truelabel$ of a \gls{datapoint} 
		based solely on its features $\featurevec$. The label $\truelabel$ belongs to a finite set, 
		such as $\truelabel \in \{ -1,1\}$, or $\truelabel \in \{1,\ldots,19\}$ and represents a category to which the 
		corresponding \gls{datapoint} belongs to.},first={classification},text={classification} 
}




\newglossaryentry{condnr}
{
	name={condition number},
	description={The condition number $\kappa(\mathbf{Q}) \geq 1$ of a \gls{psd} matrix $\mathbf{Q}$ is 
		the ratio $\eigvalgen_{\rm max} /\eigvalgen_{\rm min}  $ between the largest $\eigvalgen_{\rm max}$ 
		and the smallest $\eigvalgen_{\rm min}$ \gls{eigenvalue} of $\mathbf{Q}$. One example for such 
	a matrix $\mQ$ is obtained from the \gls{featuremtx} $\mX$ of a \gls{dataset}, $\mQ = \mX \mX^{T}$. 
From a computational perspective, we prefer $\mQ$ to have a condition number close to $1$.},first={condition number},text={condition number} 
}

\newglossaryentry{classifier}
{
	name={classifier},
	description={A classifier is a \gls{hypothesis} (map) $\hypothesis(\featurevec)$ that is 
		used to predict a discrete-valued label. Strictly speaking, a classifier is a \gls{hypothesis} $\hypothesis(\featurevec)$ 
		that delivers values from a finite set $\labelspace$ (referred to as the \gls{labelspace}). However, we 
		are sometimes sloppy and use the term classifier also for a \gls{hypothesis} that delivers a real number 
		which is quantized, i.e., compared against a threshold, to obtain the predicted label value. For example, 
		in a binary classification problem with label values $\truelabel \in \{ -1,1\}$, we refer to a \gls{hypothesis} $\hypothesis(\featurevec)$ 
		as classifier if it is used to compute a predicted \gls{label} 
		 according to 
		 \begin{equation} 
		 	\label{equ_def_threshold_bin_classifier}
		 	\hat{\truelabel} =1   \mbox{ for } \hypothesis(\featurevec) \geq 0, \mbox{ and } 	\hat{\truelabel} =-1  \mbox{ otherwise.}
	 		\end{equation}},first={classifier},text={classifier} 
}

\newglossaryentry{emprisk}
{name={empirical risk},
  description={The empirical risk of a given hypothesis on a given set of \gls{datapoint}s 
  	is the average loss of the hypothesis computed over all \gls{datapoint}s in that set.},first={empirical risk},text={empirical risk} 
}

\newglossaryentry{nodedegree}
{name={node degree},
	description={The degree of a node $\nodeidx$ in an undirected \gls{graph} is 
		the number of its neighbours.},first={node degree},text={node degree} 
}

\newglossaryentry{graph}
{name={graph},
	description={A graph $\graph = \pair{\nodes}{\edges}$ is a pair that consists of a node set $\nodes$ 
		and an edge set $\edges$. In general, a graph is specified by a map that assigns to 
		each edge $\edgeidx \in \edges$ a pair of nodes \cite{RockNetworks}. One important family of 
		graphs (simple undirected graphs) is obtained by identifying each edge $\edgeidx \in \edges$ 
		with two different nodes $\{\nodeidx,\nodeidx'\}$. Weighted graphs also specify numeric 
	   weights $\edgeweight_{\edgeidx}$ for each edge $\edgeidx \in \edges$.},first={empirical graph},text={empirical graph} 
}

\newglossaryentry{empgraph}
{name={empirical graph},
	description={Empirical graphs represent collections of local \gls{dataset}s and corresponding \gls{localmodel}s \cite{SemiSupervisedBook}. 
		An empirical graph is an undirected weighted \gls{graph} whose nodes carry \gls{localdataset}s and 
		\gls{model}s. \Gls{fl} methods learn a local \gls{hypothesis} $\localhypothesis{\nodeidx}$, for each node $\nodeidx \in \nodes$, 
		such that it incurs small \gls{loss} on the \gls{localdataset}s.},first={empirical graph},text={empirical graph} 
}

\newglossaryentry{norm}
{name={norm},
	description={A norm is a function that maps each element (vector) of a linear vectorspace to 
	a non-negative number. This function must be homogeneous, definite and satisfy the triangle inequality. },
	first={norm},text={norm} 
}

\newglossaryentry{explanation}
{name={explanation},
	description={Some information that is provided along with the output of an AI system. 
		The form of an explanation can vary significantly. An explanation could be a natural text 
		or a quantitive importance measure provided for the \gls{feature}s of a \gls{datapoint}. 
		We can also use visual forms of explanations such as intensity plots for image classification.},
	first={explanation},text={explanation} 
}

\newglossaryentry{risk}
{name={risk},
	description={Consider a hypothesis $\hypothesis$ that is used to predict the \gls{label} 
		$\truelabel$ of a \gls{datapoint} based on its \gls{feature}s $\featurevec$. We measure 
		the quality of a particular \gls{prediction} using a \gls{lossfunc} $\loss{(\featurevec,\truelabel)}{\hypothesis}$. 
		If we interpret \gls{datapoint}s as the \gls{realization}s of \gls{iid} \gls{rv}s, 
		also the $\loss{(\featurevec,\truelabel)}{\hypothesis}$ becomes the \gls{realization} 
		of a \gls{rv}. Using such an \gls{iidasspt} allows to define the risk of a \gls{hypothesis} 
		as the expected \gls{loss} $\expect \big\{\loss{(\featurevec,\truelabel)}{h} \big\}$. 
		Note that the risk of $\hypothesis$ depends on both, the specific choice for the \gls{lossfunc} and the 
		\gls{probdist} of the \gls{datapoint}s.},
	first={risk},text={risk} 
}

\newglossaryentry{actfun}
{name={activation function},
	description={Each artificial neuron within an \gls{ann} is assigned an activation function $g(\cdot)$ 
		that maps a weighted combination of the neuron inputs $\feature_{1},\ldots,\feature_{\nrfeatures}$ 
		to a single output value $a = g\big(\weight_{1} \feature_{1}+\ldots+\weight_{\nrfeatures} \feature_{\nrfeatures} \big)$. 
		Note that each neuron is parametrized by the weights $\weight_{1},\ldots,\weight_{\nrfeatures}$.},
first={activation function},text={activation function} 
}




\newglossaryentry{transparency}
{name={transparency},
	description={One of the key requirements for trustworthy AI is their transparency \cite{HLEGTrustworhtyAI}. 
		Transparency is to enable a person to utilise their right to take action where they 
		believe they have been treated wrongly. This is closely related to the right to 
		data protection. In order to take steps against a potentially unlawful processing or 
		an unjustified outcome of an \gls{erm}-based AI system, one has to have enough 
		information to understand how processing has taken place or how a decision was 
		reached.},
	first={transparency},text={transparency} 
}


\newglossaryentry{sensattr}
{name={sensitive attribute},
	description={ML revolves around learning a \gls{hypothesis} map that allows 
		to predict the \gls{label} of a \gls{datapoint} from its \gls{feature}s. In some 
		applications we must ensure that the output delivered by an ML system does 
		not allow to infer sensitive attributes of a \gls{datapoint}. Which parts of a \gls{datapoint} 
		is considered as a sensitive attribute is a design choice that varies across different application domains.},
	first={sensitive attribute},text={sensitive attribute} 
}


\newglossaryentry{sbm}
{name={stochastic block model},
	description={The stochastic block model (SBM) is a (family) probabilistic generative model for an undirected graph $\graph = \big( \nodes, \edges \big)$ 
		with given nodeset $\nodes$. In its most basic forms, the SBM amounts to generating a graph by first randomly assigning labels $c_{i} \in \{1,\ldots,\nrcluster\}$ 
		to each node $i \in \nodes$ of the graph. A pair of different nodes in the graph is connected by edge with probabailiy $p_{i,j}$ that 
	depends solely on the labels $c_{i}, c_{j}$.},
	first={stochastic block model (SBM)},text={SBM} 
}

\newglossaryentry{deepnet}
{name={deep net},
	description={We refer to an \gls{ann} with a (relatively) large number of hidden layers as a deep \gls{ann} or ``deep net''. Deep nets 
	are used to represent the \gls{hypospace}s of deep learning methods \cite{Goodfellow-et-al-2016}.},
	first={deep \gls{ann} (deep net)},text={deep net} 
}

\newglossaryentry{baseline}
{name={baseline},
	description={A reference value or benchmark for the average loss incurred by a hypothesis when applied to the \gls{datapoint}s 
		generated in a specific ML application. Such a reference value might be obtained from human performance (e.g., error rate 
		of dermatologists diagnosing cancer from visual inspection of skin areas) or other ML methods (``competitors'')}, 
	first={baseline},text={baseline} 
}


\newglossaryentry{spectogram}
{name={spectogram},
	description={The spectogram of a time signal, e.g., an audio recording, characterizes the 
	time-frequency distribution of the signal. Loosely speaking, the spectogram quantities the 
	signal strength at a specific time and frequency.}, 
	first={spectogram},text={spectrogram} 
}

\newglossaryentry{specclustering}
{name={spectral clustering},
	description={Spectral clustering groups the nodes of an undirected graph by applying 
		\gls{kmeans} clustering to node-wise feature vectors. These feature vectors are built 
		from the \gls{eigenvector}s of the graph Laplacian matrix \cite{Luxburg2007,FlowSpecClustering2021}. }, 
	first={spectral clustering},text={spectral clustering} 
}

\newglossaryentry{flowbasedclustering}
{name={flow-based clustering},
	description={Flow-basted clustering groups the nodes of an undirected graph by applying 
		\gls{kmeans} clustering to node-wise feature vectors. These feature vectors are built 
		from flows between carefully selected source and destination nodes \cite{FlowSpecClustering2021}. }, 
	first={flow-based clustering},text={flow-based clustering} 
}



\newglossaryentry{esterr}
{name={estimation error},
	description={Consider \gls{datapoint}s with feature vectors $\featurevec$ and \gls{label} 
		$\truelabel$. In some applications we can model the relation between features and label 
		of a \gls{datapoint} as $\truelabel = \bar{\hypothesis}(\featurevec) + \varepsilon$. Here we 
		used some true hypothesis $\bar{h}$ and a noise term $\varepsilon$ which might represent 
		modelling or labelling errors. The estimation error incurred by a ML method that learns a 
		\gls{hypothesis} $\widehat{\hypothesis}$, e.g., using \gls{erm}, is defined as $\widehat{\hypothesis} - \bar{\hypothesis}$. 
		For a parametrized hypothesis space, consisting of hypothesis maps that are determined by 
		a parameter vector $\weights$, we define the estimation error in terms of parameter vectors 
		as $\Delta \weights = \widehat{\weights} - \overline{\weights}$.}
	first={estimation error},text={estimation error} 
}


\newglossaryentry{dob}
{name={degree of belonging},
	description={A number that indicates the extend by which a \gls{datapoint} belongs to a \gls{cluster}. 
	The degree of belonging can be interpreted as a soft \gls{cluster} assignment. Soft clustering methods 
   typically represent the degree of belonging by a real number in the interval $[0,1]$. The boundary values 
   $0$ and $1$ correspond to hard cluster assignments.}, first={degree of belonging},text={degree of belonging} 
}

\newglossaryentry{msee}
{name={mean squared estimation error},
	description={Consider a ML method that uses a parametrized \gls{model}. For a given \gls{trainset}, 
		whose \gls{datapoint}s are interpreted as realizations of \gls{rv}s, the ML method learns \gls{modelparams} 
		incurring the \gls{esterr} $\Delta \weights$. The mean squared estimation error is defined as the 
		expectation $\expect \big\{ \big\| \Delta \weights \big\|^{2} \big\}$ of the squared Euclidean norm of the \gls{esterr}.},
	first={mean squared estimation error (MSEE)},text={MSEE} 
}

\newglossaryentry{gtvmin}
{name={GTV minimization},
	description={GTV minimization is an instance of \gls{rerm} using the \gls{gtv} of local \gls{modelparams} 
		as a \gls{regularizer}.},
	first={GTV minimization (GTVMin)},text={GTVMin} 
}

\newglossaryentry{regression}
{name={regression},
	description={Regression problems revolve around the problem of predicting a numeric \gls{label} solely 
		from the \gls{feature}s of a \gls{datapoint}.},
	first={regression},text={regression} 
}

\newglossaryentry{acc}
{name={accuracy},
	description={Consider \gls{datapoint}s characterized by \gls{feature}s $\featurevec \in \featurespace$ and 
		a categorical label $\truelabel$ which takes on values from a finite \gls{labelspace} $\labelspace$. The 
		accuracy of a \gls{hypothesis} $\hypothesis: \featurespace \rightarrow \labelspace$, when applied 
		to the \gls{datapoint}s in a \gls{dataset} $\dataset = \big\{ \big(\featurevec^{(1)}, \truelabel^{(1)} \big), \ldots, \big(\featurevec^{(\samplesize)},\truelabel^{(\samplesize)}\big) \big\}$ 
		is then defined as $1 - (1/\samplesize)\sum_{\sampleidx=1}^{\samplesize} \loss{\big(\featurevec^{(\sampleidx)},\truelabel^{(\sampleidx)}\big)}{\hypothesis}$ using the \gls{zerooneloss}.},
	first={accuracy},text={accuracy} 
}



\newglossaryentry{expert}
{name={expert},
	description={ML aims at learning a \gls{hypothesis} $\hypothesis$ that accurately predicts the label 
		of a \gls{datapoint} based on its features. We measure the prediction error using 
		some \gls{lossfunc}. Ideally we want to find a \gls{hypothesis} that incurs minimum loss. 
		One approach to make this goal precise is to use the \gls{iidasspt} and use the resulting 
		\gls{bayesrisk} as the benchmark level for the (average) \gls{loss} of a \gls{hypothesis}. 
		Alternatively, we might know a reference or benchmark \gls{hypothesis} $\hypothesis'$ 
		which might be obtained by some existing ML method. We can then compare the \gls{loss} 
		incurred by $\hypothesis$ against the \gls{loss} incurred by $\hypothesis'$. Such a reference 
		or baseline hypothesis $\hypothesis'$ is referred to as an \gls{expert}. 
		Note that an expert might deliver very poor predictions. We typically compare against many 
	   different experts and aim at incurring not much more \gls{loss} than the best among those experts (this is 
	   known as regret minimization) \cite{PredictionLearningGames,HazanOCO}.}
	first={expert},text={expert} 
}


%\newglossaryentry{zerooneloss}
%{name={$0/1$ loss},
%	description={Consider \gls{datapoint}s characterized by a $\label \in \labelspace$ whose value 
%	belongs to a finte \gls{labelspace} $\labelspace$. We try to predict the \gls{label} of a \gls{datapoint} 
%	from its \gls{feature}s using a \gls{hypothesis} $\hypothesis(\featurevec)$ to compute a predicted \gls{label} 
%	$\widehat{\truelabel}$. The $0/1$ \gls{loss} incurred by the $\hypothesis$ is equal 
%	to $0$ if $\widehat{\truelabel} = \truelabel$ and equal to $1$ otherwise.}, first={$0/1$ loss},text={$0/1$ loss} 
%}


\newglossaryentry{nfl}
{name={networked federated learning},
	description={Networked federated learning refers to methods that learn personalized models 
		in a distributed fashion from local datasets that are related by an intrinsic network structure.},
 first={networked federated learning (NFL)},text={NFL} 
}




\newglossaryentry{regret}
{name={regret},
	description={The regret of a hypothesis $\hypothesis$ relative to another hypothesis $\hypothesis'$, which 
		       serves as a reference (or baseline), 
		      is the difference between the \gls{loss} incurred by $\hypothesis$ and the \gls{loss} incurred by $\hypothesis'$ \cite{PredictionLearningGames}. 
		      The baseline hypothesis $\hypothesis'$ is also referred to as an \gls{expert}.},
	first={regret},text={regret} 
}

\newglossaryentry{strcvx}
{name={strongly convex},
	description={A continuously \gls{differentiable} real-valued function $f(\featurevec)$ is strongly 
		convex with coefficient $\sigma$ if $f(\vy) \geq f(\vx) + \nabla f(\vx)^{T} (\vy - \vx) + (\sigma/2) \normgeneric{\vy - \vx}{2}^{2}$ \cite{nesterov04},\cite[Sec. B.1.1.]{CvxAlgBertsekas}.},
	first={strongly convex},text={strongly convex} 
}

\newglossaryentry{differentiable}
{name={differentiable},
	description={A function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}$  is differentiable if it 
		has a \gls{gradient} $\nabla f ( \mathbf{x})$ everywhere (for every $\mathbf{x} \in \mathbb{R}^{\featuredim}$) \cite{RudinBookPrinciplesMatheAnalysis}.},
	first={differentiable},text={differentiable} 
}

\newglossaryentry{gradient}
{name={gradient},
	description={For a real-valued function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}: \weights \mapsto f(\weights)$, 
	a vector $\vg$ such that $\lim_{\weights \rightarrow \weights'} \frac{f(\weights) - \big(f(\weights')+ \vg^{T} (\weights- \weights') \big) }{\| \weights-\weights'\|}=0$ 
	is referred to as the gradient of $f$ at $\weights'$. If such a vector exists it is denoted $\nabla f(\weights')$ or $\nabla f(\weights)\big|_{\weights'}$ \cite{RudinBookPrinciplesMatheAnalysis}.},
	first={gradient},text={gradient} 
}

\newglossaryentry{subgradient}
{name={subgradient},
description={For a real-valued function $f: \mathbb{R}^{\featuredim} \rightarrow \mathbb{R}: \weights \mapsto f(\weights)$, 
		a vector $\va$ such that $f(\weights) \geq  f(\weights') +\big(\weights-\weights' \big)^{T} \va$ is 
		referred to as a subgradient of $f$ at $\weights'$ \cite{BertCvxAnalOpt,BertsekasNonLinProgr}.},
	first={subgradient},text={subgradient} 
}

\newglossaryentry{fedavg}
{name={federated averaging (FedAvg)},
	description={Federated averaging is an iterative \gls{fl} algorithm that alternates between local model trainings and 
	averaging the resulting local model parameters. Different variants of this algorithm are obtained 
	by different techniques for the model training. The authors of \cite{pmlr-v54-mcmahan17a} consider 
	federated averaging methods where the local model training is implemented by running several \gls{gd} steps }, first = {federated averaging (FedAvg)}, text={FedAvg} 
}

\newglossaryentry{relu}
{name={rectified linear unig (ReLU)},
	description={The rectified linear unit or ``ReLU'' is a popular choice for the \gls{actfun} of a neuron within an \gls{ann}. 
	It is defined as $g(z) = \max\{0,z\}$ with $z$ being the weighted input of the neuron.}, first = {rectified linear unit (ReLU)}, text={ReLU} 
}

\newglossaryentry{hypothesis}
{name={hypothesis},
	description={A map (or function) $h: \featurespace \rightarrow \labelspace$ from the 
		feature space $\featurespace$ to the label space $\labelspace$. 
		Given a \gls{datapoint} with features $\featurevec$ we use a hypothesis map $h$
		to estimate (or approximate) the label $\truelabel$ using the predicted label 
		$\hat{\truelabel} = h(\featurevec)$. ML is about learning (or finding) a hypothesis map $h$
		such that $\truelabel \approx h(\featurevec)$ for any \gls{datapoint}.},
	first={hypothesis},text={hypothesis}  
}



\newglossaryentry{vcdim}
{name={Vapnik–Chervonenkis (VC) dimension},
	description={The VC dimension of an infinite \gls{hypospace} is a widely-used measure 
		for its size. We refer to \cite{ShalevMLBook} for a precise definition of VC dimension 
		as well as a discussion of its basic properties and use in ML.},
	first={Vapnik–Chervonenkis (VC) dimension},text={VC dimension}  
}

\newglossaryentry{effdim}
{name={effective dimension},
	description={The effective dimension $\effdim{\hypospace}$ of an infinite \gls{hypospace} $\hypospace$ 
		is a measure of its size. Loosely speaking, the effective dimension is equal to the number 
		of ``independent'' tunable parameters of the model. These parameters might be the coefficients  
		used in a linear map or the weights and bias terms of an \gls{ann}.},
	first={effective dimension},text={effective dimension}  
}

\newglossaryentry{labelspace}
{name={label space},
	description={Consider a ML application that involves \gls{datapoint}s characterized by features 
		and labels. The \gls{label} space is constituted by all potential values that the \gls{label} 
		of a \gls{datapoint} can take on. Regression methods, aiming at predicting numeric \gls{label}s, often
 use the \gls{label} space $\labelspace = \mathbb{R}$. Binary classification methods use a label space 
		 that consists of two different elements, e.g., $\labelspace =\{-1,1\}$, $\labelspace=\{0,1\}$ 
		or $\labelspace = \{ \mbox{``cat image''}, \mbox{``no cat image''} \}$  }, first={label space},text={label space}  
}

\newglossaryentry{prediction}
{name={prediction},
	description={A prediction is an estimate or approximation for some quantity of interest. ML 
		revolves around learning or finding a \gls{hypothesis} map $\hypothesis$ that reads in the 
		\gls{feature}s $\featurevec$ of a \gls{datapoint} and delivers a prediction $\widehat{\truelabel} \defeq \hypothesis(\featurevec)$ 
		for its \gls{label} $\truelabel$. },
	first={prediction},text={prediction}  
}


\newglossaryentry{histogram}
{name={histogram},
	description={Consider a \gls{dataset} $\dataset$ that consists of $\samplesize$ \gls{datapoint}s 
		$\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}$ that belong to some cell $[-U,U] \times \ldots \times [-U,U] \subseteq \mathbb{R}^{\featuredim}$
		with side length $U$. We partition this cell evenly into smaller elementary cells with side 
		length $\Delta$. The histogram of $\dataset$ assigns each elementary cell to the corresponding 
		fraction of \gls{datapoint}s in $\dataset$ that fall into this elementary cell. 
	},
	first={histogram},text={histogram}  
}

\newglossaryentry{bootstrap}
{name={bootstrap},
	description={Consider a probabilistic model that interprets a given set of \gls{datapoint}s $\dataset = \big\{ \datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}\big\}$ as realizations of \gls{iid} \gls{rv}s with a common \gls{probdist} $p(\datapoint)$. The bootstrap 
	uses the histogram of $\dataset$ as the underlying \gls{probdist} $p(\datapoint)$. 
	},
	first={bootstrap},text={bootstrap}  
}

\newglossaryentry{featurespace}
{name={feature space},
	description={
		The feature space of a given ML application or method is constituted by all potential 
		values that the feature vector of a \gls{datapoint} can take on. Within this book the most 
		frequently used choice for the feature space is the \gls{euclidspace} $\mathbb{R}^{\featuredim}$ 
		with dimension $\featurelen$ being the number of individual features of a \gls{datapoint}.},
	first={feature space},text={feature space}  
}


\newglossaryentry{missingdata}
{name={missing data},
	description={By missing data, we refer to a situation where some feature values of a 
		subset of \gls{datapoint}s are unknown. Data imputation techniaues aim at estimating 
		(predicting) these missing feature values \cite{Abayomi2008DiagnosticsFM}. },
	first={missing data},text={missing data}  
}


\newglossaryentry{psd}
{name={positive semi-definite},
	description={A symmetric matrix $\mQ = \mQ^{T} \in \mathbb{R}^{\featuredim \times \featuredim}$ 
		is referred to as positive semi-definite if $\featurevec^{T} \mQ \featurevec \geq 0$ for every 
		vector $\featurevec \in \mathbb{R}^{\featuredim}$.},
	first={positive semi-definite (psd)},text={psd}  
}

\newglossaryentry{feature}
{name={feature},
	description={A feature of a \gls{datapoint} is one of its properties that can be measured or computed in an 
		automated fashion. For example, if a \gls{datapoint} is a bitmap image, then we could use 
		the red-green-blue intensities of its pixels as features. Some widely used synonyms for 
		the term feature are ``covariate'',``explanatory variable'', ``independent variable'', ``input (variable)'', ``predictor (variable)'' or ``regressor''  \cite{Gujarati2021,Dodge2003,Everitt2022}. However, this book makes consequent use of the term 
		features for low-level properties of \gls{datapoint}s that can be measured easily.}, first={feature},text={feature}  
}

\newglossaryentry{label}
{name={label},
	description={A higher-level fact or quantity of interest associated with a \gls{datapoint}. 
		For example, if the \gls{datapoint} is an image, the label could indicate whether the 
		image contains a cat or not. Synonyms for label, commonly used in specific domains, 
		include \emph{response variable}, \emph{output variable}, and \emph{target} \cite{Gujarati2021,Dodge2003,Everitt2022}.
 },
	first={label},text={label}  
}


\newglossaryentry{noniid}
{name={non-i.i.d.},
	description={See \gls{noniiddata}.},first={non-i.i.d.},text={non-i.i.d.}  
}

\newglossaryentry{data}
{name={data},
	 description={See \gls{dataset}.},
	text={data}
}

\newglossaryentry{dataset}
{name={dataset},
	description={With a slight abuse of notation we use the terms ``dataset`` or ``set of \gls{datapoint}s'' to 
		refer to an indexed list of \gls{datapoint}s $\datapoint^{(1)},\datapoint^{(2)},\ldots$. Thus, there is a first \gls{datapoint} 
		$\datapoint^{(1)}$, a second \gls{datapoint} $\datapoint^{(2)}$ and so on. Strictly speaking a dataset is a list 
		and not a set \cite{HalmosSet}. By using indexed lists of \gls{datapoint}s we avoid some of the challenges 
		arising in concept of an abstract set.},first={dataset},text={dataset}  
}

\newglossaryentry{predictor}
{name={predictor},
	description={A predictor is a \gls{hypothesis} whose function values are numeric, such as real numbers. 
		Given a \gls{datapoint} with features $\featurevec$, the predictor value $h(\featurevec) \in \mathbb{R}$ 
		is used as a prediction (estimate/guess/approximation) for the true numeric label $\truelabel \in \mathbb{R}$ of the \gls{datapoint}. },first={predictor},text={predictor}  
}

\newglossaryentry{labeled datapoint}
{name={labeled datapoint},
 description={A \gls{datapoint} whose label is known or has been determined by some means (might require human experts).},
 first={labeled datapoint},text={labeled datapoint}  
}

\newglossaryentry{rv}
{name={random variable (RV)},
 description={A random variable is a mapping from a probability space $\mathcal{P}$ to a value space \cite{BillingsleyProbMeasure}. 
 	The probability space, whose elements are elementary events, is equipped with a probability 
 	 measure that assigns a probability to subsets of $\mathcal{P}$. A binary random variable maps elementary events 
 	to a set containing two different values, e.g., $\{-1,1\}$ or $\{ \mbox{cat}, \mbox{no cat} \}$. 
 	A real-valued random variable maps elementary events to real numbers $\mathbb{R}$. 
 	A vector-valued random variable maps elementary events to the \gls{euclidspace} $\mathbb{R}^{\featuredim}$. 
 	Probability theory uses the concept of measurable spaces to rigorously define and study the properties of (large) 
 	collections of random variables \cite{GrayProbBook,BillingsleyProbMeasure}.}, first={RV},text={RV}  }
 
	
\newglossaryentry{realization}
{name={realization},
	description={Consider a \gls{rv} $x$ which maps each element (outcome, or elementary event) $\omega \in \mathcal{P}$ of a 
		probability space $\mathcal{P}$ to an element $a$ of a measurable space $\mathcal{N}$ \cite{BillingsleyProbMeasure,RudinBookPrinciplesMatheAnalysis,HalmosMeasure}. 
		A realization of $x$ is any element $a' \in \mathcal{N}$ such that there is 
		an element $\omega' \in \mathcal{P}$ with $x(\omega') = a'$.  }, first={realization},text={realization}  }

\newglossaryentry{trainset}
{name={training set},
description={A set of data points that is used in \gls{erm} to learn a \gls{hypothesis} $\learnthypothesis$. 
	The average \gls{loss} of $\learnthypothesis$ on the training set is referred to as the \gls{trainerr}. 
	The comparison between \gls{trainerr} and \gls{valerr} of $\learnthypothesis$ allows to diagnose ML 
	methods and informs how to improve them (e.g., using a different \gls{hypospace} or collecting more \gls{datapoint}s).},first={training set},text={training set}  
}

\newglossaryentry{netmodel}
{name={networked model},
  description={A networked model over an \gls{empgraph} $\graph = \pair{\nodes}{\edges}$ assigns 
   a \gls{localmodel} (\gls{hypospace}) to each node $\nodeidx \in \nodes$ of the \gls{empgraph} $\graph$.}, 
   first={networked model},text={networked model}  
}

\newglossaryentry{batch}
{
	name={batch},
	description={A set of randomly selected \gls{datapoint}s out of a (typically very large) \gls{dataset}.}, 
	first={batch},text={batch}  
}

\newglossaryentry{netdata}
{
	name={networked data},
	description={Networked data consists of \gls{localdataset}s that are related by some notion of pair-wise 
		similarity. We represent networked data using an \gls{empgraph} whose nodes carry \gls{localdataset}s 
		and an edge indicates a similarity between the connected nodes.}, 
	first={networked data},text={networked data}  
}

\newglossaryentry{trainerr}
{
	name={training error},
	description={The average \gls{loss} of a \gls{hypothesis} when predicting the \gls{label}s of \gls{datapoint}s in a \gls{trainset}. 
		We sometimes refer by training error also the minimum average \gls{loss} incurred on the \gls{trainset} 
		by any \gls{hypothesis} out of a \gls{hypospace}.},first={training error},text={training error}  
}

\newglossaryentry{datapoint}
{
	name={data point},
	description={A \gls{datapoint} is any object that conveys information \cite{coverthomas}. Data points might be 
		students, radio signals, trees, forests, images, \gls{rv}s, real numbers or proteins. We characterize data points 
		using two types of properties. One type of property is referred to as a feature. \Gls{feature}s are properties of a 
		\gls{datapoint} that can be measured or computed in an automated fashion. Another type of property is 
		referred to as \gls{label}s. The \gls{label} of a \gls{datapoint} represents some higher-level fact (or quantity of 
		interest). In contrast to \gls{feature}s, determining the \gls{label} of a \gls{datapoint} typically requires human 
		experts (domain experts). Roughly speaking, ML aims at predicting the \gls{label} of a \gls{datapoint} based 
		solely on its \gls{feature}s.}, first={data point},text={data point}  
}


\newglossaryentry{valerr}
{name={validation error},
 description={Consider a hypothesis $\widehat{h}$ which is obtained by \gls{erm} on a \gls{trainset}. The 
 average loss of $\widehat{h}$ on a \gls{valset}, which is different from the \gls{trainset}, is referred to as 
 the validation error.},first={validation error},text={validation error}  
}

\newglossaryentry{validation}
{name={validation},
	description={Consider a \gls{hypothesis} $\learnthypothesis$ that has been 
		learn via \gls{erm} on some \gls{trainset} $\dataset$. Validation refers to the practice 
		of trying out a \gls{hypothesis} $\learnthypothesis$ on a \gls{valset} that consists of 
		\gls{datapoint}s that are not contained in the \gls{trainset} $\dataset$. },first={validation},text={validation}  
}

\newglossaryentry{quadfunc}
{name={quadratic function},
	description={A quadratic function $f(\weights)$, reading in a vector $\weights \in \mathbb{R}^{\nrfeatures}$ as 
		its argument, is such that $$f(\weights) =  \weights^{T} \mathbf{Q} \mathbf{w} + \mathbf{q}^{T} \weights+a,$$
	with some matrix $\mQ \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$, vector $\vq \in \mathbb{R}^{\nrfeatures}$ 
	and scalar $a \in \mathbb{R}$.  },first={quadratic function},text={quadratic function}  
}

\newglossaryentry{valset}
{name={validation set},
  description={A set of \gls{datapoint}s that have not been used as \gls{trainset} in \gls{erm} to learn 
  	a \gls{hypothesis} $\widehat{\hypothesis}$. The average \gls{loss} of $\widehat{h}$ on the validation set 
  	is referred to as the validation error and used to diagnose the ML method (see \cite[Sec. 6.6.]{MLBasics}). 
  	The comparison between \gls{trainerr} and \gls{valerr} can inform directions for improvements 
  	of the ML method (such as using a different \gls{hypospace}).},first={validation set},text={validation set}  
}

\newglossaryentry{testset}
{name={test set},
	description={A set of \gls{datapoint}s that have neither been used in a \gls{trainset} to learn parameters of a model 
		nor in a \gls{valset} to choose between different models (by comparing validation errors).},first={test set},text={test set}  
}

\newglossaryentry{linclass}{name={linear classifier}, description={A classifier $\hypothesis(\featurevec)$ 
		maps the \gls{feature} vector $\featurevec \in \mathbb{R}^{\featuredim}$ of a \gls{datapoint} to a 
		predicted label $\hat{\truelabel} \in \labelspace$ out of a finite set of label values $\labelspace$. 
		We can characterize such a classifier equivalently by the \gls{decisionregion}s $\decreg{a}$, for 
		every possible \gls{label} value $a \in \labelspace$. Linear classifiers are such that the boundaries 
		between the regions $\decreg{a}$ are hyperplanes in the \gls{euclidspace} $\mathbb{R}^{\featuredim}$.  },first={linear classifier},text={linear classifier} }

\newglossaryentry{erm}{name={empirical risk minimization}, description={Empirical risk minimization is the 
		optimization problem of finding the hypothesis with minimum average \gls{loss} (or \gls{emprisk}) on 
		a given set of \gls{datapoint}s (the \gls{trainset}). Many ML methods are special cases of \gls{emprisk}.},
	first={empirical risk minimization (ERM)},text={ERM} }

\newglossaryentry{multilabelclass}{name={multi-label classification}, description={Multi-label classification 
		problems and methods involve \gls{datapoint}s that are characterized by several individual labels.},
	    first={multi-label classification},text={multi-label classification} }


\newglossaryentry{ssl}{name={semi-supervised learning}, description={Semi-supervised learning methods 
		use (large amounts of) unlabeled \gls{datapoint}s to support the learning of a \gls{hypothesis} 
		from (a small number of) labeled \gls{datapoint}s \cite{SemiSupervisedBook}. },first={semi-supervised learning (SSL)},text={SSL} }
	
	
\newglossaryentry{objfunc}{name={objective function}, description={An objective function is a map that assigns each possible 
		value of an optimization variable, such as the parameters $\weights$ of a \gls{hypothesis} $\hypothesis^{(\weights)}$, to 
		an objective value $f(\weights)$. The objective value $f(\weights)$ could be the 
		\gls{risk} or the \gls{emprisk} of a \gls{hypothesis} $\hypothesis^{(\weights)}$.},first={objective function},text={objective function} }
	
\newglossaryentry{regularizer}{name={regularizer}, description={A regularizer assigns each \gls{hypothesis} $\hypothesis$ from 
		a \gls{hypospace} $\hypospace$ a quantitative measure $\regularizer{\hypothesis}$ for how much its prediction error on a \gls{trainset} 
		might differ from its prediction errors on \gls{datapoint}s outside the \gls{trainset}. \Gls{ridgeregression} uses the regularizer 
		$\regularizer{\hypothesis} \defeq \normgeneric{\weights}{2}^{2}$ for linear \gls{hypothesis} maps $\hypothesis^{(\weights)}(\featurevec) \defeq \weights^{T} \featurevec$ \cite[Ch. 3]{MLBasics}. The \gls{lasso} uses the regularizer 
		$\regularizer{\hypothesis} \defeq \normgeneric{\weights}{1}$ for linear \gls{hypothesis} maps $\hypothesis^{(\weights)}(\featurevec) \defeq \weights^{T} \featurevec$ \cite[Ch. 3]{MLBasics}. },first={regularizer},text={regularizer} }


\newglossaryentry{regularization}{name={regularization}, description={Regularization techniques modify the \gls{erm} 
		principle such that the learnt \gls{hypothesis} performs well (generalizes) beyond the \gls{trainset}.
		One specific implementation of \gls{regularization} is to add a penalty or regularization term to the 
		objective function of \gls{erm} (which is the average \gls{loss} on the \gls{trainset}). This regularization 
		term can be interpreted as an estimate for the increase in the expected \gls{loss} (\gls{risk}) compared to the 
		average \gls{loss} on the \gls{trainset}. },first={regularization},text={regularization} }

\newglossaryentry{rerm}{name={regularized empirical risk minimization}, description={Synonym for \gls{srm}.},
	first={regularized empirical risk minimization (RERM)},text={RERM} }
	
\newglossaryentry{gtv}{name={generalized total variation}, description={Generalized total variation measures the changes of 
	vector-valued node attributes of a graph.},first={generalized total variation (GTV)},text={GTV} }
	
\newglossaryentry{srm}{name={structural risk minimization}, description={Structural risk minimization is the problem 
		of finding the hypothesis that optimally balances the average \gls{loss} (or \gls{emprisk}) on 
		a \gls{trainset} with a \gls{regularization} term. The \gls{regularization} term penalizes a \gls{hypothesis}
		 that is not robust against (small) perturbations of the \gls{datapoint}s in the \gls{trainset}.},first={structural risk minimization (SRM)},text={SRM} }

\newglossaryentry{datapoisoning}{name={data poisoning}, description={\gls{fl} methods allow to leverage 
		the information contained in \gls{localdataset}s generated by other parties to improve the training of 
		a tailored \gls{model}. Depending on how much we trust the other parties, \gls{fl} can be compromised 
		by data poisoning. Data poisoning refers to the intentional manipulation (or fabrication) of \gls{localdataset}s to 
		steer the training of a specific \gls{localmodel} \cite{Liu2021,PoisonGAN}.},first={data poisoning},text={data poisoning} }
	
	
\newglossaryentry{backdoor}{name={backdoor}, description={A backdoor attack refers 
		to the intentional manipulation of the training process underlying a ML method. The manipulation 
		can be implemented by perturbing the \gls{trainset} (data poisoning) or optimization algorithm 
		used by an \gls{erm} based method. The goal of a backdoor attack is to nudge the learnt \gls{hypothesis} 
		towards specific predictions for a certain range of \gls{feature} values. This range of \gls{feature} 
		values serves as a key (or trigger) to unlock a ``backdoor'' in the sense of delivering anomolous  
		\gls{prediction}s. These anomouls predictions are known to the attacker but cannot 
		be inferred (easily) from the clean \gls{trainset} or optimization algorithm.},
	first={backdoor},text={backdoor} }


\newglossaryentry{clustasspt}{name={clustering assumption}, description={The clustering 
		assumption postulates that \gls{datapoint}s in a dataset form a (small) number of groups or clusters. 
	    \Gls{datapoint}s in the same cluster are more similar with each other than with those outside the cluster \cite{SemiSupervisedBook}. 
	    We obtain different clustering methods by using different notions of similarity between \gls{datapoint}s.},first={clustering assumption},text={clustering assumption} }
	
\newglossaryentry{dosattack}{name={denial-of-service attack}, description={A denial-of-service attack uses \gls{datapoisoning} 
		to steer the training of a local (client) model such that it performs poorly for typical \gls{datapoint}s},
	first={denial-of-service attack},text={denial-of-service attack} }

\newglossaryentry{netexpfam}{name={networked exponential families}, description={A networked collection of 
		exponential families having a separaate parameter vector for each node of the network. These parameter 
		vectors are coupled via the network structure. },first={networked exponential family (nExpFam)},text={nExpFam} }
	 


\newglossaryentry{scatterplot}{name={scatterplot}, description={A visualization technique that depicts data points by markers in a 
	two-dimensional plane.},first={scatterplot},text={scatterplot} }


\newglossaryentry{stepsize}{name={step size}, description={
		Many ML methods use iterative optimization methods (such as \gls{gdmethods}) 
		to construct a sequence of increasingly accurate hypothesis 
		maps $h^{(1)},h^{(2)},\ldots$. The $\itercntr$th iteration of such an algorithm starts from the current 
		hypothesis $h^{(\itercntr)}$ and tries to modify it to obtain an improved hypothesis $h^{(\itercntr+1)}$. 
		Iterative algorithms often use a step size (hyper-) parameter. The step size controls the amount by 
		which a single iteration can change or modify the current hypothesis. Since the overall goal of such 
		iteration ML methods is to learn a (approximately) optimal hypothesis we refer to a step size parameter 
		also as a \gls{learnrate}.}, 
	first={step size},text={step size} }

\newglossaryentry{learnrate}{name={learning rate}, description={Consider an iterative method for finding or learning 
				a good choice for a hypothesis. Such an iterative method repeats similar computational (update) steps that adjust 
				or modify the current choice for the hypothesis to obtain an improved hypothesis. A prime example for such an 
				iterative learning method is \gls{gd} and its variants. We refer by learning rate to any parameter 
				of an iterative learning method that controls the extent by which the current \gls{hypothesis} 
				might be modified or improved in each iteration. A prime example for such a parameter is the 
				step size used in \gls{gd}. Some authors use the term learning rate mostly as a synonym for the 
				step size of (a variant of) \gls{gd}},
	first={learning rate},text={learning rate} }

\newglossaryentry{featuremap}{name={feature map}, description={A map that transforms the original  
		 \gls{feature}s of a \gls{datapoint} into new \gls{feature}s. The so-obtained new \gls{feature}s might 
		 be preferable over the original features for several reasons. For example, the shape of datasets might 
		 become simpler in the new feature space, allowing to use linear models in the new \gls{feature}s. 
		 Another reason could be that the number of new \gls{feature}s is much smaller which is preferable 
		 in terms of avoiding \gls{overfitting}. The special case of feature maps that deliver two numeric features are particulary 
		 useful for data visualization. Indeed, we can then depict \gls{datapoint}s in a \gls{scatterplot} by using these two features as the 
		 coordinates of a \gls{datapoint}.},
	first={feature map},text={feature map} }
 
  \newglossaryentry{lasso}{name={ least absolute shrinkage and selection operator (Lasso)}, 
	description={The least absolute shrinkage and selection operator (Lasso) is an instance of \gls{srm} for 
		learning the weights $\weights$ of a linear map $h(\featurevec) = \weights^{T} \featurevec$. 
		The Lasso minimizes the sum consisting of an average squared error loss (as in \gls{linreg}) 
		and the scaled $\ell_{1}$ norm of the weight vector $\weights$. 
	},
	first={ least absolute shrinkage and selection operator (Lasso)},text={Lasso} }
 
 
 

 
 \newglossaryentry{simgraph}{name={similarity graph}, 
 	description={Some applications generate \gls{datapoint}s that are related by a domain-specific 
 		notion of similarity. These similarities can be represented conveniently using a similarity 
 		graph $\graph = \big(\nodes \defeq \{1,\ldots,\samplesize\},\edges\big)$. 
 		The node $\sampleidx \in \nodes$ represents the $\sampleidx$-th \gls{datapoint}. Two 
 		nodes are connected by an undirected edge if the corresponding \gls{datapoint}s are similar. 
 	},
 	first={similarity graph},text={similarity graph} }
 
 
 \newglossaryentry{kld}{name={Kullback-Leibler divergence}, 
 	description={
 		 The Kullback–Leibler divergence is a quantitive measure for how much one \gls{probdist} 
 		 is different from another \gls{probdist} \cite{coverthomas}.  
 	},
 	first={Kullback-Leibler divergence},text={KL divergence} }

\newglossaryentry{LapMat}{name={Laplacian matrix}, 
	description={
		The geometry or structure of a graph $\graph$ can be analyzed using the properties 
		of special matrices that are associated with $\graph$. One such matrix is the graph Laplacian 
		matrix $\mL$ which is defined for an undirected and weighted graph (e.g., the \gls{empgraph} of networked data) \cite{Luxburg2007,Ng2001}. 
	},
	first={Laplacian matrix},text={Laplacian matrix} }


\newglossaryentry{kernel}{name={kernel}, 
	description={Consider \gls{datapoint}s characterized by features $\featurevec \in \featurespace$ with values 
	in some arbirtrary \gls{featurespace}. A kernel is a map that assigns each pair of feature values 
	$\featurevec, \featurevec' \in \featurespace$ a real number. This number measures the similarity between 
	$\featurevec$ and $\featurevec'$. For more details about kernels and the resulting kernel methods, 
	we refer to the literature \cite{LampertNowKernel,LearningKernelsBook}.},
	first={kernel},text={kernel} }

\newglossaryentry{cm}{name={confusion matrix}, 
	description={Consider \gls{datapoint}s characterized by features $\featurevec$ and label $\truelabel$ 
		having value $\clusteridx \in \{1,\ldots,\nrcluster\}$. The confusion matrix is $\nrcluster \times \nrcluster$ matrix 
		with rows representing different values $\clusteridx$ of the true label of a \gls{datapoint}. 
		The columns of a confusion matrix correspond to different values $\clusteridx'$ delivered by a hypothesis $h(\featurevec)$. 
		The $(\clusteridx,\clusteridx')$-th entry of the confusion matrix is the fraction of \gls{datapoint}s 
		with label $\truelabel\!=\! \clusteridx$ and predicted label $\hat{\truelabel}\!=\!\clusteridx'$.},
	first={confusion matrix},text={confusion matrix} }


\newglossaryentry{featurematrix}{name={feature matrix}, 
	description={Conisder a \gls{dataset} $\dataset$ with $\samplesize$ \gls{datapoint}s, each of them 
		characterized by the \gls{feature}s $\featurevec^{(\sampleidx)}$, $\sampleidx=1,\ldots,\samplesize$. 
		The feature matrix $\featuremtx$ of $\dataset$ is constructed by stacking, colum-wise, 
	the \gls{feature}s of the \gls{datapoint}s into a matrix $\featuremtx = \big( \featurevec^{(1)},\ldots, \featurevec^{(\samplesize)} \big)$ 
	of size $\samplesize \times \nrfeatures$.} 
	first={feature matrix},text={feature matrix} }


\newglossaryentry{dbscan}{name={density-based spatial clustering of applications with noise (DBSCAN)}, 
	description={A clustering algorithm for \gls{datapoint}s that are characterized by numeric feature vectors. 
		Similar to \gls{kmeans} and \gls{softclustering} via \gls{gmm} also DBSCAN uses the Euclidean 
		distances between feature vectors to determine the clusters. However, in contrast to these other 
		clustering methods, DBSCAN uses a different notion of similarity between \gls{datapoint}s. 
		In particular, DBSCAN considers two \gls{datapoint}s as similar if they are ``connected'' via 
		a sequence (path) of close-by intermediate \gls{datapoint}s. Thus, DBSCAN might consider 
		two \gls{datapoint}s as similar (and therefore belonging to the same cluster) even if 
		their feature vectors have a large Euclidean distance.},
	first={density-based spatial clustering of applications with noise (DBSCAN)},text={DBSCAN} }

\newglossaryentry{fl}{name={federated learning (FL)}, description={Federated learning is an 
		umbrella term for ML methods that train models in a collaborative fashion using decentralized data and computation.},
	first={federated learning (FL)},text={FL} }
	
\newglossaryentry{cfl}{name={clustered federated learning (CFL)}, description={Clustered \gls{fl} assumes that \gls{localdataset}s 
		clusters. The \gls{localdataset}s belonging to the same cluster have similar statistical properties.},
	first={clustered \gls{fl}},text={CFL} }

\newglossaryentry{iid}{name={i.i.d.}, description={It can be useful to 
		interpret \gls{datapoint}s $\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)}$ 
		as realizations of independent and identically distributed \gls{rv}s with a common \gls{probdist}. 
		If these \gls{rv}s are continuous, their joint \gls{pdf} is $p\big(\datapoint^{(1)},\ldots,\datapoint^{(\samplesize)} \big) = \prod_{\sampleidx=1}^{\samplesize} p \big(\datapoint^{(\sampleidx)}\big)$ with $p(\datapoint)$ being the common 
		marginal \gls{pdf} of the underlying \gls{rv}s.},
	first={independent and identically distributed (i.i.d.)},text={{i.i.d.}} }


\newglossaryentry{outlier}{name={outlier}, description={Many ML methods are 
		motivated by the \gls{iidasspt} which interprets \gls{datapoint}s as realizations of 
		\gls{iid} \gls{rv}s with a common \gls{probdist}. The \gls{iidasspt} is useful for applications  
		where the statistical properties of the data generation process are stationary (time-invariant). 
		However, in some applications the data consists of a majority of ``regular'' \gls{datapoint}s 
		that conform with an \gls{iidasspt} and a small number of data points that have fundamentally different 
        statistical properties compared to the regular \gls{datapoint}s. We refer to a \gls{datapoint} that 
        substantially deviates from the statistical properties of the majority of \gls{datapoint}s as an 
        outlier. Different methods for outlier detection use different measures for this deviation.},
	          first={outlier},text={outlier} }

\newglossaryentry{decisionregion}{name={decision region}, description={Consider a hypothesis map $\hypothesis$ that delivers  
		values from a finite set $\labelspace$. We refer to the set of features $\featurevec \in \featurespace$ 
		that result in the same output $\hypothesis(\featurevec)=a$ as a decision region of the hypothesis $\hypothesis$. },first={decision region},text={decision region} }

\newglossaryentry{decisionboundary}{name={decision region}, description={Consider a \gls{hypothesis} map $h$ that reads in 
		a feature vector $\featurevec \in \mathbb{R}^{\featuredim}$ and delivers a value from a finite set $\labelspace$. 
		The decision boundary induced by $h$ is the set of vectors $\featurevec \in \mathbb{R}^{\featuredim}$ that lie between 
		different\gls{decisionregion}s. More precisely, a vector $\featurevec$ belongs to the decision boundary if and only if 
	each neighbourhood $\{ \featurevec': \| \featurevec - \featurevec' \| \leq \varepsilon \}$, for any $\varepsilon >0$, contains 
  at least two vectors with different function values.},first={decision boundary},text={decision boundary} }


\newglossaryentry{euclidspace}{name={Euclidean space}, description={The Euclidean space $\mathbb{R}^{\featuredim}$ 
		of dimension $\featuredim$ refers to the space of all vectors $\featurevec= \big(\feature_{1},\ldots,\feature_{\featurelen}\big)$, 
		with real-valued entries $\feature_{1},\ldots,\feature_{\featuredim} \in \mathbb{R}$, whose geometry 
		is defined by the inner product $\featurevec^{T} \featurevec' = \sum_{\featureidx=1}^{\featuredim} \feature_{\featureidx} \feature'_{\featureidx}$ 
		between any two vectors $\featurevec,\featurevec' \in \mathbb{R}^{\featuredim}$ \cite{RudinBookPrinciplesMatheAnalysis}.},first={Euclidean space},text={Euclidean space} }

\newglossaryentry{eerm}{name={explainable empirical risk minimization}, description={An instance 
		of structural risk minimization that adds a \gls{regularization} term to the training error in \gls{erm}. 
		The \gls{regularization} term is chosen to favour \gls{hypothesis} maps that are intrinsically 
		explainable for a specific user. This user is characterized by user signals that she provides for 
	the \gls{datapoint}s in a \gls{trainset}.},first={explainable empirical risk minimization (EERM)},text={EERM} }
	
	
\newglossaryentry{kmeans}{name={$k$-means}, description={The $k$-means algorithm 
		is a hard \gls{clustering} method which assigns each \gls{datapoint}s to precisely one out 
		of $\nrcluster$ different clusters. The method iteratively updates this assignment in order to 
		minimize the average distance between \gls{datapoint}s in their nearest cluster mean (centre).},first={$k$-means},text={$k$-means} }


\newglossaryentry{xml}{name={explainable machine learning}, description={Explainable ML 
		methods aim at complementing predictions with explanations for how the prediction has 
		been obtained.},first={explainable ML},text={explainable ML} }

\newglossaryentry{fmi}{name={Finnish Meteorological Institute}, description={The Finnish Meteorological Institute is a 
		government agency responsible for gathering and reporting weather data in Finland.},first={Finnish Meteorological Institute (FMI)},text={FMI} }
	
\newglossaryentry{samplemean}{name={sample mean}, description={The sample mean 
			$\vm \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$ for a given set of \gls{feature} 
			vectors $\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)} \in \mathbb{R}^{\nrfeatures}$ 
			is defined as 
			$$\vm = (1/\samplesize) \sum_{\sampleidx=1}^{\samplesize} \featurevec^{(\sampleidx)}.$$ 
		},
		first={sample mean},text={sample mean} }
	
\newglossaryentry{samplecovmtx}{name={sample covariance matrix}, description={The sample covariance matrix 
		$\widehat{\bf \Sigma} \in \mathbb{R}^{\nrfeatures \times \nrfeatures}$ for a given set of \gls{feature} vectors 
		$\featurevec^{(1)},\ldots,\featurevec^{(\samplesize)} \in \mathbb{R}^{\nrfeatures}$ is defined as 
		$$\widehat{\bf \Sigma} = (1/\samplesize) \sum_{\sampleidx=1}^{\samplesize} (\featurevec^{(\sampleidx)}\!-\!\widehat{\vm}) (\featurevec^{(\sampleidx)}\!-\!\widehat{\vm})^{T}.$$ 
		Here, we used the \gls{samplemean} $\widehat{\vm}$. 
	},
	first={sample covariance matrix},text={sample covariance matrix} }

\newglossaryentry{covmtx}{name={covariance matrix}, description={The covariance matrix of a \gls{rv} $\vx \in \mathbb{R}^{\featuredim}$ 
		is defined as $\expect \bigg \{ \big( \vx - \expect \big\{ \vx \big\} \big)  \big(\vx - \expect \big\{ \vx \big\} \big)^{T} \bigg\}$.},
	first={covariance matrix},text={covariance matrix} }
	
\newglossaryentry{highdimregime}{name={high-dimensional regime}, description={The high-dimensional regime of \gls{erm} is 
		characterized by the \gls{effdim} of the \gls{model} being larger than the \gls{samplesize}, i.e., the number of (labeled) \gls{datapoint}s 
		in the \gls{trainset}. For example, \gls{linreg} methods operate in the high-dimensional regime whenever the number $\featuredim$ of \gls{feature}s 
		used to characterize \gls{datapoint}s exceeds the number of \gls{datapoint}s in the \gls{trainset}. Another example 
		for ML methods that operate in the high-dimensional regime is deep learning with large \gls{ann}s, having 
		more tunable weights (and bias terms) than the number of \gls{datapoint}s in the \gls{trainset}. High-dimensional 
		statistics is a recent main thread of probability theory that studies the behavior of ML methods in the high-dimensional 
		regime \cite{Wain2019,BuhlGeerBook}.},
   first={high-dimensional regime},text={high-dimensional regime} }

\newglossaryentry{gmm}{name={Gaussian mixture model}, description={Gaussian mixture models (GMM) are a family of 
		\gls{probmodel}s for \gls{datapoint}s characterized by a numeric \gls{feature} vector $\featurevec$. A GMM interprets 
	     $\featurevec$ as being drawn from one out of $\nrcluster$ different \gls{mvndist}s $p^{(\clusteridx)} = \mvnormal{\meanvec{\clusteridx}}{\covmtx{\clusteridx}}$, indexed by $\clusteridx=1,\ldots,\nrcluster$. 
	     The probability that $\featurevec$ is drawn from the $\clusteridx$-th \gls{mvndist} is 
	     denoted $p_{\clusteridx}$. Thus, a GMM is parametrized by the probability $p_{\clusteridx}$, the 
		mean vector $\clustermean^{(\clusteridx)}$ and \gls{covmtx} $\clustercov^{(\clusteridx)}$ for each $\clusteridx=1,\ldots,\nrcluster$. 
	 },first={Gaussian mixture model (GMM)},text={GMM} }
 
\newglossaryentry{ml}{name={maximum likelihood}, description={
		Consider \gls{datapoint}s $\dataset=\big\{ \datapoint^{(1)}, \ldots, \datapoint^{(\samplesize)} \}$ that are interpreted 
		as realizations of \gls{iid} \gls{rv}s with a common \gls{probdist} $\prob{\datapoint; \weights}$ which 
		depends on a parameter vector $\weights \in \mathcal{W} \subseteq \mathbb{R}^{n}$. Maximum likelihood methods aim at finding a parameter vector $\weights$ 
		such that the probability (density) $\prob{\dataset; \weights} = \prod_{\sampleidx=1}^{\samplesize} \prob{\datapoint^{(\sampleidx)}; \weights}$ 
		of observing the data is maximized. Thus, the maximum 
		likelihood estimator is obtained as a solution to the optimization problem $\max_{\weights \in \mathcal{W}} \prob{\dataset; \weights}$.
	%	Loosely speaking, we try out all possible parameter vectors $\weights$ and determine the resulting 
%		probability of observing the given \gls{datapoint}s if they would be \gls{iid} with common \gls{probdist} $\prob{\datapoint; \weights}$. 
		%The maximum likelihood estimate is the parameter vector that results in the highest probability (density). 
	},first={maximum likelihood},text={maximum likelihood}}



\newglossaryentry{em}{name={expectation maximization}, description={Expectation maximization is a generic 
		technique for estimating the parameters of a probabilistic model (a parametrized \gls{probdist}) $\prob{\datapoint; \weights}$ 
		from data \cite{BishopBook,hastie01statisticallearning,GraphModExpFamVarInfWainJor}. Expectation maximization 
		delivers an approximation to the \gls{ml} estimate for the model parameters $\weights$. 
  },first={expectation maximization (EM)},text={EM}}

\newglossaryentry{ppca}{name={probabilistic PCA}, description={Probabilistic \gls{pca} (PPCA) 
		extends basic \gls{pca} by using a \gls{probmodel} for \gls{datapoint}s. The \gls{probmodel} of PPCA 
		reduces the task of dimensionality reduction to an estimation problem that can be solved using \gls{em} 
		methods.},first={probabilistic PCA (PPCA)},text={PPCA}}
	
\newglossaryentry{polyreg}{name={polynomial regression}, description={Polynomial regression aims at learning a 
			polynomial \gls{hypothesis} map to predict a numeric \gls{label} based on numeric \gls{feature}s of a \gls{datapoint}. 
			For \gls{datapoint}s characterized by a single numeric \gls{feature}s, polynomial regression uses the \gls{hypospace} 
			$\hypospace^{(\rm poly)}_{\nrfeatures} \defeq \{ \hypothesis(x) = \sum_{\featureidx=0}^{\nrfeatures-1} x^{\featureidx} \weight_{\featureidx} \}.$
			The quality of a polynomial \gls{hypothesis} map is measured using the average \gls{sqerrloss} 
			incurred on a set of labeled \gls{datapoint}s (which we refer to as \gls{trainset}).},first={polynomial regression},text={polynomial regression}}

\newglossaryentry{linreg}{name={linear regression}, description={Linear regression aims at learning a 
		linear \gls{hypothesis} map to predict a numeric \gls{label} based on numeric \gls{feature}s of a \gls{datapoint}. 
		The quality of a linear \gls{hypothesis} map is measured using the average \gls{sqerrloss} incurred on a set 
  	    of labeled \gls{datapoint}s (which we refer to as \gls{trainset}).},first={linear regression},text={linear regression}}
        
\newglossaryentry{ridgeregression}{name={ridge regression}, description={Ridge regression learns 
		the parameter (or weight) vector $\weights$ of a linear \gls{hypothesis} map $\hypothesis^{(\weights)}(\featurevec)= \weights^{T} \featurevec$. 
		The quality of a particular choice for the parameter vector $\weights$ is measured by the sum 
		of two components. The first component is the average \gls{sqerrloss} incurred by $\hypothesis^{(\weights)}$ on a set of 
		labeled \gls{datapoint}s (the \gls{trainset}). The second component is the scaled squared 
		Euclidean norm $\regparam \| \weights \|^{2}_{2}$ with a \gls{regularization} parameter 
		$\regparam > 0$. It can be shown that the effect of adding to $\regparam \| \weights \|^{2}_{2}$ to 
	the average \gls{sqerrloss} is equivalent to replacing the original \gls{datapoint}s by an ensemble of 
realizations of a \gls{rv} centered around these \gls{datapoint}s.},first={ridge regression},text={ridge regression}}


\newglossaryentry{expectation}{name={expectation}, description={Consider a numeric \gls{rv} $\featurevec$ with \gls{probdist} $p(\featurevec)$. 
		The expectation of $\featurevec$ is defined as the integral $\expect \{ \featurevec \} \defeq \int \featurevec p(\featurevec)$ (if this integral 
		is well-defined!) \cite{HalmosMeasure,BillingsleyProbMeasure,RudinBookPrinciplesMatheAnalysis}.},first={expectation},text={expectation}}

\newglossaryentry{logreg}{name={logistic regression}, description={Logistic regression learns a 
		linear \gls{hypothesis} map (classifier) $\hypothesis(\featurevec) = \weights^{T} \featurevec$ 
		to predict a binary \gls{label} $\truelabel$ based on numeric \gls{feature}s $\featurevec$ of a \gls{datapoint}. 
		The quality of a linear \gls{hypothesis} map is measured using its average \gls{logloss} 
		on some labeled \gls{datapoint}s (the \gls{trainset}).},first={logistic regression},text={logistic regression}}
	
\newglossaryentry{logloss}{name={logistic loss}, description={Consider a \gls{datapoint} that is 
		characterized by the features $\featurevec$ and a binary label $\truelabel \in \{-1,1\}$. 
		We use a real-valued \gls{hypothesis} $\hypothesis$ to predict the label $\truelabel$ solely
		 from the features $\featurevec$. 
		The logistic loss incurred by a specific \gls{hypothesis} $\hypothesis$ is defined as 
	\begin{equation} 
		\label{equ_log_loss_gls}
		\loss{(\featurevec,\truelabel)}{\hypothesis} \defeq  \log ( 1 + \exp(- \truelabel \hypothesis(\featurevec))).
\end{equation}. Carefully note that the expression \eqref{equ_log_loss_gls} for the logistic loss 
applies only for the \gls{labelspace} $\labelspace = \{ -1,1\}$ and using the 
     thresholding rule \eqref{equ_def_threshold_bin_classifier}. },first={logistic loss},text={logistic loss}}
	
\newglossaryentry{hingeloss}{name={hinge loss}, description={Consider a \gls{datapoint} that is 
		characterized by a \gls{feature} vector $\featurevec \in \mathbb{R}^{\featuredim}$ and a 
		binary \gls{label} $\truelabel \in \{-1,1\}$. The hinge loss incurred by a specific \gls{hypothesis} $\hypothesis$ 
		is defined as 
		\begin{equation} 
			\label{equ_hinge_loss_gls}
				\loss{(\featurevec,\truelabel)}{\hypothesis} \defeq \max \{ 0 , 1 - \truelabel \hypothesis(\featurevec) \}. 
			\end{equation}
	    A regularized variant of the hinge loss is used by the \gls{svm} \cite{LampertNowKernel} to learn a \gls{linclass} 
	    with maximum margin between the two classes (see Figure \ref{fig_svm_gls}). 
		\begin{figure}[htbp]
			\begin{center}
				\begin{tikzpicture}[auto,scale=0.8]
					%\draw [thick] (0,-3) rectangle (4,4) node [anchor=east,above] {$\featurespace$} ;
					\draw [thick] (1,2) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(5)}$};
					\draw [thick] (0,1.6) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(4)}$};
					\draw [thick] (0,3) circle (0.1cm)node[anchor=west] {\hspace*{0mm}$\featurevec^{(3)}$};
					\draw [thick] (2,1) circle (0.1cm)node[anchor=east,above] {\hspace*{0mm}$\featurevec^{(6)}$};
					\node[] (B) at (-2,0) {``support vector''};
					\draw[->,dashed] (B) to (1.9,1) ; 
					\draw [|<->|,thick] (2.05,0.95)  -- (2.75,0.25)node[pos=0.5] {$\xi$} ; 
					\draw [thick] (1,-1.5) -- (4,1.5) node [right] {$h^{(\weights)}$} ; 
					\draw [thick] (3,-1.9) rectangle ++(0.1cm,0.1cm) node[anchor=west,above]  {\hspace*{0mm}$\featurevec^{(2)}$};
					\draw [thick] (4,.-1) rectangle ++(0.1cm,0.1cm) node[anchor=west,above] {\hspace*{0mm}$\featurevec^{(1)}$};
				\end{tikzpicture}
				\caption{The \gls{svm} learns a hypothesis (or classifier) $h^{(\weights)}$ with minimum average 
					soft-margin \gls{hingeloss}. Minimizing this \gls{loss} is equivalent to maximizing 
					the margin $\xi$ between the \gls{decisionboundary} of $\hypothesis^{(\weights)}$ 
					and each class of the \gls{trainset}.}
				\label{fig_svm_gls}
			\end{center}
		\end{figure}
	},first={hinge loss},text={hinge loss}}

\newglossaryentry{iidasspt}{name={i.i.d.\ assumption}, description={The i.i.d.\ assumption interprets \gls{datapoint}s of a \gls{dataset} 
		as the realizations of \gls{iid} \gls{rv}s.},first={i.i.d.\ assumption},text={i.i.d.\ assumption} }

\newglossaryentry{hypospace}{name={hypothesis space}, description={Every practical ML method uses a specific hypothesis
		 space (or \gls{model}) $\hypospace$. The hypothesis space of a ML method is a subset of all possible maps 
		from the \gls{featurespace} to \gls{labelspace}. The design choice of the hypothesis space should take into 
		account available computational resources and statistical aspects. If the computational infrastructure 
		allows for efficient matrix operations, and there is a (approximately) linear relation between \gls{feature}s and \gls{label}, 
		a useful choice for the hypothesis space might be the \gls{linmodel}.},first={hypothesis space},text={hypothesis space} }
	
\newglossaryentry{model}{name={model}, description={We use the term model as a synonym for \gls{hypospace}},first={model},text={model} }

\newglossaryentry{modelparams}{name={model parameters}, 
	description={Model parameters are numbers that select a \gls{hypothesis} map out of a \gls{hypospace}.},
	first={model parameters},text={model parameters} }

\newglossaryentry{ai}{name={artificial intelligence}, description={Artificial intelligence aims to develop systems that
		behave rational in the sense of maximizing a long-term reward.},first={artificial intelligence (AI)},text={AI} }
	
\newglossaryentry{hardclustering}{name={hard clustering}, description={Hard clustering refers to the task of 
		partitioning a given set of \gls{datapoint}s into (few) non-overlapping clusters. Each \gls{datapoint} is 
		assigned to one specific cluster.},first={hard clustering},text={hard clustering} }
	
\newglossaryentry{softclustering}{name={soft clustering}, description={Soft clustering refers to the task 
		of partitioning a given set of \gls{datapoint}s into (few) overlapping clusters. Each \gls{datapoint} is 
		assigned to several different clusters with varying \gls{dob}. Soft clustering amounts to determining 
		such a \gls{dob} (or soft cluster assignment) for each \gls{datapoint} and each \gls{cluster}.},first={soft clustering},text={soft clustering} }
	
\newglossaryentry{clustering}{name={clustering}, description={Clustering methods decompose a given 
		set of \gls{datapoint}s into few subsets, which are referred to as clusters. Each cluster consists of \gls{datapoint}s 
		that are more similar to each other than to \gls{datapoint}s outside the cluster. 
		Different clustering methods use different measures for the similarity between \gls{datapoint}s and different 
		representation of clusters. The clustering method \gls{kmeans} uses the average feature vector (``cluster means'') 
		of a cluster as its representative. A popular soft-clustering method based on \gls{gmm} represents 
		a cluster by a \gls{mvndist}.},first={clustering},text={clustering} }
	
\newglossaryentry{clusterempgraph}{name={cluster}, description={A cluster within an \gls{empgraph} is a subset 
		of nodes that carry local datasets with (nearly) identical statistical distributions. Clustered \gls{fl} aims at identying 
		the clusters and use the pooled local darasets to train a separate model for each cluster.},first={cluster},text={cluster} }
	
\newglossaryentry{cluster}{name={cluster}, description={A cluster is a subset of \gls{datapoint}s that are more 
	similar to each other than to the \gls{datapoint}s outside the cluster.	The notion and measure of similarity 
	between \gls{datapoint}s is a design choice. If \gls{datapoint}s are characterized by numeric feature 
	 vectors in some \gls{euclidspace} we can define the similarity between two \gls{datapoint}s via the 
	 Euclidean distance between their feature vectors.},first={cluster},text={cluster} }

%\newglossaryentry{softclustering}{name={soft clustering}, description={Soft clustering methods determine, for each \gls{datapoint} within a dataset, 
%		a soft cluster assignment or the degree of belonging to a particular cluster.},first={soft clustering},text={soft clustering} }


\newglossaryentry{huberloss}{name={Huber loss}, description={The Huber loss is a mixture of the squared error loss 
		and the absolute value of the prediction error.},first={Huber loss},text={Huber loss} }

\newglossaryentry{svm}{name={support vector machine}, description={A binary classification method for learning a 
		linear \gls{hypothesis} map that maximally separates \gls{datapoint}s from the two different classes in the \gls{feature} space (``maximum margin''). Maximizing this 
		separation is equivalent to minimizing a regularized variant of the \gls{hingeloss} \eqref{equ_hinge_loss_gls}.},first={support vector machine (SVM)},text={SVM} }

\newglossaryentry{eigenvalue}{name={eigenvalue}, description={We refer to a number $\lambda \in \mathbb{R}$ 
		as eigenvalue of a square matrix $\mathbf{A} \in \mathbb{R}^{\featuredim \times \featuredim}$ if there is a 
		non-zero vector $\vx \in \mathbb{R}^{\featuredim} \setminus \{ \mathbf{0} \}$ such that $\mathbf{A} \vx = \lambda \vx$. },first={eigenvalue},text={eigenvalue} }
	
\newglossaryentry{eigenvector}{name={eigenvector}, description={An eigenvector of a matrix $\mathbf{A}$ is a 
		non-zero vector $\vx \in \mathbb{R}^{\featuredim} \setminus \{ \mathbf{0} \}$ such that $\mathbf{A} \vx = \lambda \vx$ 
	with some \gls{eigenvalue} $\lambda$.},first={eigenvector},text={eigenvector} }

\newglossaryentry{evd}{name={eigenvalue decomposition}, 
	description={The eigenvalue decomposition for a square matrix 
		$\mA \in \mathbb{R}^{\dimlocalmodel \times \dimlocalmodel}$ 
		is a factorization of the form 
		$$\mA = \mathbf{V} {\bm \Lambda} \mathbf{V}^{-1}.$$ 
		The columns of the matrix $\mV = \big( \vv^{(1)},\ldots,\vv^{(\dimlocalmodel)} \big)$ are the 
		\gls{eigenvector}s of the matrix $\mV$. The diagonal matrix 
		${\bm \Lambda} = {\rm diag} \big\{ \eigval{1},\ldots,\eigval{\dimlocalmodel} \big\}$ 
		contains the \gls{eigenvalue}s $\eigval{\featureidx}$ corresponding to the \gls{eigenvector}s $\vv^{(\featureidx)}$. 
		Note that the above decomposition exists only if the matrix $\mA$ is diagonalizable.},first={eigenvalue decomposition (EVD)},text={EVD} }

%\newglossaryentry{svd}{name={singular value decomposition}, 
%	description={The singular value decomposition for a matrix 
%		$\mA \in \mathbb{R}^{\samplesize \times \dimlocalmodel}$ 
%		is a factorization of the form 
%		$$\mA = \mathbf{V} {\bm \Lambda} \mathbf{U}^{T},$$ 
%		with orthonormal matrices $\mV \in \mathbb{R}^{\samplesize \times \samplesize}$ and $\mU \in \mathbb{R}^{\dimlocalmodel \times \dimlocalmodel}$. 
%		The matrix ${\bm \Lambda} \in \mathbb{R}^{\samplesize \times \dimlocalmodel}$ is only non-zero 
%		along the main diagonal, whose entries $\Lambda_{\featureidx,\featureidx}$ are non-negative and 
%		referred to as singular values. In contrast to the EVD, which only exists for diagonalizable 
%		matrices, we can find a SVD for any matrix.
%	},first={singular value decomposition (SVD)},text={SVD} }


\newglossaryentry{tv}{name={total variation}, description={Consider some \gls{empgraph} whose 
		nodes carry (personalized) \gls{localmodel} \gls{parameters}. 
		The total variation measures the discrepancies between across edges $\edge{\nodeidx}{\nodeidx'}$. 
		%If we measure the \gls{discrepancy}} as $\normgeneric{\localparams{\nodeidx}- \localparams{\nodeidx'}}{2}^{2}$, 
		%we define the total variation as $\sum_{\nodeidx,\nodeidx'} \edgeweight_{\nodeidx,\nodeidx'} \normgeneric{\localparams{\nodeidx}- \localparams{\nodeidx'}}{2}^{2}$.  
		},
	first={total variation},text={total variation} }


\newglossaryentry{gdmethods}{name={gradient-based method}, description={Gradient-based methods 
		are iterative algorithms for finding the minimum (or maximum) of a \gls{differentiable} 
		objective function of the \gls{modelparams}. These algorithms construct a sequence of 
		approximations to an optimal choice for \gls{modelparams} that results in a minimum objective function value. 
		As their name indicates, gradient-based methods use the \gls{gradient}s of the objective function 
		evaluated during previous iterations to construct new (hopefully) improved \gls{modelparams}.},
		first={gradient-based methods},text={gradient-based methods} }

\newglossaryentry{sgd}{name={subgradient descent}, description={Subgradient descent is a 
		generalization of \gls{gd} that does not require differentiablity of the function to be minimized. 
		This generalization is obtained by replacing the concept of a \gls{gradient} with that of a sub-gradient. 
		Similar to \gls{gradient}s, also sub-gradients allow to construct local approximations of an objective function. 
		The objective function might be the \gls{emprisk} $\emperror\big( \hypothesis^{(\weights)} \big| \dataset \big)$ viewed 
		as a function of the \gls{modelparams} $\weights$ that select a \gls{hypothesis} $\hypothesis^{(\weights)} \in \hypospace$.},first={subgradient descent},text={subgradient descent} }
	
\newglossaryentry{stochGD}{name={stochastic gradient descent}, description={Stochastic \gls{gd} is 
		obtained from \gls{gd} by replacing the \gls{gradient} of the objective function with a noisy (or stochastic) 
		estimate.},first={stochastic gradient descent (SGD)},text={SGD} }

\newglossaryentry{pca}{name={principal component analysis (PCA)}, description={Principal component analysis 
		determines a given number of new features that are obtained by a linear transformation (map) of the 
		raw features. },first={principal component analysis (PCA)},text={PCA} }
	
\newglossaryentry{loss}{name={loss}, description={With a slight abuse of language, we use the term loss either for
		the \gls{lossfunc} itself or for its value for a specific pair of a \gls{datapoint} and a \gls{hypothesis}.},first={loss},text={loss} }

\newglossaryentry{lossfunc}{name={loss function}, description={A loss function is a map 
		$$\lossfun: \featurespace \times \labelspace \times \hypospace \rightarrow \mathbb{R}_{+}: \big( \big(\featurevec,\truelabel\big), \hypothesis\big) \mapsto  \loss{(\featurevec,\truelabel)}{\hypothesis}$$ which assigns a pair consisting of a \gls{datapoint}, with features $\featurevec$ 
		and label $\truelabel$, and a hypothesis $\hypothesis \in \hypospace$ the non-negative real number $\loss{(\featurevec,\truelabel)}{h}$. 
		The loss value $\loss{(\featurevec,\truelabel)}{\hypothesis}$ quantifies the discrepancy between the true label $\truelabel$ 
		and the predicted label $\hypothesis(\featurevec)$. Smaller (closer to zero) values $\loss{(\featurevec,\truelabel)}{\hypothesis}$ 
		mean a smaller discrepancy between predicted label and true label of a \gls{datapoint}. Figure \ref{fig_loss_function_gls} 
		depicts a \gls{lossfunc} for a given \gls{datapoint}, with features $\featurevec$ and label $\truelabel$, as a 
		function of the \gls{hypothesis} $\hypothesis \in \hypospace$. \begin{figure}[htbp]
			\begin{center}
				\begin{tikzpicture}[scale = 0.7]
					\begin{axis}
						[%grid, 
						axis x line=center,
						axis y line=center,
						%	xtick={-2,-1,...,2},
						%	ytick={0,1,...,2},
						xlabel={\hspace*{3mm} hypothesis $\hypothesis$},
						%	ylabel={\hspace*{3mm} loss $\lossfun$},
						xlabel style={below right},
						ylabel style={above right},
						xtick=\empty,
						ytick=\empty,
						xmin=-4,
						xscale = 1.4, 
						xmax=4,
						ymin=-0.5,
						ymax=2.5
						]
						\addplot [smooth, ultra thick] table [x=a, y=b, col sep=comma] {logloss.csv};    
						%	\addplot [color=blue, ultra thick] table [x=a, y=b, col sep=comma] {hingeloss.csv};     
						%	\addplot [color=black, ultra thick] table [x=a, y=b, col sep=comma] {zerooneloss.csv};     
						%		\addplot[domain=-1:4, thin,dashed] {(x-1)^2};
					\end{axis}
					%	\node [right] at (10,5) {very confident in $\predictedlabel\!=\!1 \Rightarrow$}; 
					\node [above] at (1,5) {$\loss{(\featurevec,\truelabel)}{\hypothesis}$};
					%		\node [right] at (7,3) {squared error (for $\truelabel\!=\!1$)};
					%		\node [right,color=blue] at (4,4) {hinge loss (for $\truelabel\!=\!1)$};
					%		\node [left] at (2.5,3) {$0/1$ loss (for $\truelabel\!=\!1)$};
					%		\node [left] at (2,5) {$\Leftarrow$ very confident in $\predictedlabel\!=\!-1$};
				\end{tikzpicture}
			\end{center}
			\vspace*{-7mm}
			\caption{Some \gls{lossfunc} $\loss{(\featurevec,\truelabel)}{\hypothesis}$ for a fixed \gls{datapoint}, with 
				\gls{feature} vector $\featurevec$ and \gls{label} $\truelabel$, and varying \gls{hypothesis} $\hypothesis$. 
				ML methods try to find (learn) a \gls{hypothesis} that incurs minimum \gls{loss}.}
			\label{fig_loss_function_gls}
	\end{figure}
 },first={loss function},text={loss function} }

\newglossaryentry{decisiontree}{name={decision tree}, description={A decision tree is a flow-chart 
		like representation of a hypothesis map $h$. More formally, a decision tree is a directed graph 
		which reads in the feature vector $\featurevec$ of a \gls{datapoint} at its root node. The root node 
		then forwards the \gls{datapoint} to one of its children nodes based on some elementary test on 
		the features $\featurevec$. If the receiving children node is not a leaf node, i.e., it has itself children nodes, 
	  it represents another test. Based on the test result, the \gls{datapoint} is further pushed to one of its neighbours. This testing and 
	  forwarding of the \gls{datapoint} is repeated until the \gls{datapoint} ends up in a leaf node (having no children nodes). 
	  The leaf nodes represent sets (decision regions) constituted by feature vectors $\featurevec$ that are mapped to 
	  the same function value $h(\featurevec)$.},first={decision tree},text={decision tree} }

\newglossaryentry{noniiddata}{name={non i.i.d.\ data}, description={A dataset consisting of \gls{datapoint}s 
		that cannot be well modelled as \gls{realization}s of \gls{iid} \gls{rv}s.},first={non-i.i.d.\ data},text={non-i.i.d.\ data} }
	
	


%\newglossaryentry{linclass}
%{
%	name=linear classifier,
%	description={A linear classifier $h(\vx)$ divides the feature space $\mathbb{R}^{\featurelen}$ into two half-spaces 
%		such that data points in the same half-space result in the same predicted label.}
%}

\newglossaryentry{API} 
{
	name={Application Programming Interface (API)},
	description={An Application Programming Interface (API) is a particular set of rules and 
		specifications that a software program can follow to access and make use of the services 
		and resources provided by another software program that implements that API.},
	first={Application Programming Interface (API)},
	text={API}
}

\newglossaryentry{hilbertspace}{name={Hilbert space},description={A Hilbert space is a linear vector space 
		that is equipped with an inner product between pairs of vectors. One important example for a Hilbert 
		space is the Euclidean spaces $\mathbb{R}^{\featuredim}$, for some dimension $\featuredim$, which 
		consists of Euclidean vectors $\vu = \big(u_{1},\ldots,u_{\featurelen}\big)^{T}$ along with the inner 
		product $\vu^{T} \vv$.},first={Hilbert space},text={Hilbert space}}



\newglossaryentry{sample}{name={sample},description={A finite sequence (list) of \gls{datapoint}s $\datapoint^{(1)},\ldots,\datapoint^{(\sampleidx)}$ that 
		is obtained or interpreted as the realizations of $\samplesize$ \gls{iid} \gls{rv}s with the common \gls{probdist} $p(\datapoint)$.
		The length $\samplesize$ of the sequence is referred to as the \gls{samplesize}.},first={sample},text={sample}}
	
\newglossaryentry{samplesize}
{name=sample size,
	description={The number of individual \gls{datapoint}s contained in a dataset that is 
	obtained from realizations of \gls{iid} \gls{rv}s.},first={sample size},text={sample size}
}

\newglossaryentry{ann}
{name=artificial neural network,
	description={An artificial neural network is a graphical (signal-flow) representation of a map from 
		features of a \gls{datapoint} at its input to a predicted label at its output.},first={artificial neural network (ANN)},text={ANN}
}

\newglossaryentry{randomforest}
{name=random forest,
	description={A random forest is a set (ensemble) of different \gls{decisiontree}s. Each of these \gls{decisiontree}s is 
		obtained by fitting a perturbed copy of the original dataset.},first = {random forest}, text={random forest}
}

\newglossaryentry{bagging}{name={bagging},description={bagging (or ``bootstrap aggregation'') is a generic 
		technique to improve (the robustness of) a given ML method. The idea is to use the bootstrap to generate 
		perturbed copy of a given training set and then apply the original ML method to learn a separate 
		hypothesis for each perturbed copy of the training set. The resulting set of hypotheses is then 
		used to predict the label of a \gls{datapoint} by combining or aggregating the individual predictions of each 
		individual hypothesis. For hypotheses that deliver numeric label values (regression methods) this 
		aggregation could be implemented by computing the average of individual predictions.},first={bootstrap aggregation (bagging)},text={bagging}}

\newglossaryentry{gd}{name={gradient descent (GD)},description={Gradient descent is an iterative method for finding the minimum 
		of a differentiable function $f(\weights)$. },first={gradient descent (GD)},text={GD}}


\newglossaryentry{ladregression}{name={least absolute deviation regression},description={Least absolute deviation regression uses 
		the average of the absolute precondition errors to find a linear hypothesis.},first={least absolute deviation regression},
	   text={least absolute deviation regression}}



\newglossaryentry{metric}{name={metric},description={A metric refers to a loss function that is used solely 
	    for the final performance evaluation of a learnt hypothesis. The metric is typically a \gls{lossfunc} that 
	    has a ``natural'' interpretation (such as the \gls{zerooneloss}) but is not a good choice to guide 
	    the learning process, e.g., via \gls{erm}. For \gls{erm}, we typically prefer \gls{lossfunc}s that depend smoothly 
	    on the (parameters of the) hypothesis. Examples for such smooth \gls{lossfunc}s include the \gls{sqerrloss} \eqref{equ_squared_loss_gls} and the \gls{logloss} \eqref{equ_log_loss_gls}.},first={metric},text={metric}}

\newglossaryentry{bayesrisk}{name={Bayes risk},description={We use the term Bayes risk as a synonym for the \gls{risk} or expected \gls{loss} 
		of a hypothesis. Some authors reserve the term Bayes risk for the \gls{risk} of a hypothesis that achieves minimum \gls{risk}, such a hypothesis 
		being referred to as a \gls{bayesestimator} \cite{LC}.},first={Bayes risk},text={Bayes risk}}
	
\newglossaryentry{bayesestimator}{name={Bayes estimator},description={A \gls{hypothesis} $\hypothesis$ 
		whose \gls{bayesrisk} is minimal \cite{LC}.},first={Bayes estimator},text={Bayes estimator}}




\newglossaryentry{weights}{name={weights},
	description={We use the term weights synonymously for a finite set of parameters within a \gls{model}. 
		For example, the linear model consists of all linear maps $h(\featurevec)= \weights^{T} \featurevec$ 
		that read in a feature vector $\featurevec=\big(\feature_{1},\ldots,\feature_{\featurelen}\big)^{T}$ of a \gls{datapoint}. 
		Each specific linear map is characterized by specific choices for the parameters for weights $\weights = \big( \weight_{1},\ldots,\weight_{\featuredim}\big)^{T}$.},first={weights},text={weights}}
	
\newglossaryentry{probdist}{name={probability distribution},
	description={The \gls{data} generated in some ML applications can be reasonably well modelled as 
		realizations of a \gls{rv}. The overall statistical properties (or intrinsic structure) of such \gls{data} 
		are then governed by the probability distribution of this \gls{rv}. We use the term probability distribution 
		in a highly informal manner and mean the collection of probabilities assigned to different values or value 
		ranges of a \gls{rv}. The probability distribution of a binary \gls{rv} $\truelabel \in \{0,1\}$ is fully specified 
		by the probabilities $\prob{\truelabel = 0}$ and $\prob{\truelabel=1} \big(\!=\!1\!-\!\prob{\truelabel=0} \big)$. 
	    The probability distribution of a real-valued \gls{rv} $\feature \in \mathbb{R}$ might be specified 
	    by a probability density function $p(\feature)$ such that $\prob{ \feature \in [a,b] } \approx  p(a) |b-a|$. 
	    In the most general case, a probability distribution is defined by a probability measure \cite{GrayProbBook,BillingsleyProbMeasure}.},first={probability distribution},text={probability distribution}}
    
    
\newglossaryentry{pdf}{name={probability density function (pdf)},
	description={The probability density function (pdf) $p(\feature)$ of a real-valued 
		\gls{rv} $\feature \in \mathbb{R}$ is a particular representation of its \gls{probdist}. 
		If the pdf exists, it can be used to compute the probability that $\feature$ takes on a 
		value from a (measurable) set $\mathcal{B} \subseteq \mathbb{R}$ via $\prob{\feature \in \mathcal{B}} = \int_{\mathcal{B}} p(\feature') d \feature'$ \cite[Ch. 3]{BertsekasProb}. The pdf of a vector-valued \gls{rv} $\featurevec \in \mathbb{R}^{\featuredim}$ (if it exists) 
        allows to compute the probability that $\featurevec$ falls into a (measurable) region $\mathcal{R}$ via 
        $\prob{\featurevec \in \mathcal{R}} = \int_{\mathcal{R}} p(\featurevec') d \feature_{1}' \ldots d \feature_{\featuredim}' $ \cite[Ch. 3]{BertsekasProb}.},
first={probability density function (pdf)},text={pdf}}


\newglossaryentry{parameters}{name={parameters},
	description={The parameters of a ML \gls{model} are tunable (learnable or adjustable) quantities that 
		allow to choose between different hypothesis maps. For example, the linear model $\hypospace \defeq \{h: h(\feature)= \weight_{1} \feature + \weight_{2}\}$ consists  of all hypothesis maps $h(\feature)= \weight_{1} \feature + \weight_{2}$ with a particular 
		choice for the parameters $\weight_{1},\weight_{2}$. Another example of parameters are the weights 
		assigned to the connections of an \gls{ann}.},first={parameters},text={parameters}}

\newglossaryentry{lln}{name={law of large numbers},
	description={The law of large numbers refers to the convergence of the average of an increasing (large) 
		number of \gls{iid} \gls{rv}s to the mean (or expectation) of their common \gls{probdist}. Different 
	    instances of the law of large numbers are obtained using different notions of convergence.},first={law of large numbers},text={law of large numbers}}
    
\newglossaryentry{stopcrit}{name={stopping criterion},
	description={Many ML methods use iterative algorithms that construct a sequence of model parameters (such as the weights of a linear map or 
		the weights of an \gls{ann}) that (hopefully) converge to an optimal choice for the model parameters. In practice, given finite computational 
		resources, we need to stop iterating after a finite number of times. A stopping criterion is any well-defined condition required for stopping 
		iterating.},first={stopping criterion},text={stopping criterion}}
    
    
    

\newglossaryentry{kCV}{name={$\nrfolds$-fold cross-validation ($\nrfolds$-fold CV)},
	description={$\nrfolds$-fold cross-validation is a method for learning and validating a \gls{hypothesis} using 
		a given \gls{dataset}. This method first divides the \gls{dataset} evenly into $\nrfolds$ 
		subsets or ``folds'' and then executes $\nrfolds$ repetitions of training and validation. 
		Each repetition uses a different fold as the \gls{valset} and the remaining $\nrfolds-1$ folds 
		as a \gls{trainset}. The final output is the average of the \gls{valerr}s obtained from the $\nrfolds$ repetitions.},first={$\nrfolds$-fold cross-validation ($\nrfolds$-fold CV)},text={$\nrfolds$-fold CV}}
	
\newglossaryentry{renyidiv}{name={R\'enyi divergence}, 
	description={The R\'enyi divergence measures the (dis-)similarity between two \gls{probdist}s.}, 
	first = {R\'enyi divergence}, text = {R\'enyi divergence}} 

\newglossaryentry{nonsmooth}{name={non-smooth},
	description={We refer to a function as non-smooth if it is not \gls{smooth} \cite{nesterov04}.},first={non-smooth},text={non-smooth}}

\newglossaryentry{convex}{name={convex},
	description={A set $\mathcal{C} \subseteq \mathbb{R}^{\featuredim}$ is convex 
		if it contains the line segment between any two points of that set. We define a 
		function as convex if its epigraph is a convex set \cite{BoydConvexBook}.},first={convex},text={convex}}


\newglossaryentry{smooth}{name={smooth},
	description={We refer to a real-valued function as smooth if it is \gls{differentiable} 
		and its \gls{gradient} is continuous \cite{nesterov04,CvxBubeck2015}. In particular, a 
		differentiable function $f(\weights)$ is referred to as $\beta$-smooth if the \gls{gradient} 
		$\nabla f(\weights)$ is Lipschitz continuous with Lipschitz constant $\beta$, i.e., 
		$$\| \nabla f(\weights) - \nabla f(\weights') \| \leq \beta \| \weights - \weights' \|.$$ },first={smooth},text={smooth}}

\newglossaryentry{dataug}{name={data augmentation},
	description={Data augmentation methods add synthetic \gls{datapoint}s to an existing set of \gls{datapoint}s. 
		These synthetic \gls{datapoint}s might be obtained by perturbations (adding noise) or 
		transformations (rotations of images) of the original \gls{datapoint}s.},first={data augmentation},text={data augmentation}}
	
	
\newglossaryentry{localdataset}{name={local dataset},description={The concept of a local dataset is 
		in-between the concept of a \gls{datapoint} and a \gls{dataset}. A local dataset consists of several 
		individual \gls{datapoint}s which are characterized by \gls{feature}s and \gls{label}s. In contrast to a 
		single \gls{dataset} used in basic ML methods, a local dataset is also related to other local datasets via different notions 
		of similarities. These similarities might arise from \gls{probmodel}s or communication infrastructure and 
		are encoded in the edges of an \gls{empgraph}.},first={local dataset},text={local dataset}}
	
\newglossaryentry{localmodel}{name={local model},description={Consider a collections of \gls{localdataset}s that 
		are assigned to the nodes of an \gls{empgraph}. A local model $\localmodel{\nodeidx}$ is a \gls{hypospace} that 
		is assigned to a node $\nodeidx \in \nodes$. Different nodes might be assigned different \gls{hypospace}s, i.e., in general 
		$\localmodel{\nodeidx} \neq \localmodel{\nodeidx'}$ for different nodes $\nodeidx, \nodeidx' \in \nodes$.  },first={local model},text={local model}}
	
\newglossaryentry{mutualinformation}
{name={mutual information},
 description={The mutual information $\mutualinformation{\featurevec}{\truelabel}$ between two \gls{rv}s $\featurevec$, $\truelabel$ 
		defined on the same probability space is given by \cite{coverthomas} $$\mutualinformation{\featurevec}{\truelabel} \defeq \expect \left\{ \log \frac{p (\featurevec,\truelabel)}{p(\featurevec)p(\truelabel)} \right\}.$$ It is a measure for how well we can estimate $\truelabel$ based 
		solely from $\featurevec$. A large value of $\mutualinformation{\featurevec}{\truelabel}$ indicates that 
		$\truelabel$ can be well predicted solely from $\featurevec$. This \gls{prediction} could be obtained by a 
		\gls{hypothesis} learnt by a \gls{erm}-based ML method. 
	 }, first = {mutual information (MI)}, text={MI} 
}

\newglossaryentry{zerogradientcondition}{name={zero-gradient condition},
	description={Consider the unconstrained optimization problem $\min_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights)$  with 
			a \gls{smooth} and \gls{convex} \gls{objfunc} $f(\weights)$. A necessary and sufficient condition 
			for a vector $\widehat{\weights} \in \mathbb{R}^{\dimlocalmodel}$ to solve this problem is that the 
			\gls{gradient} $\nabla f \big( \widehat{\weights} \big)$ is the zero-vector, 
			$$ \nabla f \big( \widehat{\weights} \big) = \mathbf{0} \Leftrightarrow  f \big( \widehat{\weights} \big) = \min_{\weights \in \mathbb{R}^{\dimlocalmodel}} f(\weights) .$$ }, 
			first={zero-gradient condition},text={zero-gradient condition}}


\newglossaryentry{edgeweight}{name={edge weight},
	description={Each edge $\edge{\nodeidx}{\nodeidx'}$ of an \gls{empgraph} is 
		assigned a non-negative edge weight $\edgeweight_{\nodeidx,\nodeidx'}\geq0$. 
		A zero weight $\edgeweight_{\nodeidx,\nodeidx'}=0$ indicates the absence 
		of an edge between 
		nodes $\nodeidx, \nodeidx' \in \nodes$.}, 
	first={edge weight},text={edge weight}}


\newglossaryentry{dataminprinc}{name={data minimization principle},
	description={The data minimization principle is one of the core tenets of the General 
		Data Protection Regulation (GDPR). It dictates that organizations should only collect 
		and process personal data that is adequate, relevant, and limited to what is necessary 
		for the specific purposes for which it is being processed. This principle is encapsulated 
		in Article 5(1)(c) of the GDPR.Key aspects of the data minimization principle:
		\begin{itemize} 
		\item Adequacy: The data collected must be sufficient to fulfill the stated purposes.
		\item Relevance: The data must be relevant and have a clear connection to the purpose for which it is collected.
		\item Limitation: Only the minimum amount of data required should be collected and processed—no more than necessary..
	 \end{itemize}}, 
	first={data minimization principle},text={data minimization principle}}






%\newglossaryentry{psdg}{name={positive semi-definite},
%	description={A matrix $\mathbf{X} \in \mathbb{C}^{\featurelen \times \featurelen}$ is referred to as positive semi-definite if $\vx^{H} \mathbf{X} \vx \geq 0$ for every vector $\vx \in \mathbb{R}^{\featurelen}$.},first={positive semi-definite (psd)},text={psd}}

%%%% define the acronym and use the see= option
%\newglossaryentry{psd}{type=\acronymtype, name={psd}, description={positive semi-definite}, first={positive semi-definite (psd)\glsadd{psdg}}, see=[Glossary:]{psdg}}


